Dynamic Partial Order Reduction for Checking Correctness against Transaction Isolation Levels

Modern applications, such as social networking systems and e-commerce platforms are centered around using large-scale databases for storing and retrieving data. Accesses to the database are typically enclosed in transactions that allow computations on shared data to be isolated from other concurrent computations and resilient to failures. Modern databases trade isolation for performance. The weaker the isolation level is, the more behaviors a database is allowed to exhibit and it is up to the developer to ensure that their application can tolerate those behaviors. In this work, we propose stateless model checking algorithms for studying correctness of such applications that rely on dynamic partial order reduction. These algorithms work for a number of widely-used weak isolation levels, including Read Committed, Causal Consistency, Snapshot Isolation, and Serializability. We show that they are complete, sound and optimal, and run with polynomial memory consumption in all cases. We report on an implementation of these algorithms in the context of Java Pathfinder applied to a number of challenging applications drawn from the literature of distributed systems and databases.

==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/.git/objects/0a/2c672ea402278081c404021e90b0f1e06a7192 <==
xµKNÄ0DYûޏùÿ'bÃ	8AÇÝÉxgè8s~œ•TªÕ+½ºo[Òéø2˜H'u)ÎÅ'OżÅ@ÅÁ…¼dº,ÀԇÑåœfð‹5.óŒ¥ú\M-Éb),^%à÷åGçöu'|¥¿ñNxò›zðªŽUå"2)LÆtööT×Q;6$ÞÇ´ð›41ÚdbˆIÞ´ÕZÔ_‰Aÿ"Ÿx´¾J¦ú#]ïÐW:Ä7*cÙ

==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/.git/objects/10/283727d54396edc3300699243cfd9a0ebd570e <==
x5Ž1OÃ0"™ý+Ž:D‰'!'®J%j;×ÄÄñ‹ž†
ñßI'¾ï\‡‡ûÇ«›ëýæ*Rð"Á†T~™L_'¤õwíû$sdÓr`*ùǘ7¢t6õK6I:2e(O35ã(zقâdãd]$Ždã¬ï+컐1‹ö˜mFžÆQ´°;ÿñê–É[{Ñۈ†ØÑwÔ%¸­·»;´jSù—`Tù\Îâp¨>ËËëjUóŒ7Mí

==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/.git/objects/12/e277e4090df6f641b076351064bfab330aa333 <==
x¥MjA…³îSÔ^Fºkªÿ 	˜+TWWtбµ3'Ǐ˜Ü »ïñ=ió<-€!¾,]Cáú•ÔªÏ$¹XrìˆX"ŒUº,ŒæÂ]ÏP‹'‹\Bv5Ô)0G£èEóX*¦hø¶Z‡í¹Oכ«þ†ÍŽå½µãðÙÛPuøëק&|zb&ÊÎGXYg­'§ï¢ÿ_2Óüz"ÇÞw¾`ÓÌ{ý6?[Um

==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/.git/objects/17/f4c1e93a8a2f4e587ac2f8c4266254b8681293 <==
x¥MjÃ0F³Ö)f_f$ëB("Dˆ!'Œ­@{ûš,z®>x‹Çû¸×ºÐ֟Æ&".™br'ÏÖ»ÈFÓ¬çÙ-Q2e¶Æ©5mÒH™¤Ä0ˆD›µ›'™'6\(å<3²OH*½Æ£oðÕÛ>RKƒ{"W–c>ùïç¥&¾<z•óÑ9gá	Qñ;wÈ¿EJ¾Wٖz|Ø¡ö}<Ô/3"TH

==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/.git/objects/1a/76992187d46664eecd74fd7ee6f18385543d8c <==
x¥ŽMjÃ0F»Ö)f\F?–e¥º,ä
#iDMbO+ËÅÇo'öÝ=xð¾/É<O
Œ×O­2CÔÔsÀl-6'Kɞ÷ã˜=‡Á؈.«Oª¼4¾à0Øl£Éi¼)­'Jq{,eÌÁ'·IÑÖ>¤ÂÛR§¯áÈ¿ðúNé$réÎUºÌݟ¾J¢ëèûppÖ
p@¨Òãoãÿ—T™vΰÊÌ ß\£ì¼ª÷fTH

==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/.git/objects/1b/63dfd951bb6f265aa200228749da4da14bafc9 <==
x¥ÁjB1E]ç+f/-"L'QJ?d'LðIä½ú÷•.ú]]8‹Ã¹y´¶LpwsUO*ª"ä3zÇ^«NÕB!Ù=Í]VíB!Iö6×¢"œÚC¨!&B­	}áX³8ë<æu¬ð5ú6¥Ï¥ÃwWSÖ÷\òÞ>–&ùó:šžÁF>æàöhMþ͝úo'Ñç]×¥½?lÐÆ6o/óVJT‹

==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/.git/objects/24/7e930bef1ef5ea4be6e82cd661869bd3780ca9 <==
x¥ŽKj1½Ö)zoôÿ@"ø­VË3‹'ÂLûþ6^ä^=ªÅ£¹m«€
ñ$;3ô¨ƒ%´¾•žkÉ¥ßb·dk3Õûäsk5õ‡;ÄJ9TŒ'œÍ\\ʨ«qÑ=Á:®©÷FÞe™;\æ8‡¬~#|?ç‡þõñ±nHŸËÜøLL%Dm'³6Z+zÝ~;¤dÙçý¶À•IÖ9 ¨""T

==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/.git/objects/27/119bf44abeb538aef0e3df00b5c65c0a898edd <==
xµKNÃ0Egžu€üb"PQ[ÁØÁ³ýœZj"â8]?Ä\é®î'Lçs®L‰î¦"&"7É
å¢V$å7ôA"Øu''4Æ	Փm.Xh¬Q{kÕNÑ/Ñ&68-@Ð.Ù›þüàMStüZ$F"BHÙÛµ	UDPSp
.õ8vKþ\ˆ=Ð/l).eÂ3¿"Ï®ãڑj»ŒùÊ×ayæ1G*SmSyd`¬Ó¶
ìV€Mø9]éŸâ›W*1_pG¶y9<í7lJlÈu»ê¸øv]pÿŒ§LWºÛá2ãi7sË÷ïoü/TÚÕÙ|ç<€Ý

==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/.git/objects/2e/b5402ab691d8b2e8746aa61430725ce93bd287 <==
x¥MjÃ0…³Ö)foô/B…fWÈF£qlG®ª@ŽßÐæÙ<|ðø•e™h6­2C&Ÿƒ‰Cô1¡É6&©¤QNƒsÁ[ֈ+ß`V<¸1FÎZk•1Êg8ò-Ú8F
Ú/ÞÛT*|Þêü}gØñ9|!}"réOµô™ûß^áuʇÁZ¤"N*)ýù6~I縭ç<W\'è`^ðÌ?âÂRUÏ

==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/.git/objects/45/15101c935eae0488519873e4c3a329359a16c9 <==
x¥Qj!"óì)|ÔU…RB¡^Ꮞdi6n­=~–¤7ÃÀÀðMªó<ui\ÜõH²#{Š¤c
P›;ǁJ¦<úў³šÅÂ
·.S¦KƜcdïˆt•ÈE™ÌÈJ‡h¡¯ýR›ü¼µég…|Ã3Oœ>jý¾Z2†ÿþp­‰¯ïRû
Åmå^i¥Dzðv¼¾$Ö%s‡Ä߂6Íۙ_q¯\TH

==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/.git/objects/56/3887ba4f45c6fbbd9c48c1c972d991dda2ddda <==
xµ1nÄ ESs
úd)ŠÒì	r'1^
ãÍïùã$gH÷ô‹ÿôò¾mmhoñe³N™Ìzœ}ä˜#ØR¼`¡®H=H¸Í9/Pƒ·ÎZð"ÄLג,rÂ@¥:TtŽû.úÖ¥}¬ßø>¸œ²Óf²šc5΄d\ŠSç1½=Í%j‡)­°ìcªò®"$‡—F¿Z°Vå߈Áÿt¯>Éh}ÕÂù':ß©¯|¨ombí

==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/.git/objects/6c/7a73f40339b98c4d80b650484ddf97c62f922f <==
x¥ŽAŠ1E]絕Tº"t@d@<'(+l0‰t—÷Ÿf^ÀÕç½Åãs¯uVpÁítÄ$\'ss""¥0†\¦ÈäSä|·Aòd͋i
¹H1–$¼›†qCt	'Šö[ªðÀ(†Þúè\z[•šÎ
®MN,ÛüòG¯‡¹½Ê0Ä4ÚèB€‹Öþ¿«òuȼ_ nÂ:÷~ô¬}Uó–UÌ

==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/.git/objects/7a/9a57b758075a44d57cb1f3d4271e45819bc106 <==
x­ŽMjÃ0F³Ö)f_F²õ3Bhé2+Œ5ãÄ$–'­Þ¿¦›^ «ރǗë<O
\»¶¨'ϝ'³ŒÈÔ+â†úHid²ãè1H"óâEKê'Dë77¸aì¢ø¡w$J^ë°Û¼öÞðO»×¾jY—6ø.Êp̺Íù¯ûçÏZûëRϚùyBB›9ø@‹hòßí¦ošµÎ
í>•Ûj~îËUù

==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/.git/objects/7c/5d2b681c4656aeb4d02288c9eae4fa4f0c4060 <==
x¥OINÃ@äìWÌ-d3›gA'.V~ÐÓӓX8ž0±y?Ë8"TR-݅ù|î'¦Œ¸™
Ó)p'P"ÎIëQomD	UhEKtмº@¡qbÚi¥'·¼ô¨•qÖr@zIŸÀÙ?¿ÔÑs…¦
'''''M(Ij²*Yi´Ž\ótʅíÆÒÌÄ臬÷€Ï9¿×]Éu¤úWo†Œ0<2aœXþWJ³[.9¯ð{ßDÿoªöTŽÄBOlõº{Ú®XNìØOë§94˱ûzú¤»
ÌW6y¼6õ¶{;Ô\¨4‹³úÊsE

==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/.git/objects/8d/0ac9f52cb55400d72645531ed7027c7e238e6e <==
x¥A
Â0E]çÙKe&i"DDp)x…i2Á`k4¦àñ-ê
Ü=þ‡Çÿ>OSªR\ÕÂ,­&g-#F@kŒi	d
^å®%Û·ŝ
ߪDÎ10A«]ì"VÑS?À':ì"|¯Íõ'‹<ÞJzÌ,·ü…ý‰ü!çks.¹	Üüú͘=;‰ÆXg•ë´\ÿÙ[ù"àםKš–O9åbâ ÞfÙSô

==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/.git/objects/a5/86fd7d9968169641e1297cd40950fe337b8ff4 <==
xµKn!³æì#FÐ|¤(ò&é‡Åv›ñùc%gÈîmªJoûÞ§†bߦ0kr8ÛµDOvC [+g(ô bCOÐÔ­
/°º¶â²£)´ÀÑdžÙÆxõ"ªçü¢¿é÷"õÿÓ)£îæ&Wó¸gB2e9x.çџæ•éCXÆ\6ùÔ.¥"Îçô»kÕú{aò¿ÈUmC¦®DLêŒq\J

==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/.git/objects/a6/4a8fb63b7c037c13661c96c0346e5faf5388c8 <==
x­Wmoã6Þgý
°ëÖÄoq»M{
Ð˵Y[t»Om+‰Yò$¹iúëGÙé[Òå|ÀAbI|DŠ|HÑ©P)âÄÿéfÁ
Å7ìŸCzË´áJR¿›$9ý€stÂï
ý0< 'PBÆíúˆðpg¬ærn>†¾ûҘŝáìíL©yÁ>"‰È͂Q«ÊŽ`÷LP¨¸à ×tÆs»rÙÅÉZÌص`›…ã"/+6cšÉŒuΔ.ÀvScÉ!T–åÔ 5ânVÉ̺#|`Â6æôP'
|ŸrË
CgZ4ö»?½âÏšÍŽê>žýµîÇ]r
R0ÍéÏÁæü)O·—Â#š§¢ì¾³QÈ
ÐèŽ]\·ä&«—~œ§æ"u±¿+­Þ9iøæœÁ–çÈ;üÚG5':F߂7Š™DjnEw?òû©ñ7h‰|êtXQÚ5…<×Ì`ªHz:šL2%g^÷ÞqšWBÀñù$è"-—Ær[ÕlD äkèØ3ÜlK¾»=Ïræ#hréû­µAsÐ+'ÓéMl£¶-'–çʲm±wͱñŽµ'ÜœO®ƒa+«´2kã@°9˜Ó³«éÅu·ÂºãŒG÷.øèS´)™Uúûq†Ï•#kŒQr4þry™´´³Q‰IŽwYð®3¹1y#ït^NVœQY)b—¼Ž¹Žu©²ê
¤?J4ƒg"ßâåÿn¾Ãåd,UjÙ± ^lØ{¡|©JfWÖd‹õ©ûÚô}0'ó7°väÁ,s±<aH:æ[Ò¦¶ñD€^²O×ÃhϹr–¡39`äk	Åw8áL€"9ȱÿM'8ϔÞXå/ž';µâ]–Ô'y½¢É>_»•5ȯg˜lít݋<õΕ^±%賫k¿¥6ÙÏj©"šs–Ü´ÌT0¥Pf¶+u•a'?x˜sÁädzuôöÄù…¿Fa&B­ó³ÏÇÁN}|7
˜¨_à±ÒKÎV<{¶ó熻È}Þ¶XUzÀõÔoé¥J#À»PZssì#{Zé¬êHf×í®W}§L°<Ù·ë‹kK­æŠÂû«r5›]Ã=!1üP–h÷B'ý ÆtĬ‹
ç7sª¾€¡"Þ-lø°Ý퀥тw‹LO?û;¤Ù¹ 
'_Uõ+¶ÀȸœöÊ$ö½Ìúê'Àº&œK–wžÛк;Å~t€
u@74±¸GI¯×§Ù=Y¬þ‡ÄzìhZqleñxÚ´"a×K3UIké #wGàä!͎ÈGÚéÐ$ÆóýéžÂ^â"?ܓO~wC?!ú!
Éoî!îG19ªqƒ(ò	fB·dš«ü·>qJ»v]²z¦´UÎYۂfª÷qNw­êrik©8!øÂÐ,cNòªܵëÍÃ0!u)«‡½Aì"YÓÜc1~B…!á³Z F}ŸàÞNjjPOèÍFŠlîÍz¢Q'­F¥÷1ÁÛ³ë˜f$8VÚFº%¤ÔŠTlô"²Ò|¶®—"¨Gþ­°cªG>1K¾ÁÅØ+ µ²åÓJ…¯'îý¨÷? fð ËlW09·‹
¢žAÕ3þð4³1Ê'Ï^b´oÕô¦µ".ðå©ôú!Yñüy˕~ö}ýß¾4£+÷%t³9 ÿå¢ä

==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/.git/objects/b1/68150c3d2b2120b2ba6c7f23df5a7c7f6ffc3f <==
xV]oâ8ÝçþŠû¶/ú1Pi¤¦´³C§hÐi´rCÜ&vÖv`(êßc'Ójv7-q®ï=÷øØQ¦"êt;Áo'W–Ç©æ…Òv3õûïNˆXiS¥é¹'7Rê̽¦Ö—­ÖjµjÚ"n*½háÿ,Qq™siÍ,.µÆÙ'k#"4­"™»F<[ž7ÛífÐĈ‡ÒXaK‹0¿'fÒ°Ø¿Ž´Š¹1B.hÄõ\éœÉ˜S_•2™Ÿ+iSr?òH—L¯ýðš3Ÿw'h/'/''WFÍíŠi¾>K8/f'0+ff ÓžŸgÁyg¯hòpÇu<]ûxb2Çύ(,OKú̞VLŠ7âîÖʦ'þäI©YÂވêƒ2ÀY!éVò·¢Â'fRºg 1ãÛ´÷f¨ä_ß\_Òí|ÎÁè'gkšrÐ
Bû
Š­¿Tʄkz¥*úÊÙ
ŒÊ˜oÈ=†yÙg¾Zñ^8ö<ñ»,¹n¸(£L˜«àAr߸T‰ò8µD¶8#YaRennÐkŸú¨D‰-ªhÍóN·Ýzö@ͺ>ÔiôǃµœX
Ô
¯Ô7¦:•ìɄI%×¹*½@Ngﻝ³ó³‹×¦9OèZ•ìñ±n<Øý©è¤—œÆ*ÿëw&}–-+
Ž[7Ýí–ÑÝèãk"³B¿Nøé$|t3htN›Ë‹ÃtMÄÿaz;ÕïÇ=»&ýK«["Ê[C§ŒgÁÙÓèá-Àñ°Iõw¿|M›Ózx¾ÐHCžØ40'o=㍯J'4@Cté}ÅøÙG¾3¸Ò4U93tפ¯ÌÀŒ¹'Ä)õËµŸ'Ë<'Ž±ê¸OÓ ÛóÃ;#ºcòЇ¼`;ApæèÀi·¥ZÀÙ¬'­{‰'ÝîaýcGª¸£ê»ó
ºS'Ù"IšÐïÈjqÌËh_.)$³ŒE0P™ó\Õ^yDÄh›
=HXüÛ®ßÑ
/˜¶ÎÜIÍ!ï¼(AMbÁ'ø1Óq£Ý
Ýî3a¹(õƒµO€Åvq^EšØ"a6a²f½Þ!¡-3rŽjôc¿	c'ËÚU»à'k–‰gT
HTê	S…9ÂDL"/2îÊñÆf‡%ø¤E"Â0k·MÓ¯xDÓp0ý©^¯êðɸqÆ7¾¿¦ŒraÚºW+ì›êÿƒ-aóîËQa[§v©ÝZ<³HdèÇk	íºå:ôå;¦%>îQ•ZÂG°Öƒ7zŸŽU%*€F/jØÔfZõã3+›º~ü¸¸ŸÜڄڦ¥¦*ÈCí,­ڄÈaý쎞	×Â5§.ÆŠ	kFaQd"®ºR4ñ¦JU¦^£ÝN?Ñ·RcWÔë±$Ñî(sO3Y	ûÌuÜ:èÇáTGàvð¾þäÌÿ¨m£É—CNF!¶üÀ96ècÙ;¼ÆbgFàŒªÐÖ!`t¶Ôœ†Î2œüþFD•kìoƒ^åWPh¼YpÝ~÷‡êçïX~Õ½û˜;âªYÍXå-Íݙ½ä
­"l:wηœ*ç¸[aª»ù… ô"։ã'©Äø6ü'&ÖLvZUì.SñÓ!ZÛچûö‹¬þd¸iŇsvð=ý‡+L«Á_@ó$Ç=G©à{ø5 Wý?¶_ut

==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/.git/objects/d0/ead236578f52bb040b7c0bb2957f37ac1cfffb <==
x¥ËJÄ0…]÷)²›…tšûeFq%¾ÁŸäÏ40MKšúüVA_ÀՁÃw8až¦ÜˆPî®UDÂCtQJ'hŒQ ×%çÖ8‡Àµ¨±ÝK#4¡g\&/*£8¤Á*
\ZÉA‹¤û;‰Ú8®'S'ÒݬLòÆ%N•ORÂʶ6Ŝç²6(-òRÈCÀ=žÂ^û<A8Žó""im´ÒÎZrO¥]ø¹×ðߢî
뉯PÂHär s"ckËz†knãæûÞð
·ŒŸ8œa[áö}àØ?_Þ?ú,X»//ÐsT

==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/.git/objects/d6/18e3cc6fae38c4f6ef75600de1ecc476419599 <==
xµKNÄ0DYçÞÍyÆwü'bÒC˜v;câ‡ó1âìžT¥§*Z—¥ve>uaVP²‹Á@F.6»ݘ!@ÑÂa¤)G3ܓpëŠÁD2c¤"	' BÓá²fô˜K âBš|þëƒwqDÞ²õ)wø›ìAÈè£
CÚûuõÞ¤~í¬^øoœwYÓ¢ï2ëmÖ 5ºsã~Þ[ýÖÇ®ºé\3ËÚÏE^8ÐMÆFõlÀ˜~?wþûðÁ2³^ÖκK¢[m³ú"ÔèªNÂe»<Âí²Jk»,©¶Óðóûz.

==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/.git/objects/d8/3ed702e3c28b79b1f03b17972a7e884cb2c959 <==
xµMjÅ E;v΋ÁÏh¢ð(…Ò…øs}Mvý}´kèìrçpc;Ž2ø*éit€ÇÕY4cuFÜ Õ@\'€Úã*]Îìôupom€
2jë¼rF*c\TÁ[íö"='6'˜Ÿã£uþ^{ùšà7üW¤Ù›?ÄÙïâºZ½-c™µ|‹G§\"•"Þƒû§m·»#¥ˆ?K''Åßÿcgoí8?1Pq]|žÉ$ö£ta¬

==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/.git/objects/da/54e73a09bcb895865fdea89efa0b6f53c59447 <==
x­WmoÛ6Þgþ
°v‹-J–,+XÄI"!uS/	²õSp'h›0Ej$Çùõ;ÑNšÚAª5[<òár©s:²ÑO×a)~Ç"¿æÿÐn¬ÐŠ²~–•ô
ÊèDÜq±(zKŽ¡†B¸õ!­àþÖ:#Ôܾ‹Xû9 °‹[+øגڈŠ¿S\3 ×N®{'ßqI¡¹R€Yә¼ÝU¨>
ý2ë֒o'ŽŽ?ö.ùŒ®
Þ;Õ¦×Ï­#—¤Ô8^R‹ÖÈÛY£
×á
—ncNüuҐ1*¯,]фõ z%ž4Û=ÕC<ûsÝ÷É	8ÈÁnÎH·çÏE¾;Ò2—uÿ…©Á!…¢ƒîØÇŸ¥°…ŸúqžšË¼ýmíÌÞI£¯ÎîøxŽy²?÷'ÏŸÐÇè[ðb®05w¢û:òûSã0
ó©×ãUíÖÊÒp‹¥¢èÉx2=,´šÜGyÙH	Gç"pHv@BY'\㳁P®¡çÜ
»»òÅíEQòàA"OŒuBxƒæ`V §Óë(ÜEíZ¤œ(µã»Ë^4ÇA682Z	{>¹
GP¼1Ú®m0Éç`ON/§WaÒ	Ûg̺w!ÆïìH«¢1ߏ³b^éqØc¬V㳏Ÿ>eíܨĢŽÎö³à™3gPð\ëeρît˜Z×2›ÆÙb±>a7aÚ
&Kñ¬[¬0©[×sŒ1gg£äm<–`–üýÕhðŠ%/@•°àÓr­ ú'œJP0uƺŤ68Ó%Çv/Êì›Ôƶ~†Ù«èg±üÒ¼¾(ê¢6·Ÿ0Óì5·íir¶õù먛3mþÒòqjšÅ¯Ä苲;YæÁ¹6+¾szyź¬nsïƒ^j©çÕÁR؎¥¶–ÚoFÎ7ãÆr%î,Âpr<½¼	»ÒjŒøDêuyúá(Ük˜/Šà#<4f)øJ£nQØV×f±9ïÚ=­®ƒfÊ:ºAëÚJ.´1ž"¯åUޘ¢é)îÖÝî£6e§\ò²k¶=7PUÁßMÛÄùÕ(z%ñ¬¸\
K´{¡@E,L°a`_‡´[ÕC­'È‡Ä¨Ûu!¬uÜà7Ól/iönL+ÈgÝüŠœ3®¤Ã˜r…D˜ÛBŸ}'lҖbÿŠ—½'^êé*Ô@Äâ"n)5݂Æ,JRZ,Ð…C^~@°{R$4or[¤›ö
¤Á´Ðrö€ŽXZª'Â
†'w´×C2ògûˆ;Èí#¿·#œéù‡4%¿µÉãuèiŠÅ¥Ð¯¹ºü¥D	iµöݺæ^2Œ	«æ¼Da#Š‡ÊLßé¾Pn³*"ø
±™ÑßeSKÑx?›FHZ<åòÄáÛWK÷ñ¾xD¥	3¿ Ìâ8%¸w«5yaü(@wnV¤Á-ô£(‰â+‰añã­PMåX/I°<±«oV'IJjáÊåV?©#fk?¥ù¯AåGŒØ¥ØâR4s«X>Î4øÂÒ¾1ùñ0Îpz›Å#¼Ø¿w}ÉÕÜ-¶/AÕ3qÿ(ÙÅȓ×Ã!ÉjÃVýª˜'Õ_§ü a#²åӖ+óä{ô-yƒïc†ÓUû3ºÝƾ%ÿºê©?

==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/.git/objects/ea/d7033f9bddc93fc8738bda487c6bc608ef4714 <==
x5N½NÃ@c¾§0j‹"(¨CTºv(•``èý|MŽ\î‹î.
UÅ»""u°Û²­+"OåÝÃý~ó‰ÀœðŠNZŸ'ú_'t²ì/•n=ŽLMù…ø ¤Fúvb'ôìρN–F
GWÏœ¤¤r"#'QR·9ö9´eDúžC"uþï«jòš°•×yé`;Ò
…	˜WÛÝu>ÝFÐþžÎâp¨­ùí}6Ãü&Nùlù'­7å*+Šây'ñA€Tý

==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/.git/objects/ec/cb2f264301026023f2525ca643706e764adf16 <==
x¥ŽK
1]ç½r##=ɤ"\¸OétññþŠzwª(çËåXA[3©E¢ñN}ÐΈ%F/d£k£Æ"ðÀ¦G3¨[(r­àɶŽB—Ì€H½a;è>E¢"œ}«G*<ë˜l®åx
,ä;V»ÀëœO;ä&Jóãósæp^BK¤‰Þ"jDş¿Uþ/©ýaSÈu"òP/'ŽOü

==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/abstract.tex <==
%Parallel programming represents a challenge to computer scientists as the number of possible behaviors is quite large. This number grows exponentially when the program employs a distributed database with a weak level of isolation as Causal Consistency (CC). Therefore, efficient techniques for verifying and testing are required. In this paper we present a complete, sound and optimal algorithm which employs dynamic partial order reduction (DPOR) techniques for exploring all possible histories a transactional concurrent program may have; the only one up to now designed for this purpose. Our algorithm can be used under several isolation levels such as Causal Consistency, Read Atomic or Read Committed with linear memory consumption in all cases. 
%Dynamic Partial Order Reduction for Checking Correctness Against Weak Isolation Levels

Modern applications, such as social networking systems and e-commerce platforms are centered around using large-scale databases for storing and retrieving data. Accesses to the database are typically enclosed in transactions that allow computations on shared data to be isolated from other concurrent computations and resilient to failures. Modern databases trade isolation for performance. The weaker the isolation level is, the more behaviors a database is allowed to exhibit and it is up to the developer to ensure that their application can tolerate those behaviors. 

In this work, we propose stateless model checking algorithms for studying correctness of such applications that rely on dynamic partial order reduction. These algorithms work for a number of widely-used weak isolation levels, including Read Committed, Causal Consistency, Snapshot Isolation and Serializability. We show that they are complete, sound and optimal, and run with polynomial memory consumption in all cases. We report on an implementation of these algorithms in the context of Java Pathfinder applied to a number of challenging applications drawn from the literature of distributed systems and databases.  

==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/acknowledgements.tex <==
%!TEX root = main.tex
\section*{Acknowledgements}

We thank anonymous reviewers for their feedback, and Ayal Zaks for shepherding our paper. This work was partially supported by the project AdeCoDS of the French National Research Agency. % ANR (France).
% supported by the Agence National de Recherche (ANR) grant for the project ``AdeCoDS''.



==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/algo-class.tex <==
%!TEX root = main.tex
\section{Swapping-Based Model Checking Algorithms}\label{sec:algs}

%\subsection{Definition}

%The above-mentioned classes are, notwithstanding, quite dense and contain lots of algorithms we are not interested in (as non-DPOR algorithms for example). In particular, our work focuses on the collection of algorithms defined by the schema \ref{algorithm:algo-class} for some functions $\genericNext, \genericEvaluate, \genericValidWrites, \genericCompute, \genericProtocol, \genericSwap$ to be defined. %Thanks to this approach we will show the existence of some sound and complete algorithms and easily prove some of their properties.

We define a class of stateless model checking algorithms for enumerating executions of a given transactional program, that we call \emph{swapping-based algorithms}. Section~\ref{sec:CC-algorithm} will describe a concrete instance that applies to isolation levels that are prefix-closed and causally extensible.


%{\parfillskip0pt\par}
%\noindent

These algorithms are defined by the recursive function \textsc{explore} listed in Algorithm~\ref{algorithm:algo-class}. The function \textsc{explore} receives as input a program $\prog$, an \emph{ordered history} $\hist_<$, which is a pair $(\hist,<)$ {\parfillskip0pt\par}

\begin{wrapfigure}{l}{0.45\textwidth}
\vspace{-6mm}
\begin{minipage}{0.45\textwidth}
\begin{algorithm}[H]
\caption{\textsc{explore} algorithm}
\begin{algorithmic}[1]
\Function{\textsc{explore}}{$\prog$, $\hist_<$, $\locals$}
\State $j, e, \gamma \gets  \genericNext(\prog, \hist_<, \locals)$

\State $\locals' \gets \locals[e\mapsto \gamma]$
\If{$e = \bot$ and $\genericEvaluate(h)$}
%			\If{$\genericEvaluate(\prog, h, \locals)$}
\State \textbf{output} $h$, $\locals'$
%			\EndIf
%\State $\textbf{\genericEvaluate}(h)$
%		\State \Return
\ElsIf{$\mathit{type}(e) = \iread$}

\ForAll{$t \in \genericValidWrites(h,e)$} 
\State $h'_< \gets h_< \oplus_j e \oplus \wro(t,e)$

\State $\textsc{explore}(\prog, h'_< , \locals')$
%\label{algorithm:algo-class:exploreRead}
\State $\textsc{exploreSwaps}(\prog, h'_< , \locals')$
\EndFor
\Else %If{$\genericEvaluate(h\bullet e)$}
\State $h'_< \gets h_< \oplus_j e$
\State $\textsc{explore}(\prog, h'_<,\locals')$
\State $\textsc{exploreSwaps}(\prog, h'_< , \locals')$
\label{algorithm:algo-class:exploreStd}
%		\Else
%			\State \Return
\EndIf
\EndFunction

\end{algorithmic}
\label{algorithm:algo-class}
%\caption{Generic method for exploring every possible history $h$ of a program $\mathcal{P}$ running under a database with $\mathcal{M}$ as isolation level.}
\end{algorithm}
\end{minipage}
%\vspace{-2mm}
\end{wrapfigure}

\noindent of a history and a total order $<$ on all the events in $\hist$, and a mapping $\locals$ that associates each event $e$ in $\hist$ with the valuation of local variables in the transaction of $e$ ($\trans{h}{e}$) just before executing $e$. 
For an ordered history $(\hist,<)$ with $\hist=\tup{T, \so, \wro}$, we assume that $<$ is consistent with $\po$, $\so$, and $\wro$, i.e., $e_1 < e_2$ if $(\trans{h}{e_1},\trans{h}{e_2})\in (\so\cup\wro)^+$ or $(e_1,e_2)\in\po$. Initially, the ordered history and the mapping $\locals$ are empty. 

%{\parfillskip0pt\par}
%\noindent




The function \textsc{explore} starts by calling $\genericNext$ to obtain an event representing the next database access in some pending transaction of $\prog$, or a  $\ebegin$/$\ecommit$/$\eabort$ event for starting or ending a transaction. This event is associated to some session $j$. For example, a typical implementation of $\genericNext$ would choose one of the pending transactions (in some session $j$), execute all local instructions until the next database instruction in that transaction (applying the transition rules \textsc{if-true}, \textsc{if-false}, and \textsc{local}\appendixver{from Figure~\ref{fig:op:sem:baseline} in Appendix~\ref{app:rules}}) and return the event $e$ corresponding to that database instruction and the current local state $\gamma$. $\genericNext$ may also return $\bot$ if the program finished.
%or if the history $\hist$ is not consistent with the intended isolation level. 
If $\genericNext$ returns $\bot$, then the function $\genericEvaluate$ can be used to filter executions that satisfy the intended isolation level before outputting the current history and local states \nver{(the use of $\genericEvaluate$ will become relevant in Section~\ref{sec:ser})}.



%the history satisfies the consistency requirements
%The function $\genericEvaluate$ is used to select the cases in which the program finished and the history satisfies all the consistency requirements before outputting the current history (and local states).
%Algorithm \ref{algorithm:algo-class} explores systematically the space of histories, selecting a new event $e$ to be added to some history $h$ if possible, thanks to the function $\genericNext$ called \textit{next}. If it wasn't possible, it is due to $h$ being either a total execution or an undesirable one; both behaviors discriminated via \textit{evaluating} $h$ with the $\genericEvaluate$ function. 

Otherwise, the event $e$ is added to the ordered history $h_<$. If $e$ is a read event, then $\genericValidWrites$ computes a set of write events $w$ in the current history that are valid for $e$, i.e., adding the event $e$ along with the $\wro$ dependency $(w,e)$ leads to a history that still satisfies the intended isolation level.
% along with a $\wro$ dependency selected via $\genericValidWrites$ if it is a read. linking a \textit{valid} $\iwrite$ event with the new $\iread$ event (valid means satisfying consistency w.r.t. the intended isolation level). 
%
Concerning notations, let $\hist$ be a history where $\so$ is represented as a function $\so:\mathsf{SessId}\rightharpoonup \mathsf{Tlogs}^*$ (as in \S~\ref{ssec:semantics}). 
%that contains a representation of $\so$ as above. 
%We use $\hist\oplus_j \tup{\tr,E,\po_t}$ to denote a history where $\tup{\tr,E,\po_t}$ is appended to $\so(j)$. 
For event $e$, $\hist\oplus_j e$ is the history obtained from $\hist$ by adding $e$ to the last transaction in $\so(j)$ as the last event in $\po$ (i.e.,  if $\so(j)=\sigma; \tup{t,E,\po_t}$, then the session order $\so'$ of $\hist\oplus_j e$ is defined by $\so'(k)=\so(k)$ for all $k\neq j$ and $\so(j) =\sigma; \tup{t,E\cup\{e\},\po_t\cup \{(e',e): e'\in E\}}$). This is extended to ordered histories: $(\hist,<) \oplus_j e$ is defined as $(\hist \oplus_j e, < \cdot\ e)$ where $<\cdot\ e$ means that $e$ is added as the last element of $<$. Also, $\hist \oplus_j (e,\ebegin)$ is a history where $\tup{\tr,\{\tup{e,\ebegin}\},\emptyset}$ with $\tr$ a fresh id is appended to $\so(j)$, and 
$\hist\oplus\wro(t,e)$ is defined by adding $(t,e)$ to the write-read of $\hist$.
%Moreover, we simplify the notation and write $h\oplus\wro(w,e)$ for $w$ a write event and $e$ a read event instead of $h\oplus\wro(\trans{h}{w},e)$.

\begin{wrapfigure}{lt}{0.47\textwidth}
\vspace{-8mm}
\begin{minipage}{0.47\textwidth}
\begin{algorithm}[H]
\caption{\textsc{exploreSwaps} }
\begin{algorithmic}[1]
\Function{\textsc{exploreSwaps}}{$\prog$, $\hist_<$, $\locals$}
%		\State $e \gets \laste(\hist_<)$
\State $l \gets \genericCompute(h_<)$		
\ForAll{$(\alpha, \beta) \in l$}
\If{$\genericProtocol(h_<, \alpha, \beta,\locals)$}
\State $\textsc{explore}(\prog,\genericSwap(h_<, \alpha, \beta, \locals))$	

\EndIf
\EndFor
\EndFunction

\end{algorithmic}
\label{algorithm:explore-swaps}
%\caption{Generic method for exploring every possible history $h$ of a program $\mathcal{P}$ running under a database with $\mathcal{M}$ as isolation level.}
\end{algorithm}
\end{minipage}
\vspace{-4mm}
\end{wrapfigure}

%TODO GIVE AN EXAMPLE OF SUCCESSIVE EXTENSIONS OF A HISTORY USING NEXT TO GET NEXT EVENTS. ADD SOME LOCAL INSTRUCTIONS AS WELL TO EXPLAIN LOCAL STATES.
Once an event is added to the current history, the algorithm may explore other histories obtained by re-ordering events in the current one. Such re-orderings are required for completeness. New read events can only read from writes executed in the past which limits the set of explored histories to the scheduling imposed by $\genericNext$. Without re-orderings, writes scheduled later by $\genericNext$ cannot be read by read events executed in the past, although this may be permitted by the isolation level. 
%TODO GIVE AN EXAMPLE (PROGRAM, CURRENT HISTORY, NEXT RETURNING A WRITE, THERE EXISTS A HISTORY WHERE THE WRITE CAN BE READ BY A READ IN THE CURRENT HISTORY).

The function $\textsc{exploreSwaps}$ calls $\genericCompute$ to compute pairs of sequences of events $\alpha, \beta$ that should be re-ordered; $\alpha$ and $\beta$ are \emph{contiguous and disjoint} subsequences of the total order $<$, and $\alpha$ should end before $\beta$ (since $\beta$ will be re-ordered before $\alpha$). Typically, $\alpha$ would contain a read event $r$ and $\beta$ a write event $w$ such that re-ordering the two enables $r$ to read from $w$. Ensuring soundness and avoiding redundancy, i.e., exploring the same history multiple times, may require restricting the application of such re-orderings. This is modeled by the Boolean condition called $\genericProtocol$. If this condition holds, the new explored histories are computed by the function $\genericSwap$. This function returns local states as well, which are necessary for continuing the exploration. 
%A typical implementation of this function would return ordered histories where the events in $\beta$ and their $\so$ or $\wro$ dependencies 
%%($(\so\cup\wro)^*$ predecessors) 
%are ordered before the events in $\alpha$. 
We assume that $\genericSwap(\hist_<, \alpha, \beta, \locals)$ returns pairs $(\hist'_{<'},\locals')$ such that 
\begin{enumerate}
	\item $\hist'$ contains \nver{at least} the events in $\alpha$ and $\beta$,
	\item $\hist'$ without the events in $\alpha$ is a prefix of $\hist$, and
	\item if a read $r$ in $\alpha$ reads from different writes in $\hist$ and $\hist'$ (the $\wro$ relations of $\hist$ and $\hist'$ associate different transactions to $r$),
	%transactions associated with $r$ by the   are different) 
	 then $r$ is the last event in its transaction (w.r.t. $\po$).
\end{enumerate}

%"the change of a read-from dependency is restricted to the last read in a transaction (third condition) because changing the value returned by a read may disable later events in the same transaction." Aren't the possibilities for the previous reads missed? Why is explore swaps complete?
%No, other possibilities for previous reads will be considered by other swaps. The supplemental text includes a proof of completeness, but we will try to include more intuition in the main text. 
The first condition makes the re-ordering ``meaningful'' while the last two conditions ensure that the history $\hist'$ is feasible by construction, i.e., it can be obtained using the operational semantics defined in Section~\ref{ssec:semantics}. Feasibility of $\hist'$ is ensured by keeping prefixes of transaction logs from $\hist$ and all their $\wro$ dependencies except possibly for read events in $\alpha$ (second condition). In particular, for events in $\beta$, it implies that $\hist'$ contains all their $(\po\cup\so\cup\wro)^*$ predecessors. Also, the change of a read-from dependency is restricted to the last read in a transaction (third condition) because changing the value returned by a read may disable later events in the same transaction\footnote{\nver{Different $\wro$ dependencies for previous reads can be explored  in other steps of the algorithm.}}.
% \nver{and (2) changing a read-from dependency from a previous event can be covered by a different pair of subsequences}.
%Also, the second condition restricts the possible changes of the $\wro$ relation to events in $\alpha$ since for the rest $\hist'$ must be a prefix of $\hist$ and therefore keep all the $\wro$ dependencies. For events in $\beta$, it implies that $\hist'$ contains all their $(\po\cup\so\cup\wro)^*$ predecessors. The last condition is required since changing the value returned by a read access may disable later events in the same transaction. % (they need to be re-executed).

%\begin{itemize}
%	\item $\hist'$ contains a subset of the events/transactions in $\hist$ that includes all the events in $(\hist,<)$ up to and including all events in $\alpha$ w.r.t. $<$, all the events in $\beta$, and all the events which are $(\so\cup\wro)^*$ predecessors of events in $\beta$,
%	\item $<'$ coincides with $<$ until the last event before $\alpha$, and it orders all events in $\beta$ before events in $\alpha$,
%	\item the $\so$ relation of $\hist'$ equals the $\so$ relation of $\hist$ projected on transactions in $\hist'$,
%	\item the $\wro$ relation of $\hist'$ equals the $\wro$ relation of $\hist$ projected on events/transactions in $\hist'$ except its last event w.r.t. $<'$,
%	\item $\locals'$ is the projection of $\locals$ on events in $\hist'$.
%\end{itemize}

%TODO GIVE AN EXAMPLE. A HISTORY, $\alpha$ and $\beta$ such that $\beta$ has some $(\so\cup\wro)^*$ predecessors. EXPLAIN WHY ONLY THE WR OF THE LAST EVENT CAN CHANGE (OTHERWISE, WE DON'T KNOW IF EVENTS REMAIN ENABLED, LOCAL STATES MAY CHANGE.

%some collection of events $\alpha, \beta$ that may needed to be reordered. Every events' rescheduling possibly lead to a different execution, so for controlling which reorderings we are shall explore, we enforce a \textit{reordering protocol} (function $\genericProtocol$). In the affirmative case, the new histories would be generated via $\genericSwap$, \textit{swapping} $\beta$ and all their dependencies before $\alpha$. However, the reader shall take into account that this high-level description of algorithm \ref{algorithm:algo-class} may not be satisfied for some $\textsc{explore}$'s instance.
%may not be satisfied for some $\textsc{explore}$'s instances.

%determines so, we will also explore the history generated via $\genericSwap$; where $\alpha$ and $\beta$ have different relative order. It is assumed that \ref{algorithm:algo-class} maintains a total order between events in the history that doesn't contradict $\so$. Finally, let's take into account that this high-level description of the algorithm may not be satisfied for some $\textsc{explore}$'s instances. %\textcolor{red}{Here I wanted to guide the reader of what does this algorithm mean; but remarking that of course, if you add a weird function, then all what I said is a lie (for example if the swap history does not swap at all).}

%TODO WE ASSUME THAT THE NEXT FUNCTION IS INDEPENDENT OF THE FUTURE. IT IS A NON-DETERMINISTIC FUNCTION, BUT ITS SET OF POSSIBLE RESULTS IS THE SAME IF THE PROGRAM HAS MORE/DIFFERENT THINGS AFTER THE NEXT DATABASE ACCESS.

%\begin{definition}
%The \callout{swapping-based algorithm's class} for the memory model $\mathcal{M}$, $\mathcal{S}_{\mathcal{M}}$, is the minimal collection containing all algorithms $A$ that can be described as algorithm \ref{algorithm:algo-class}'s instances: $ \textsc{explore}(\genericNext, \genericEvaluate, \genericValidWrites, \genericCompute, \genericProtocol, \genericSwap)$; where $\genericNext, \genericEvaluate , \genericValidWrites, \genericCompute, \genericProtocol, \genericSwap$ are functions defined as follows: 
%\begin{itemize}
%	\item $\genericNext: \mathcal{H}_\mathcal{P} \to \mathcal{E}_\mathcal{P}$, where for every $h \in \mathcal{H}_{\mathcal{P}}$, $\genericNext(h) \not\in h$ and for every event $e$ s.t. $e \ [\so] \ \genericNext(h)$, $e \in h$, %\textcolor{red}{redundant with weakly optimal; it may be helpful to the reader}
%	\item $\genericEvaluate: \mathcal{H}_\mathcal{P} \to \{0, 1\}$, %which determines if an execution is total or not,
%	\item $\genericValidWrites: \mathcal{H}_\mathcal{P} \times \mathcal{E}_\mathcal{P} \to \mathcal{P}(\mathcal{E}_\mathcal{P})$, %\textcolor{red}{this is for determine when computing a total inconsistent history shall be taken into account}
%	\item $\genericCompute: \mathcal{H}^<_\mathcal{P} \to \mathcal{E}_\mathcal{P}^* \times \mathcal{E}_\mathcal{P}^*$, where for every history $h$, $\genericCompute(h) = (\alpha, \beta)$, $\alpha \cap \beta = \emptyset$ and for every $(e, e') \in \alpha \times \beta$, $e <_h e'$.
%	\item $\genericProtocol: \mathcal{H}^<_\mathcal{P} \times \mathcal{E}_\mathcal{P}^* \times \mathcal{E}_\mathcal{P}^* \to \{0,1\}$, %\textcolor{red}{shall we impose the protocol to only be true in only one history for each class? not needed though...}
%	\item $\genericSwap: \mathcal{H}^<_\mathcal{P} \times \mathcal{E}_\mathcal{P}^* \times \mathcal{E}_\mathcal{P}^* \to \mathcal{H}^<_\mathcal{P}$, where for every $h, \alpha, \beta$, we have $\genericSwap(h \bullet e, \alpha, \beta) = h'$, $\alpha, \beta \in h'$, for every $(e, e') \in \alpha \times \beta \implies e >_{h'} e'$ and there exists some $(e, e') \in (\alpha, \beta)$ s.t. $\tr(e') \ [\wro] \ \tr(e)$.
%\end{itemize}
%\end{definition}

A concrete implementation of \textsc{explore} is called:
\vspace{-1mm}
\begin{itemize}
	\item \emph{$I$-sound} if it outputs only histories in $\histOf[I]{\prog}$ for every program $\prog$,
	\item \emph{$I$-complete} if it outputs every history in $\histOf[I]{\prog}$ for every program $\prog$,
	\item \emph{optimal} if it does not output the same history twice,
	\item \emph{strongly optimal} if it is optimal and never engages in fruitless explorations, i.e., \textsc{explore} is never called (recursively) on a history $\hist$ that does not satisfy $I$, and every call to \textsc{explore} results in an output or another recursive call to \textsc{explore}.
\vspace{-1mm}
\end{itemize}


%\subsection{Other}
%
%\begin{definition}
%Given an algorithm $A$ and a model $\mathcal{M}$, we say:
%\begin{itemize}
%	%\item $A$ is \callout{blind} if for every program $\mathcal{P}$ and every history $h$, $A$ cannot determine the evaluation of any instruction $i$ not yet executed (i.e. $i \in \mathcal{P} \setminus h$),
%	%\item $A$ is \callout{weakly $\mathcal{M}$-sound} if for every program $\mathcal{P}$, every total history $h$ computed by $A$ is $\mathcal{M}$-consistent,
%	%\item $A$ is \callout{$\mathcal{M}$-sound} if for every program $\mathcal{P}$, every history $h$, partial or not, computed by $A$ is $\mathcal{M}$-consistent,
%	\item $A$ is \callout{$\mathcal{M}$-sound} if for every program $\mathcal{P}$, every total history $h$ computed by $A$ is $\mathcal{M}$-consistent,
%	\item $A$ is \callout{complete} if for every program $\mathcal{P}$ it computes every possible execution,
%	\item $A$ is \callout{weakly optimal} if for every program $\mathcal{P}$ it computes every execution at most once,
%	\item $A$ is \callout{optimal} if for every program $\mathcal{P}$ it is weakly optimal and it does not compute blocking executions (i.e. partial histories that cannot be completed), 
%\end{itemize}
%\end{definition}
%
%
%\begin{definition}
%The algorithm's class $\mathcal{O}^n_{\mathcal{M}}$ is defined as the minimal collection containing all algorithms $\mathcal{M}$-sound, complete and optimal that employ polynomial memory and allows at most $n$ pending transactions. %We also denote $\mathcal{O}_{\mathcal{M}} = \bigcup\limits_{n \in \mathbb{N}} \mathcal{O}^n_{\mathcal{M}}$.
%\end{definition}
%
%
%\begin{definition}
%The algorithm's class $\mathcal{W}^n_{\mathcal{M}}$ is defined as the minimal collection containing all algorithms $\mathcal{M}$-sound, complete and weakly optimal that employ polynomial memory and allows at most $n$ pending transactions. 
%\end{definition}
%
%\textcolor{red}{TODO: change this to not be a class...}
%
%%\textcolor{red}{We need the three classes for the following: RA/RC/CC/PRE algorithms belong to $O^1$, our PRE+SER/PRE+SI version is $W^1$, for SER we cannot obtaining it in $O^n$ for any $n$ nor in $L^1$ and in RA/RC/CC/PRE $O^1 = L^1$. Moreover, if we allow the subindex there, we can talk about future work allowing multiple pending transactions (it may be reasonable to prove that there is an algorithm for SER in $L^n$) and indicate Viktor's algorithm is not in $L^n$ for any $n$ as it employs exp memory. If we don't want to be that expressive, we can only talk about weakly optimal and then proof that under RA/RC/CC/PRE with our algorithms there is no blocking branches as an extra feature thanks to the models; but I thought it may be clearer to distribute it in this way.}
%
%
%TODO
%The swapping-based algorithms have been already studied in the literature as for example \textcolor{red}{cite Viktor's algorithm}, which belongs to $\mathcal{S}_{SC}$; where SC in this case is the axiomatic representation of sequential consistency memory model. \textcolor{red}{cite SC.}

==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/algorithm-main.tex <==
%!TEX root = main.tex
\section{Swapping-based model checking for Prefix-Closed and Causally-Extensible Isolation Levels}
\label{sec:CC-algorithm}

%The main goal in this section is describing a deterministic algorithm for transactional model-checking under a causally-closed model $\mathcal{M}$ that obtains all possible behaviors a program may have. We present during this section a swapping-based sound, complete and optimal algorithm employing polynomial memory. In particular, we will show that our algorithm has at most one pending transaction and why this is key to guarantee the rest of the properties. For the legibility of this document, we will postpone their proofs to section \ref{sec:proofs-algorithm}.

We define a concrete implementation of $\textsc{explore}$, denoted as $\textsc{explore-ce}$, that is $I$-sound, $I$-complete, and strongly optimal for any isolation level $I$ that is prefix-closed and causally-extensible. The isolation level $I$ is a parameter of $\textsc{explore-ce}$. The space complexity of $\textsc{explore-ce}$ is polynomial in the size of the program. An important invariant of this implementation is that it explores histories with \emph{at most one} pending transaction and this transaction is maximal in session order. This invariant is used to avoid fruitless explorations: since $I$ is assumed to be causally-extensible, there always exists an extension of the current history with one more event that continues to satisfy $I$. \nver{Moreover, this invariant is sufficient to guarantee completeness in the sense defined above of exploring all histories of ``full'' program executions (that end in a final configuration).}

Section~\ref{ssec:extensions} describes the implementations of $\genericNext$ and $\genericValidWrites$ used to extend a given execution, Section~\ref{subsection:SwappingHistories} describes the functions $\genericCompute$ and $\genericSwap$ used to compute re-ordered executions, and Section~\ref{ssec:optimality} describes the $\genericProtocol$ restriction on re-ordering. We assume that the function $\genericEvaluate$ is defined as simply $\genericEvaluate(\hist) ::= true$ (no filter before outputting). Section~\ref{ssec:corr} discusses correctness arguments\appendixver{ (see App.~\ref{sec:proofs-algorithm} for proofs)}.

\input{extending}

\input{swaps}

%\input{blocking-branches}

%\input{maximally-added}

\subsection{Correctness}\label{ssec:corr}

The following theorem states the correctness of the algorithm presented in this section:
\begin{restatable}{theorem}{algoCorrect}
\label{th:corr}
For any prefix-closed and causally extensible isolation level $I$, $\textsc{explore-ce}$ is $I$-sound, $I$-complete, strongly optimal, and polynomial space.
\end{restatable}

$I$-soundness is a consequence of the $\genericValidWrites$ and $\genericProtocol$ definitions which guarantee that all histories given to recursive calls are $I$-consistent, and of the $\genericSwap$ definition which ensures to only produce feasible histories (which can be obtained using the operational semantics defined in Section~\ref{ssec:semantics}). The fact that this algorithm never engages in fruitless explorations follows easily from causal-extensibility which ensures that any current history can be extended with any event returned by $\genericNext$. Polynomial space is also quite straightforward since the \textbf{for all} loops in Algorithm~\ref{algorithm:algo-class} have a linear number of iterations: the number of iterations of the loop in $\textsc{explore}$, resp., $\textsc{exploreSwaps}$, is bounded by the number of write, resp., read, events in the current history (which is smaller than the size of the program; recall that we assume bounded programs with no loops as usual in SMC algorithms). On the other hand, the proofs of $I$-completeness and optimality are quite complex. \oldver{For $I$-completeness, given a history $\hist\in \histOf[I]{\prog}$, we first show how to effectively compute the order $<$ associated to $\hist$ if $\textsc{explore}$ were to output this history. Then, we define an ``inverse'' of $\textsc{explore-sc}$ and an invariant on ordered histories reached by $\textsc{explore-sc}$, which enable constructing a chain of ordered histories going backwards from $(\hist,<)$ to the initial empty history. Then, we show that $\textsc{explore-sc}$ can proceed forwardly  in this chain and indeed output $\hist$.}


%In particular, we observe that if two transactions $t, t'$ have a $(\so \cup \wro)^*$ dependency, the history order in the algorithm orders them analogously. But if they are $(\so \cup \wro)^*$-incomparable, the algorithm prioritizes the one that is read by a smaller $\iread$ event according $\ora$. Combining both arguments recursively we obtain a \textit{canonical order} for a history, which is formally defined with the function presented below. 

\nver{$I$-completeness means that for any given program $\prog$, the algorithm outputs every history $h$ in $\histOf[I]{\prog}$. The proof of $I$-completeness defines a sequence of histories produced by the algorithm starting with an empty history and ending in $h$, for every such history $h$. 
% a collection of reachable histories that starts in the initial state and ends in $h$. The structure of the proof is as follows:
It consists of several steps:}
\begin{enumerate}
    \item \nver{Define a \emph{canonical} total order $<$ for every unordered partial history $h$, such that if the algorithm reaches $h_{<'}$, for some order $<'$, then $<$ and $<'$ coincide. This canonical order is useful in future proof steps as it allows to extend several definitions to arbitrary histories that are not necessarily reachable, such as $\genericProtocol$ or $\textsc{swapped}$.}
    \item \nver{Define the notion of \emph{$\ora$-respectfulness}, an invariant satisfied by every (partial) ordered history reached by the algorithm. Briefly, a history is $\ora$-respectful if it has only one pending transaction and for every two events $e, e'$ such that $e <_{\ora} e'$, either $e < e'$ or there is a swapped event $e''$ in between. 
%    We require of canonical order to proper define swapped events on arbitrary histories.
 } 
    \item \nver{Define a deterministic function $\prev$ which takes as input a partial history (not necessarily reachable), such that if $h$ is reachable, then $\prev(h)$ returns the history computed by the algorithm just before $h$ (i.e., the previous history in the call stack). Prove that if a history $h$ is $\ora$-respectful, then $\prev(h)$ is also $\ora$-respectful.}
    
    \item \nver{Deduce that if $h$ is $\ora$-respectful, then there is a finite collection of $\ora$-respectful histories $H_h = \{h_i\}_{i=0}^{n}$ such that $h_n = h$, $h_0 = \emptyset$, and $h_i = \prev(h_{i+1})$ for each $i$. The $\ora$-respectfulness invariant and the causal-extensibility of the isolation level are key to being able to construct such a collection. In particular, they are used to prove that $h_i$ has at most the same number of swapped events as $h_{i+1}$ and in case of equality, $h_i$ contain exactly one event less than $h_{i+1}$, which implies that the collection is indeed finite.}
    
    \item \nver{Prove that if $h$ is $\ora$-respectful and $\prev(h)$ is reachable, then $h$ is also reachable. Conclude by induction that every history in $H_h$ is reachable, as $h_0$ is the initial state and $h_i = \prev(h_{i+1})$.}
    %\item \nver{Constructing a finite collection of $\ora$-respectful histories $H_h = \{h_i\}_{i=0}^{n}$ such that $h_n = h$, $h_0 = \emptyset$ and $h_i = \prev(h_{i+1})$.}
\end{enumerate}

%As $h_0$ corresponds to the initial state, we can thus conclude that $h$ is reachable by induction on the histories in $H_h$: the base case, $h_0$, is always reachable while if $h_i$ is reachable, by the property (1) of $\prev$, $h_{i+1}$ is also reachable. 

%Then, we can prove by exploiting property (2) of $\prev$ that, for every $\ora$-respectful history $h$ there exists a finite collection of $\ora$-respectful histories $H_h = \{h_i\}_{i=0}^{n}$ such that $h_n = h$, $h_0 = \emptyset$ and $h_i = \prev(h_{i+1})$.

% Thirdly, we describe a function $\prev$ defined over the set of all partial histories that, if $h$ is reachable, $\prev(h)$ returns the previous history to $h$ computed by $\textsc{explore-ce}$. This function $\prev$ satisfies (1) the previous of an $\ora$-respectful history is also $\ora$-respectful and (2) if the previous of a history is reachable, then the history is reachable.

%\nver{ For showing $I$-completeness, we prove that for any given program $\prog$, it outputs every history $h$ in $\histOf[I]{\prog}$. For doing it so, we explicit show a collection of reachable histories that starts in the initial state and ends in $h$. However, algorithm \ref{algorithm:algo-class} works with ordered histories. Therefore, we first have to furnish $h$ with a total order called \textit{canonical order} that, if $(h, <)$ were reachable, it would coincide with its history order; so one can always work with histories instead of ordered histories. This order is based in two facts about our algorithm: (1) for every pair of transactions, if $(t, t') \in (\so \cup \wro)^*$ in $h$, then $t < t'$ and (2) if $t, t'$ are $(\so \cup \wro)^*$-incomparable, the algorithm prioritizes the one that is read by a smaller $\iread$ event according $\ora$. Secondly, we define the notion of \textit{$\ora$-respectfulness}, an invariant that every partial history reachable with $\textsc{explore-sc}$ satisfy. Briefly, a history is $\ora$-respectful if it has only one pending transaction and for every two events $e, e'$ such that $e <_{\ora} e'$, either $e < e'$ or there is a swapped event $e''$ in between. Thirdly, we describe a function $\prev$ defined over the set of all partial histories that, if $h$ is reachable, $\prev(h)$ returns the previous history to $h$ computed by $\textsc{explore-ce}$. This function $\prev$ satisfies (1) the previous of an $\ora$-respectful history is also $\ora$-respectful and (2) if the previous of a history is reachable, then the history is reachable. Then, we can prove by exploiting property (2) of $\prev$ that, for every $\ora$-respectful history $h$ there exists a finite collection of $\ora$-respectful histories $H_h = \{h_i\}_{i=0}^{n}$ such that $h_n = h$, $h_0 = \emptyset$ and $h_i = \prev(h_{i+1})$. As $h_0$ corresponds to the initial state, we can thus conclude that $h$ is reachable by induction on the histories in $H_h$: the base case, $h_0$, is always reachable while if $h_i$ is reachable, by the property (1) of $\prev$, $h_{i+1}$ is also reachable. }

%Finally, albeit some intuition about the optimality arguments was given in Section~\ref{ssec:optimality}\nver{, one can deduce the optimality from the arguments employed for $I$-completeness. If a history $h$ would have a computable path different, it would have a immediate predecessor $h'$ that is different than $\prev(h)$.}
%Finally, albeit some intuition about the optimality arguments was given in Section~\ref{ssec:optimality}
\nver{The proof of strong optimality relies on arguments employed for $I$-completeness. It can be shown that if the algorithm would reach a (partial) history $h$ twice, then for one of the two exploration branches, the history $h'$ computed just before $h$ would be different from $\prev(h)$, which contradicts the definition of $\prev(h)$.}

%\nver{On one hand, when no swaps are required for $\textsc{explore-ce}$ arrive to $h$ from $h'$, $\prev(h)$ coincide with $h'$ by definition of $\prev(h)$. On the other hand, if $h$ is obtained by swapping some read event with respect a transaction from $h'$ (potentially removing some other events in the process), we distinguish between two class of events in $h'$: the events that remain in $h$ and those which have been removed. The definition of $\prev$ function guarantees that $h'$ and $\prev(h)$ coincide on the events that are not deleted while the $\ora$-respectfulness of reachable histories and $\genericProtocol$'s definition allows us to conclude that they also coincide on the deleted events.}

%\nver{, one can deduce the optimality from the arguments employed for $I$-completeness. Given a history $h$, the definition of both its canonical order and $\prev(h)$ only depends on the relations $\ora, \so$ and $\wro$. Thus, exploiting both notions we can deduce that every predecessor of a reachable history $h$ coincides with $\prev(h)$. By induction on the collection $H_h$, we conclude $h$ has only one computable path.}

\nver{In terms of time complexity, the $\textsc{explore-ce}(I)$ algorithm achieves polynomial time between consecutive outputs for isolation
levels $I$ where checking $I$-consistency of a history is polynomial time, e.g., \RC, \RA, and \CC.} 
%This
%would not be true for EXPLORE(I0, I) where I is SI or SER (checking consistency in this case
%is known to be NP-complete).

%\nver{, one can deduce the optimality from the arguments employed for $I$-completeness. Simply, as both the canonical order and $\prev$ function's definition are agnostic of \textsc{explore-sc}'s procedure, every predecessor of a reachable history $h$ coincides with $\prev(h)$. By applying induction on the collection $H_h$, we conclude $h$ has only one computable path.}

%Reasoning by contradiction, if a reachable history $h$ with minimal number of events swapped would have two computable paths, it would have two predecessors $h_1$ and $h_2$; and without loss of generality, $h_1 = \prev(h)$. However, by defintion of $\prev$ we can conclude that actually $h_1 = h_2$.

%as well in property (2) of $\prev$. This property stablish an univoque correspondance between a reachable history and its predecsor, so when applied to the collection $H_h$ one can conclude there is only one reachable path from the initial state, $h_0$ to any other history.}

%Finally, albeit some intuition about the optimality arguments was given in Section~\ref{ssec:optimality}\nver{, one can deduce the optimality from the arguments employed for $I$-completeness. In particular, the proof relies in the collection of histories $H_h$ defined during the proof of $I$-completeness as well in property (2) of $\prev$. This property stablish an univoque correspondance between a reachable history and its predecsor, so when applied to the collection $H_h$ one can conclude there is only one reachable path from the initial state, $h_0$ to any other history. }


% and secondly show how to define the inverse function of $\textsc{explore}$ and $\textsc{explore-sc}$ for, exploiting a common invariant on the histories explored by the algorithm, deducing a chain of histories starting from the initial state to $\hist$ and concluding that $\hist$ is indeed outputted. For $I$-optimality, we exploit the fact that the history order can be described without referencing any computable path along with the $\genericProtocol$ restriction on re-orderings, to conclude that there is only one possible branch that lead to it. See Appendix~\ref{sec:proofs-algorithm} (in the supplementary material) for more details.
%
%Strong optimality follows from causal extensibility which 
%
%. The former ensure that every extension with a new event returned by $\genericNext$ is $I$-consistent, and the latter implies that $\genericSwap$ outputs histories which are $I$-consistent because 
%
% and the definition 
%
% and causal extensibility: 
%\begin{itemize}
%	\item every history given as an input to a recursive call has at most one pending transaction and this is maximal in $(\so\cup\wro)+$, which implies that it admits an extension with any event,
%	\item and $\genericSwap$ outputs histories which modulo a last read in the pending transaction are prefixes of the input history, and therefore $I$-consistent assuming that the input one is.
%\end{itemize}
%
%As we show in Section~\ref{sec:proofs-algorithm}, the algorithm described above is $I$-sound assuming that $\genericEvaluate(\hist) ::= true$. Therefore, any history computed by applying the functions described above will satisfy the intended isolation level $I$.
%
%TODO THIS SHOULD PROBABLY BE ABOUT CORRECTNESS, STATING IT AND EXPLAINING A LITTLE BIT THE PROOFS.

%Altogether, our swapping-based algorithm can simply being defined as an instance of \ref{algorithm:algo-class}: $\textsc{explore}_{\mathcal{M}}(\nextEvent,\evaluate , \validWrites, \compute, \protocol, \swap)$. A full detailed pseudocode of this procedure can be seen as algorithm \ref{algorithm:optimal-instantiated}; with initial call $h = \emptyset$.

%\begin{algorithm}[H]
%	\caption{Optimal recursive \textsc{STMC}}
%	\begin{algorithmic}[1]
%		\InputAlgorithmic $h$: history
%		\Statex
%		\State $e \gets  \next(h)$
%		\If{$e = \bot$}
%		\If{$\evaluate(h)$}
%		\State \textbf{output} $h$
%		\EndIf
%		%\State $\textbf{\genericEvaluate}(h)$
%		\State \Return
%		\ElsIf{$\textsc{type}(e) = \iread$}
%		
%		\ForAll{$w \in \validWrites(h,e)$} %\writeVar{w}{x}
%		
%		\State $\textsc{explore}_{\mathcal{M}}(h \bullet_w e)$
%		\EndFor
%		\Else
%		\State $\textsc{explore}_{\mathcal{M}}(h \bullet e)$
%		\EndIf
%		
%		\Statex
%		
%		\ForAll{$(\alpha, \beta) \in \compute(h)$}
%		\If{$\protocol(h \bullet e, \alpha, \beta)$}
%		\State $\textsc{explore}_{\mathcal{M}}(\swap(h \bullet e, \alpha, \beta))$	
%		
%		\EndIf
%		\EndFor
%	\end{algorithmic}
%	\label{algorithm:optimal-instantiated}
%\end{algorithm}


==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/causal-extensibility.tex <==
%!TEX root = main.tex
\section{Prefix-Closed and Causally-Extensible Isolation Levels}\label{sec:props}

We define two properties of isolation levels, prefix-closure and causal extensibility, which enable efficient DPOR algorithms (as shown in Section~\ref{sec:CC-algorithm}).

%Besides models presented in figure \ref{fig:consistency_defs}, others isolation levels exists in literature and real life applications \textcolor{red}{cite Constantin's papers + Twitter, shoppingcart...}. However, our algorithm can not be analyzed under an arbitrary model. We characterize in this section the ones that can be employed by our algorithm.
%not all of them can verified with the algorithm

\subsection{Prefix Closure}

For a relation $R\subseteq A\times A$, the restriction of $R$ to $A'\times A'$, denoted by $R\downarrow A'\times A'$, is defined by $\{(a,b): (a,b)\in R, a,b\in A'\}$. Also, a set $A'$ is called $R$-downward closed when it contains $a\in A$ every time it contains some $b\in A$ with $(a,b)\in R$.


\begin{figure}[t]
%		\centering
%	\begin{subfigure}[b]{.25\textwidth}
%		\begin{adjustbox}{max width=\textwidth}
%			\begin{tabular}{c||c||c}
%				\begin{lstlisting}[xleftmargin=5mm,basicstyle=\ttfamily\scriptsize,escapeinside={(*}{*)}, tabsize=1]
%begin;
%a = read((*x*));
%b = read((*y*));
%commit
%				\end{lstlisting} &
%				\begin{lstlisting}[xleftmargin=5mm,basicstyle=\ttfamily\scriptsize,escapeinside={(*}{*)}, tabsize=1]
%begin;
%write((*$x$*),2);
%commit
%				\end{lstlisting} &
%			\begin{lstlisting}[xleftmargin=5mm,basicstyle=\ttfamily\scriptsize,escapeinside={(*}{*)}, tabsize=1]
%begin;
%read((*$x$*));
%commit
%			\end{lstlisting} 
%			\end{tabular} 
%		\end{adjustbox}
%		
%		\caption{Program.}
%		\label{fig:prefix:prog}
%	\end{subfigure}
%	\hspace{.15cm}
	\centering
	\begin{subfigure}[b]{.30\textwidth}
		\resizebox{\textwidth}{!}{
			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
				semithick, transform shape]
				\node[draw, rounded corners=2mm,outer sep=0] (t1) at (-3.25, 0) {\begin{tabular}{l} $\init$ \end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0] (t2) at (-3.25, -1.6) {\begin{tabular}{l} 
						$\rd{x}$ \\ $\rd{y}$
				\end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0] (t3) at (0, 0) {\begin{tabular}{l} 
						$\wrt{x}{2}$
				\end{tabular}};	
				\node[draw, rounded corners=2mm,outer sep=0] (t4) at (0, -1.6)
				{\begin{tabular}{l} 
						$\rd{x}$
				\end{tabular}};			
				
				\path (t1.south west) -- (t1.south) coordinate[pos=0.67] (t1x);
				\path (t2.north west) -- (t2.north) coordinate[pos=0.67] (t2x);
				\path (t3.north west) -- (t3.west) coordinate[pos=0.67] (t3x);
				
				\path (t3.west) edge [below] node[right] {$\wro_x$} (t2.north east);
				\path (t1.south) edge [above] node[left] {$\so \cap \wro_y$} (t2.north);
				\path (t1.east) edge [above] node[above] {$\so$} (t3.west);
				\path (t3.south) edge node[right] {$\wro_x$} (t4.north);
				\path (t1.south east) edge node[below] {$\so$} (t4.north west);
			\end{tikzpicture}
			
		}
		\caption{A history.}
		\label{fig:prefix:a}
	\end{subfigure}
	\hspace{.15cm}
	\centering
	\begin{subfigure}[b]{.30\textwidth}
		\resizebox{\textwidth}{!}{
			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
				semithick, transform shape]
				\node[draw, rounded corners=2mm,outer sep=0] (t1) at (-3.25, 0) {\begin{tabular}{l} $\init$ \end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0] (t2) at (-3.25, -1.6) {\begin{tabular}{l} 
						$\rd{x}$ \\ $\rd{y}$
				\end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0] (t3) at (0, 0) {\begin{tabular}{l} 
						$\wrt{x}{2}$
				\end{tabular}};			
				
				\path (t1.south west) -- (t1.south) coordinate[pos=0.67] (t1x);
				\path (t2.north west) -- (t2.north) coordinate[pos=0.67] (t2x);
				\path (t3.north west) -- (t3.west) coordinate[pos=0.67] (t3x);
				
				\path (t3.west) edge [below] node[right] {$\wro_x$} (t2.north east);
				\path (t1.south) edge [above] node[left] {$\so \cap \wro_y$} (t2.north);
				\path (t1.east) edge [above] node[above] {$\so$} (t3.west);

			\end{tikzpicture}
		}
		\caption{A prefix.}
		\label{fig:prefix:b}
	\end{subfigure}
	\hspace{.15cm}
	\centering
	\begin{subfigure}[b]{.30\textwidth}
		\resizebox{\textwidth}{!}{
			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
				semithick, transform shape]
				\node[draw, rounded corners=2mm,outer sep=0] (t1) at (-3.25, 0) {\begin{tabular}{l} $\init$ \end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, ] (t2) at (-3.25, -1.4) {\begin{tabular}{l} 
						$\rd{x}$ \\ $\rd{y}$
				\end{tabular}};
%				\node[draw, rounded corners=2mm,outer sep=0, white] (t3) at (0, 0) {\begin{tabular}{l} 
%					$\wrt{x}{2}$
%				\end{tabular}};	
				\node[draw, rounded corners=2mm,outer sep=0] (t4) at (0, -1.4)
				{\begin{tabular}{l} 
						$\rd{x}$
				\end{tabular}};			
				
				\path (t1.south west) -- (t1.south) coordinate[pos=0.67] (t1x);
				\path (t2.north west) -- (t2.north) coordinate[pos=0.67] (t2x);
				\path (t3.north west) -- (t3.west) coordinate[pos=0.67] (t3x);
				
				\path (t1.south east) edge node[below] {$\so$} (t4.north west);
%				\path (t3.west) edge [below] node[right] {$\wro_x$} (t2.north east);
				\path (t1.south) edge [above] node[left] {$\so \cap \wro_y$} (t2.north);
%				\path (t3.south) edge node[right] {$\wro_x$} (t4.north);
			\end{tikzpicture}
			
		}
		\caption{Not a prefix.}
		\label{fig:prefix:c}
	\end{subfigure}
	\vspace{-2mm}
	\caption{Explaining the notion of prefix of a history. $\init$ denotes the transaction log writing initial values. Boxes group events from the same transaction.}
	\vspace{-4mm}
\end{figure}
%where $T'$ contains prefixes of a subset of transaction logs $T''\subseteq T$ such that $T''$ is $(\so \cup \wro)^*$-downward closed.  

A \emph{prefix} of a transaction log $\tup{t,E, \po_t}$ is a transaction log $\tup{t,E', \po_t \downarrow E'\times E'}$ such that $E'$ is $\po_t$-downward closed. 
A \emph{prefix} of a history $\hist=\tup{T, \so, \wro}$ is a history $\hist'=\tup{T',\so\downarrow T'\times T',\wro\downarrow T'\times T'}$ such that every transaction log in $T'$ is a prefix of a different transaction log in $T$ but carrying the same id, $\events{\hist'}\subseteq\events{\hist}$, and $\events{\hist'}$ is $(\po\cup \so \cup \wro)^*$-downward closed.
For example, the history pictured in Fig.~\ref{fig:prefix:b} is a prefix of the one in Fig.~\ref{fig:prefix:a} while the history in Fig.~\ref{fig:prefix:c} is not. The transactions on the bottom of Fig.~\ref{fig:prefix:c} have a $\wro$ predecessor in Fig.~\ref{fig:prefix:a} which is not included.

\vspace{-1.5mm}
\begin{definition}
An isolation level $I$ is called \emph{prefix-closed} when every prefix of an $I$-consistent history is also $I$-consistent.
\vspace{-1.5mm}
\end{definition}

%For be denominated as \callout{STMC-model}, $\mathcal{M}$ has to satisfies the following three axioms for every program $\mathcal{P}$:

%Comparing to the model requirements described in \textcolor{red}{cite viktor's algorithm}, it is causal-extensibility property, a slightly stricter version of \textcolor{red}{Viktor}'s maximal-extensibility, the biggest difference. However, this weak formulation still forbids some axiomatic models such as Serializability \textcolor{red}{cite constantin's paper (SER)} \textcolor{red}{Appendix cite}.
%Indeed, some isolation levels cannot guarantee that reading from the last added $\iwrite$ event will maintain its consistency status.
Every isolation level $I$ discussed above is prefix-closed because if a history $\hist$ is $I$-consistent with a commit order $\co$, then the restriction of $\co$ to the transactions that occur in a prefix $\hist'$ of $\hist$ satisfies the corresponding axiom(s) when interpreted over $\hist'$. %Therefore, all these levels are prefix-clos
%When the isolation level is defined with an equation such as \ref{eq:axioms}, the restriction of $\co$ to the transactions that occur in a prefix $\hist'$ of a history $\hist$ satisfies the corresponding axiom(s) when interpreted over $\hist'$.

\vspace{-2mm}
\begin{theorem}
\textit{Read Committed}, \textit{Read Atomic}, \textit{Causal Consistency}, \textit{Snapshot Isolation}, and \textit{Serializability} are prefix closed.
\vspace{-1.5mm}
\end{theorem}
\begin{comment}
\begin{proof}(Sketch)
Let $\hist$ be a history that satisfies one of these isolation levels, and let $\co$ be a commit order of $\hist$ that satisfies the corresponding axiom(s). The restriction of $\co$ to the transactions that occur in a prefix $\hist'$ of $\hist$ satisfies the corresponding axiom(s) when interpreted over $\hist'$.
%As any $\so \cup \wro$-prefix-closed sub-history $h'$ of $h$ is a sub-graph of it, and there is a commit order $\co$ for $h$, it suffices to restrict $\co$ to $h'$ for obtaining a commit order for $h'$.
\end{proof}
\end{comment}

\subsection{Causal Extensibility}\label{ssec:causal_ext}

\begin{figure}[t]
	\begin{minipage}[b]{0.66\textwidth}
	
		\centering
		\begin{subfigure}[b]{.46\textwidth}
			\resizebox{\textwidth}{!}{
				\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
					semithick, transform shape]
					\node[draw, rounded corners=2mm,outer sep=0] (t1) at (-3.25, 0) {\begin{tabular}{l} $\init$ \end{tabular}};
					\node[draw, rounded corners=2mm,outer sep=0] (t2) at (-3.25, -1.6) {\begin{tabular}{l} 
							$\rd{x}$ \\ \textbf{\textcolor{blue}{$\rd{y}$}} %\pgfsetfillopacity{0.3}
					\end{tabular}};
					\node[draw, rounded corners=2mm,outer sep=0] (t3) at (0, 0) {\begin{tabular}{l} 
							$\wrt{x}{2}$%\\
							%\pgfsetfillopacity{0.3}$\wrt{y}{2}$
					\end{tabular}};			
					
					\path (t1.south west) -- (t1.south) coordinate[pos=0.67] (t1x);
					\path (t2.north west) -- (t2.north) coordinate[pos=0.67] (t2x);
					\path (t3.north west) -- (t3.west) coordinate[pos=0.67] (t3x);
					
					\path (t3.west) edge [below] node[right] {$\wro_x$} (t2.north east);
					\path (t1.south) edge [above] node[left] {$\so$} (t2.north);
					\path (t1.east) edge [above] node[above] {$\so$} (t3.west);
					%\path (t1x) edge [right] node {$\wro_y$} (t2x);
				\end{tikzpicture}  
				
			}
			\caption{Extensible history.}
			\label{fig:maxclosed:a}
		\end{subfigure}
		\hspace{.1cm}
		\centering
		\begin{subfigure}[b]{.5\textwidth}
			\resizebox{\textwidth}{!}{
				\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
					semithick, transform shape]
					\node[draw, rounded corners=2mm,outer sep=0] (t1) at (-3.25, 0) {\begin{tabular}{l} $\init$ \end{tabular}};
					\node[draw, rounded corners=2mm,outer sep=0] (t2) at (-3.25, -1.6) {\begin{tabular}{l} 
							$\rd{x}$ \\ $\rd{y}$
					\end{tabular}};
					\node[draw, rounded corners=2mm,outer sep=0] (t3) at (0, 0) {\begin{tabular}{l} 
							$\wrt{x}{2}$\\
							\textbf{\textcolor{blue}{$\wrt{y}{2}$}}
					\end{tabular}};			
					
					\path (t1.south west) -- (t1.south) coordinate[pos=0.67] (t1x);
					\path (t2.north west) -- (t2.north) coordinate[pos=0.67] (t2x);
					\path (t3.north west) -- (t3.west) coordinate[pos=0.67] (t3x);
					
					\path (t3.west) edge [below] node[right] {$\wro_x$} (t2.north east);
					\path (t1.south) edge [above] node[left] {$\so \cap \wro_y$} (t2.north);
					\path (t1.east) edge [above] node[above] {$\so$} (t3.west);
				\end{tikzpicture}
				
			}
			\caption{Non-extensible history.}
			\label{fig:maxclosed:b}
		\end{subfigure}
		\centering
		\vspace{-2mm}
		\caption{Explaining causal extensibility. $\init$ denotes the transaction log writing initial values. Boxes group events from the same transaction.
		%We write $\so \cap \wro_x$ when there is a $\so$ and a $\wro_x$ edge sharing both source and target.
		}
		\vspace{-2mm}

		\label{fig:maxclosed}
		%\vspace{-3mm}

	\end{minipage}
	\hfill
	\begin{minipage}[b]{0.32\textwidth}
		\resizebox{\textwidth}{!}{
			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
				semithick, transform shape]
				\node[draw, rounded corners=2mm,outer sep=0] (t1) at (-1.5, -0.25) {\begin{tabular}{l} $\init$ \end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0] (t2) at (-3, -2) {\begin{tabular}{l} 
						$\wrt{z}{1}$ \\ $\rd{x}$ \\ $\wrt{y}{1}$ 
				\end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0] (t3) at (0, -2) {\begin{tabular}{l} 
						$\wrt{z}{2}$ \\ $\rd{y}$ \\ 	\textbf{\textcolor{blue}{$\wrt{x}{2}$}}
				\end{tabular}};		
				
				\path (t1.south west) -- (t1.south) coordinate[pos=0.67] (t1sw);
				\path (t1.south east) -- (t1.south) coordinate[pos=0.67] (t1se);
				\path (t2.north east) -- (t2.north) coordinate[pos=0.67] (t2x);
				\path (t3.north west) -- (t3.north) coordinate[pos=0.67] (t3x);
				
				%\path (t3x) edge [above] node[yshift=8,xshift=0] {$\wro_x$} (t2.north east);
				\path (t1sw) edge [left] node {$\wro_x$} (t2x);
				\path (t1se) edge [right] node {$\wro_y$} (t3x);
			\end{tikzpicture}  
		}

	\vspace{-2mm}

	\caption{A counter-example to causal extensibility for $\SI$ and $\SER$. 
	%A bi-threaded program and a $\SER$/ $\SI$-consistent history. Events in gray are not yet added to the history. 
	The $\so$-edges from $\init$ to the other transactions are omitted for legibility.}
	\vspace{-2mm}

	\label{fig:non-causally-extensible}

	\end{minipage}
\vspace{-2mm}
\end{figure}



We start with an example to explain causal extensibility. Let us consider the histories $h_1$ and $h_2$ in Figures~\ref{fig:maxclosed:a} and \ref{fig:maxclosed:b}, respectively, \emph{without} the events $\erd{y}$ and $\ewrt{y,2}$ written in blue bold font. These histories satisfy Read Atomic. 
%respectively under RA; isolation level under which both are consistent. 
The history $h_1$ can be extended by adding the event $\rd{y}$ and the $\wro$ dependency $\wro(\init,\rd{y})$ while still satisfying Read Atomic.
%$w_1 \ [\wro] \ r_1$, where $w_1 = \wrt{x}{0}$. 
On the other hand, the history $h_2$ \emph{can not} be extended with the event $\wrt{y}{2}$ while still satisfying Read Atomic. Intuitively, if the reading transaction on the bottom reads $x$ from the transaction on the right, then it should read $y$ from the same transaction because this is more ``recent'' than $\init$ w.r.t. session order. The essential difference between these two extensions is that the first concerns a transaction which is maximal in $(\so\cup\wro)^+$ while the second no. The extension of $\hist_2$ concerns the transaction on the right in Figure~\ref{fig:maxclosed:b} which is a $\wro$ predecessor of the reading transaction. Causal extensibility will require that at least the $(\so\cup\wro)^+$ maximal (pending) transactions can always be extended with any event while still preserving consistency. The restriction to $(\so\cup\wro)^+$ maximal transactions is intuitively related to the fact that transactions should not read from non-committed (pending) transactions, e.g., the reading transaction in $\hist_2$ should not read from the still pending transaction that writes $x$ and later $y$.

%this is not the case of $h_2$: the only event that could be added in it is $w_2 = \wrt{y}{2}$. If $w_2$ would be added in $h_2$, any relation extending $\so \cup \wro$ and satisfying RA would be cyclic, so it wouldn't be a commit order. The essential difference between these two histories is the following: in $h_1$, $\tr(r)$ is $\so \cup \wro$-maximal while in $h_2$ $\tr(w)$ is not. As real database executions forbid transactions reading from non-committed ones, it is reasonable to allow those transactions $\so \cup \wro$-maximal to be executed completed without hindering the previous committed transactions. 
Formally, let  $\hist=\tup{T, \so, \wro}$ be a history. A transaction $t$ is called $(\so \cup \wro)^+$-maximal in $h$ if $h$ does not contain any transaction $t'$ such that $(t,t')\in (\so \cup \wro)^+$. We define a \emph{causal extension} of a pending transaction $t$ in $h$ with an event $e$ as \nver{a history $h'$} such that:
\vspace{-1mm}
\begin{itemize}
\item $e$ is added to $t$ as a maximal element of $\po_t$,
\item if $e$ is a read event and $t$ \emph{does not} contain a write to $\mathit{var}(e)$, then $\wro$ is extended with some tuple $(t',e)$ such that $(t', t) \in  (\so \cup \wro)^+$ \nver{in $h$} \nver{(if $e$ is a read event and $t$ \emph{does} contain a write to $\mathit{var}(e)$, then the value returned by $e$ is the value written by the latest write on $\mathit{var}(e)$ before $e$ in $t$; the definition of the return value in this case is unique and does not involve $\wro$ dependencies),}
\item the other elements of $\hist$ remain unchanged \nver{in $h'$}.
\vspace{-1mm}
\end{itemize}

\begin{figure}[t]
%	\centering
%	\begin{subfigure}[b]{.25\textwidth}
%		\begin{adjustbox}{max width=\textwidth}
%			\begin{tabular}{c||c}
%				\begin{lstlisting}[xleftmargin=5mm,basicstyle=\ttfamily\scriptsize,escapeinside={(*}{*)}, tabsize=1]
%begin;
%write((*$y$*),1);
%write((*$x$*),1);
%commit
%begin;
%write((*$x$*),2);
%commit
%				\end{lstlisting} &
%				\begin{lstlisting}[xleftmargin=5mm,basicstyle=\ttfamily\scriptsize,escapeinside={(*}{*)}, tabsize=1]
%begin;
%write((*$x$*),3);
%commit
%begin;
%a = read((*$y$*));
%b = read((*$x$*));
%commit
%				\end{lstlisting}
%			\end{tabular} 
%		\end{adjustbox}
%		
%		\caption{Program.\\$ $}
%		\label{fig:extension:prog}
%	\end{subfigure}
%	\hspace{.15cm}
%	\centering
	\begin{subfigure}[t]{.28\textwidth}
		\resizebox{\textwidth}{!}{
			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
				semithick, transform shape]
				\node[draw, rounded corners=2mm,outer sep=0] (t0) at (-1.5, 0) {\begin{tabular}{l} $\init$ \end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, label={[font=\small]100:$t_1$}] (t1) at (-3, -1.6) {\begin{tabular}{l} 
					$\wrt{x}{1}$ \\ $\wrt{y}{1}$
				\end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, label={[font=\small]50:$t_2$}] (t2) at (-3, -3.2) {\begin{tabular}{l} 
					$\wrt{x}{2}$
				\end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, label={[font=\small]50:$t_3$}] (t3) at (0, -1.6) {\begin{tabular}{l} 
						$\wrt{x}{3}$
				\end{tabular}};	
				\node[draw, rounded corners=2mm,outer sep=0, label={[font=\small]50:$t_4$}] (t4) at (0, -3.2)
				{\begin{tabular}{l} 
						$\rd{y}$ \\ $\cdots$%$\rd{x}$}
				\end{tabular}};			
				
				\path (t1.south west) -- (t1.south) coordinate[pos=0.67] (t1x);
				\path (t2.north west) -- (t2.north) coordinate[pos=0.67] (t2x);
				\path (t3.north west) -- (t3.west) coordinate[pos=0.67] (t3x);
				
				%\path (t3.west) edge [below] node[right] {$\wro_x$} (t2.north east);
				%\path (t1.south) edge [above] node[left] {$\so \cap \wro_y$} (t2.north);
				\path (t3.south) edge node[right] {$\so$} (t4.north);
				\path (t1.south) edge node[left] {$\so$} (t2.north);
				\path (t1.south east) edge node[above] {$\wro_y$} (t4.north west);
				\path (t0.south) edge node[above] {$\so$} (t1.north);
				\path (t0.south) edge node[above] {$\so$} (t3.north);
			\end{tikzpicture}
			
		}
		\vspace{-5.5mm}
		\caption{History $\hist$.}
		\label{fig:extension:a}
	\end{subfigure}
	\hspace{.15cm}
	\centering
	\begin{subfigure}[t]{.28\textwidth}
		\resizebox{\textwidth}{!}{
			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
				semithick, transform shape]
				\node[draw, rounded corners=2mm,outer sep=0] (t0) at (-1.5, 0) {\begin{tabular}{l} $\init$ \end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, label={[font=\small]100:$t_1$}] (t1) at (-3, -1.6) {\begin{tabular}{l} 
						$\wrt{x}{1}$ \\ $\wrt{y}{1}$
				\end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, label={[font=\small]50:$t_2$}] (t2) at (-3, -3.2) {\begin{tabular}{l} 
						$\wrt{x}{2}$
				\end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, label={[font=\small]50:$t_3$}] (t3) at (0, -1.6) {\begin{tabular}{l} 
						$\wrt{x}{3}$
				\end{tabular}};	
				\node[draw, rounded corners=2mm,outer sep=0, label={[font=\small]50:$t_4$}] (t4) at (0, -3.2)
				{\begin{tabular}{l} 
						$\rd{y}$ \\ \textbf{\textcolor{blue}{$\rd{x}$}}
				\end{tabular}};			
				
				\path (t1.south west) -- (t1.south) coordinate[pos=0.67] (t1x);
				\path (t2.north west) -- (t2.north) coordinate[pos=0.67] (t2x);
				\path (t3.north west) -- (t3.west) coordinate[pos=0.67] (t3x);
				
				%\path (t3.west) edge [below] node[right] {$\wro_x$} (t2.north east);
				%\path (t1.south) edge [above] node[left] {$\so \cap \wro_y$} (t2.north);
				\path (t3.south) edge node[right] {$\so$} (t4.north);
				\path (t1.south) edge node[left] {$\so$} (t2.north);
				\path (t1.south east) edge node[above, xshift = 4mm,yshift=-1mm] {$\wro_y$, $\wro_x$} (t4.north west);
				\path (t0.south) edge node[above] {$\so$} (t1.north);
				\path (t0.south) edge node[above] {$\so$} (t3.north);
			\end{tikzpicture}
		}
		\vspace{-5.5mm}
		\caption{$t_4$ reads $x$ and $y$ from $t_1$.}
		\label{fig:extension:b}
	\end{subfigure}
	\hspace{.15cm}
	\centering
	\begin{subfigure}[t]{.28\textwidth}
		\resizebox{1.1\textwidth}{!}{
			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
				semithick, transform shape]
				\node[draw, rounded corners=2mm,outer sep=0] (t0) at (-1.5, 0) {\begin{tabular}{l} $\init$ \end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, label={[font=\small]100:$t_1$}] (t1) at (-3, -1.6) {\begin{tabular}{l} 
						$\wrt{x}{1}$ \\ $\wrt{y}{1}$
				\end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, label={[font=\small]50:$t_2$}] (t2) at (-3, -3.2) {\begin{tabular}{l} 
						$\wrt{x}{2}$
				\end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, label={[font=\small]50:$t_3$}] (t3) at (0, -1.6) {\begin{tabular}{l} 
						$\wrt{x}{3}$
				\end{tabular}};	
				\node[draw, rounded corners=2mm,outer sep=0, label={[font=\small]10:$t_4$}] (t4) at (0, -3.2)
				{\begin{tabular}{l} 
						$\rd{y}$ \\ \textbf{\textcolor{blue}{$\rd{x}$}}
				\end{tabular}};			
				
				\path (t1.south west) -- (t1.south) coordinate[pos=0.67] (t1x);
				\path (t2.north west) -- (t2.north) coordinate[pos=0.67] (t2x);
				\path (t3.north west) -- (t3.west) coordinate[pos=0.67] (t3x);
				
				%\path (t3.west) edge [below] node[right] {$\wro_x$} (t2.north east);
				%\path (t1.south) edge [above] node[left] {$\so \cap \wro_y$} (t2.north);
				\path (t1.south east) edge node[above] {$\wro_y$} (t4.north west);
				\path (t3.south) edge node[right] {$\so \cap \wro_x$} (t4.north);
				\path (t1.south) edge node[left] {$\so$} (t2.north);
				\path (t0.south) edge node[above] {$\so$} (t1.north);
				\path (t0.south) edge node[above] {$\so$} (t3.north);
			\end{tikzpicture}
			
		}
		\vspace{-5.5mm}
		\caption{$t_4$ reads $x$ from $t_3$, $y$ from $t_1$.}
		\label{fig:extension:c}
	\end{subfigure}
	\vspace{-4mm}
	\caption{Two causal extensions of the history $h$ on the left with the $\erd{x}$ event written in blue.}
	\vspace{-3.5mm}
\end{figure}

For example, Figure~\ref{fig:extension:b} and~\ref{fig:extension:c} present two causal extensions with a $\erd{x}$ event of the transaction $t_4$ in the history $\hist$ in Figure~\ref{fig:extension:a}. The new read event reads from transaction $t_1$ or $t_3$ which were already related by $(\so \cup \wro)^+$ to $t_4$.
An extension of $h$ where the new read event reads from $t_2$ is \emph{not} a causal extension because $(t_2, t_4) \not\in (\so \cup \wro)^+$.
%and $y$ from $t_1$ is not included as it is not a causal extension ($(t_2, t_4) \not\in \so \cup \wro$)

\vspace{-1.5mm}
\begin{definition}
\label{def:causally-extensible}
An isolation level $I$ is called \emph{causally-extensible} if for every $I$-consistent history $h$, every $(\so \cup \wro)^+$-maximal pending transaction $t$ in $h$, and every event $e$, there exists a causal extension $\hist'$ of $t$ with $e$ that is $I$-consistent.
%	can be extended with an event from a $\so \cup \wro$-maximal pending transaction $T$ in $h$. Moreover, if that event $r$ is a $\iread$, it can always read from a $\iwrite$ event $w$ s.t. in $h$ $\tr(w) \ (\so \cup \wro)^* \ \tr(r)$.
\vspace{-1.5mm}
\end{definition}

\appendixver{The proof of the following theorem can be found in Appendix~\ref{app:causalExtensible}.}

\vspace{-1.5mm}
\begin{restatable}{theorem}{causalExtensibleModels}
\label{theorem:causalExtensibleModels-CC-RA-RC}
Causal Consistency, Read Atomic, and Read Committed are causally-extensible.
\vspace{-1.5mm}
\end{restatable}

%\vspace{-3mm}

Snapshot Isolation and Serializability are \emph{not} causally extensible. 
Figure~\ref{fig:non-causally-extensible} presents a counter-example to causal extensibility: the causal extension of the history $\hist$ that does \emph{not} contain the $\ewrt{x,2}$ written in blue bold font with this event does not satisfy neither Snapshot Isolation nor Serializability although $\hist$ does. Note that the causal extension with a write event is unique. \nver{(Note that both $h$ and this causal extension satisfy Causal Consistency and therefore, as expected, this counter-example does not apply to isolation levels weaker than Causal Consistency.)}
%we exhibit why $\SI$ and $\SER$ are not causally extensible. For the program in Figure~\ref{fig:non-causally-extensible:prog-ser}, the history presented in Figure~\ref{fig:non-causally-extensible:ser} is $\SER$-consistent (and therefore $\SI$-consistent) but whose only extension (Figure~\ref{fig:non-causally-extensible:ser-cont}) is $\SI$-inconsistent (and therefore $\SER$-inconsistent).




%\input{proofs:causal-extensibility}


==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/conclusions.tex <==
%!TEX root = main.tex
%\vspace{-5mm}
\section{Conclusions}\label{sec:conc}

We presented efficient SMC algorithms based on DPOR for transactional programs running under standard isolation levels. These algorithms are instances of a generic schema, called swapping-based algorithms, which is parametrized by an isolation level. Our algorithms are sound and complete, and  polynomial space. Additionally, we identified a class of isolation levels, including $\RC$, $\RA$, and $\CC$, for which our algorithms are strongly optimal, and we showed that swapping-based algorithms cannot be strongly optimal for stronger levels $\SI$ and $\SER$ (but just optimal). For the isolation levels we considered, there is an intriguing coincidence between the existence of a strongly optimal swapping-based algorithm and the complexity of checking if a given history is consistent with that level. Indeed, checking consistency is polynomial time for $\RC$, $\RA$, and $\CC$, and NP-complete for $\SI$ and $\SER$. 
%for RC, RA, and CC, , and for both SI and SER, there are no strongly optimal swapping-based algorithms and checking consistency is NP-complete. 
Investigating further the relationship between strong optimality and polynomial-time consistency checks is an interesting direction for future work. 
%An interesting question to investigate is the characterization of isolation levels for which strong optimality can be ensured (under the swapping-based paradigm), and whether this characterization is related to the complexity of checking consistency. 

==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/data-availability-statement.tex <==
%!TEX root = main.tex
\section*{Data availability statement}

The implementation is open-source and can be found in \cite{anonymous_2023_7824546}.

==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/experimental-evaluation.tex <==
%!TEX root = main.tex
\section{Experimental evaluation}\label{sec:exp}

We evaluate an implementation of $\textsc{explore-ce}$ and $\textsc{explore-ce}^*$ in the context of the Java Pathfinder (JPF)~\cite{DBLP:conf/issta/VisserPK04} model
checker for Java concurrent programs. As benchmark, we use bounded-size client programs of a number of database-backed applications drawn from the literature. % of distributed systems and databases
The experiments were performed on an Apple M1 with $8$ cores and $16$ GB of RAM.

%%Each client is a different program (following the terminology in Section 2). 5 clients x 3 sessions means 5 independent programs where each program executes 3 sessions. Those clients are studied in isolation, not considering any interleaving between them. We will clarify.

\subsection{Implementation}

We implemented our algorithms as an extension of the \texttt{DFSearch} class in JPF. For performance reasons, we implemented an iterative version of these algorithms where roughly, inputs to recursive calls are maintained as a collection of histories instead of relying on the call stack. For checking consistency of a history with a given isolation level, we implemented the algorithms proposed by \citet{DBLP:journals/pacmpl/BiswasE19}. %We plan to make our implementation publicly available.

%$\textsc{explore-ce}$ and $\textsc{explore-ce}^*$ on top of JPF and an implementation of the algorithms proposed by \citet{DBLP:journals/pacmpl/BiswasE19} for checking consistency of a history with a given isolation level. For performance issues, we implemented an iterative version of these algorithms 

%\ref{algorithm:algo-class} for reducing the actual memory consumption. We employ an annotated stack of database states that is modified in each $\textsc{explore-ce}$ call; and we consider the algorithm works with list instead of simply sets.
%At every step where we execute a $\iread$, we annotate which $\iwrite$ event is reading from and  when the state pops from the stack, we change the $\wro$-dependency. Analogously, at every step we produce a swap, we annotate which tuple given by $\compute$ we used in the swap for selecting a different tuple when the state is popped out.
Our tool takes as input a Java program and isolation levels as parameters. We assume that the program uses a fixed API for interacting with the database, similar to a key-value store interface. This API consists of specific methods for starting/ending a transaction, and reading/writing a global variable. The fixed API is required for being able to maintain the database state separately from the JVM state (the state of the Java program) and update the current history in each database access. This relies on a mechanism for ``transferring'' values read from the database state to the JVM state. 
% a verification tool for Java concurrent programs. We admit as input a Java program that (1) can be parsed and executed by JPF and (2) employs the API according to the specifications. Our tool is parametric in the isolation levels employed.

%The API provided allow $\ibegin, \iwrite, \iread$ and $\icommit$ operations. Thanks to this API, we can maintain the database state separately from JPF's internal state and update the current history in each database call. We do not rely on any concrete database but store the information as a collection of String, one per write API call executed; along with the $\so$, $\wro$-dependencies between the events associated to them. Any time there is a need to connect data from the local state to the database one or viceversa we copy and store the concrete String value from one state to the other. %Altogether, we are able to simulate from simple variables to actual tables provided the client has proper methods to transform from one to the other representative.

%Our implementation is compatible with JPF's standards, as both algorithm are instances of DFSearch; a JPF for DFS exploring algorithms. Moreover, we built consistency checkers based on the algorithm's presented in \textcolor{red}{Ranadeep and Enea's paper} for different isolation levels to ensure database's soundness. 

%However, for performance issues, we developed an iterative version of the algorithm \ref{algorithm:algo-class} for reducing the actual memory consumption. We employ an annotated stack of database states that is modified in each $\textsc{explore-ce}$ call; and we consider the algorithm works with list instead of simply sets.
%At every step where we execute a $\iread$, we annotate which $\iwrite$ event is reading from and  when the state pops from the stack, we change the $\wro$-dependency. Analogously, at every step we produce a swap, we annotate which tuple given by $\compute$ we used in the swap for selecting a different tuple when the state is popped out. % In addition, as JPF is not designed for supporting database operations, we developed an API that simulates every database instruction. operations, but they have been proved expressive enough both during our experiments and in real time applications. We admit any Java program that (1) can be parsed and executed by JPF and (2) has an equivalent translation into a program written with the syntax defined in Figure~\ref{fig:syntax}.

\vspace{-1mm}
\subsection{Benchmark}

We consider a set of benchmarks inspired by real-world applications and evaluate them under different types of client programs and isolation levels.
%both implemented following the aforementioned specifications. We provide also examples of different behaviors depending on the isolation level for each applications.

%\vspace{1mm}
%\noindent
\textit{Shopping Cart~\cite{sivaramakrishnan2015declarative5}} allows users to add, get and remove items from their shopping cart and modify the quantities of the items present in the cart. 
%We employ only one table, $\texttt{cart}$, in this application. Given a program that add an item in one section and deletes it in another one, we may observe, depending on the isolation level, that at the end of the execution the cart contains either zero, one or two items.

%\vspace{1mm}
%\noindent
\textit{Twitter~\cite{difallah2013oltp}} allows users to follow other users, publish tweets and get their followers, tweets and tweets published by other followers. 
%We model twitter with four tables: $\texttt{users}, \texttt{tweets}, \texttt{followed}, \texttt{followers}$. Under weak isolation levels, it is possible that one user can publish a tweet and not being able to obtain it from a different session. We can also detect other behaviors as users following another users in one session but the latter not being able to find the former as a follower.

%\vspace{1mm}
%\noindent
\textit{Courseware~\cite{DBLP:conf/esop/NairP020}} manages the enrollment of students in courses in an institution. It allows to open, close and delete courses, enroll students and get all enrollments. One student can only enroll to a course if it is open and its capacity has not reached a fixed limit. 
%It employs three tables, $\texttt{student}, \texttt{course}$ and $\texttt{enrollments}$. Under weak isolation levels, two students in different sessions may enroll to a course with only one free place or being able to enroll into a course that has been deleted in another session.

%\vspace{1mm}
%\noindent
\textit{Wikipedia~\cite{difallah2013oltp}} allows users to get the content of a page (registered or not), add or remove pages to their watching list and update pages. 
%It employs ten tables, but the vast majority of procedures only access to a small subset of them. Under weak isolation levels, one change in a page may be overwritten by another one done in a different session as well as the watching list may contain a variable number of pages if they are added/deleted from different sessions.

%\vspace{1mm}
%\noindent
\textit{TPC-C~\cite{TPCC}} models an online shopping application with five types of transactions: reading the stock of a product, creating a new order, getting its status, paying it and delivering it. 
%TPC-C employs nine tables and all its procedures read and write several variables. Under weak isolation level two orders may be created from different sessions or the account balance may be inconsistent if some order is payed twice.

\nver{SQL tables are modeled using a ``set'' global variable whose content is the set of ids (primary keys) of the rows present in the table, and a set of global variables, one variable for each row in the table (the name of the variable is the primary key of that row). SQL statements such as INSERT and DELETE statements are modeled as writes on that ``set'' variable while SQL statements with a WHERE clause (SELECT, JOIN, UPDATE) are compiled to a read of the table's set variable followed by reads or writes of variables that represent rows in the table (similarly to~\cite{DBLP:journals/pacmpl/BiswasKVEL21}).} % following a starting read of the table's set variable.} (see~\cite{DBLP:journals/pacmpl/RahmaniNDJ19,DBLP:journals/pacmpl/BiswasKVEL21}).
% \nver{All SQL instructions are translated to key-value paradigm by adding a ``set'' variable per table whose content is the set of  ids (primary keys) of the rows present in the table. The translation of every SQL instruction with a WHERE clause starts reading this variable while INSERT and DELETE are modelled as writes on it.}

\vspace{-1mm}
\subsection{Experimental Results}

We designed three experiments where we compare the performance of a baseline model checking algorithm, $\textsc{explore-ce}$ and $\textsc{explore-ce}^*$ for different (combinations of) isolation levels, and we explore the scalability of $\textsc{explore-ce}$ when increasing the number of sessions and transactions per session, respectively.
\appendixver{All data is exhibited in Appendix~\ref{sec:appendix:experiments} in the supplementary material \cite{bouajjani2023dynamic}. }For each experiment we report running time, memory consumption, and the number of end states, i.e., histories of complete executions and in the case of $\textsc{explore-ce}^*$, before applying the $\genericEvaluate$ filter. As the number of end states for a program on a certain isolation level increases, the running time of our algorithms naturally increases as well. 

%We have run three type of experiments to determine the algorithm's scalability. The more transactions that write into the database, the more potential behaviors allowed. Therefore, in each case we design the experiments with this guideline.



%\footnotetext{\nver{ $\CC$, $\CC + \SI$ and $\CC + \SER$ graphics overlap.}}

%Each client is a different program (following the terminology in Section 2). 5 clients x 3 sessions means 5 independent programs where each program executes 3 sessions. Those clients are studied in isolation, not considering any interleaving between them. We will clarify.

The first experiment  compares the performance of our algorithms for different combinations of isolation levels and a baseline model checking algorithm that performs no partial order reduction. We consider as benchmark five \nver{(independent)} client programs\footnote{For an application that defines a number of transactions, a client program consists of a number of sessions, each session containing a sequence of transactions defined by the application.} for each application described above ($25$ in total), each \nver{program} with 3 sessions and 3 transactions per session. Running time, memory consumption, and number of end states are reported in Fig.~\ref{fig:results1} as \nver{cactus plots~\cite{DBLP:conf/issac/BrainDG17}.} %added the citation of cactus plot.

\begin{figure}[t]
	\centering
	\begin{subfigure}[t]{0.322\linewidth}
		\centering
		\includegraphics[width=\textwidth]{figures/app-scala-Time.eps}
		\vspace{-5mm}
		\caption{Running time.}%$10$ $11$ and $18$ benchmarks timeout for $\langle \RC, \CC \rangle$, $\langle \texttt{true}, \CC \rangle$ and $\textsc{DFS}(\CC)$ respectively.
		%\caption{Execution time. For the last program, the running time is $25' 17''$ under $\RA$ and $33' 3''$ under $\langle\RA, \CC\rangle$ (out of the figure).}
		\label{fig:results-ra-cc}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.322\linewidth}
		\centering
		\includegraphics[width=\textwidth]{figures/app-scala-Mem.eps}
		\vspace{-5mm}
		\caption{Memory consumption.}
		\label{fig:results-memory}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.322\linewidth}
		\centering
		\includegraphics[width=\textwidth]{figures/app-scala-histories.eps}
		\vspace{-5mm}
		\caption{End states.}
		\label{fig:results-histories}
	\end{subfigure}
\vspace{-3mm}
	\caption[where every history is consistent]{Cactus plots comparing different algorithms in terms of time, memory, and end states. For readability, we use $\CC$ to denote $\textsc{explore-ce}$ under $\CC$, $I_1 + I_2$ stands for $\textsc{explore-ce}^*(I_1, I_2)$, and $\texttt{true}$ is the trivial isolation level where every history is consistent. \nver{Differences between $\CC$, $\CC + \SI$ and $\CC + \SER$ are very small and their graphics overlap.} Moreover, $\textsc{DFS}(\CC)$ denotes a standard DFS traversal of the semantics defined in Section~\ref{ssec:semantics}. These plots exclude benchmarks that timeout ($30$ mins): $3$ benchmarks for $\CC$, $\langle \SI, \CC \rangle$ and $\langle \SER, \CC \rangle$ and $6$, $17$, $20$ and $20$ benchmarks timeout for $\langle \RA, \CC \rangle$, $\langle \RC, \CC \rangle$, $\langle \texttt{true}, \CC \rangle$ and $\textsc{DFS}(\CC)$ respectively.}%In Figure~\ref{fig:results-memory} is deduced the minimum JPF's memory consumption ($256$ MB).
	%\caption{Comparing $\textsc{explore-ce}$ under $\CC$ and $\RA$ and $\textsc{explore-ce}^*$ under $\langle\RA, \CC\rangle, \langle\CC, \SI\rangle$ and $\langle\CC, \SER\rangle$. Client programs are ordered according to running time under $\RA$. The execution time of $\textsc{explore-ce}$ under $\CC$ is indistinguishable from the execution time of $\textsc{explore-ce}^*$ under $\langle\CC, \SI\rangle$ and $\langle\CC, \SER\rangle$.}
	\label{fig:results1}
\vspace{-4mm}
\end{figure}

%These are cactus plots. We start with a list of benchmark programs sorted by the running time (of our tool), and then plot the accumulated time for our tool on the first $i$-benchmarks in this list, for every $i$.

%One client has only one writing transaction per session while the second one has two writing transactions per session. 
 %for each application we have designed two programs with three threads each and three transactions per thread; where one contains only one transaction that writes per thread instead of the two writing transactions the second program have (in the case of TPC-C we discriminate transactions depending on the number of variables they write). 
To justify the benefits of partial order reduction, we implement a baseline model checking algorithm $\textsc{DFS}(\CC)$ that performs a standard DFS traversal of the execution tree w.r.t. the formal semantics defined in Section~\ref{ssec:semantics} for $\CC$ (for fairness, we restrict interleavings so at most one transaction is pending at a time). This baseline algorithm may explore the same history multiple times since it includes no partial order reduction mechanism. In terms of time, $\textsc{DFS}(\CC)$ behaves poorly: it timeouts for $20$ out of the $25$ programs and it is less efficient even when it terminates. We consider a timeout of $30$ mins. In comparison the strongly optimal algorithm $\textsc{explore-ce}(\CC)$ (under $\CC$) finishes in \oldver{$17$ seconds in average.}\nver{in $3' 26''$ seconds in average (counting timeouts).} $\textsc{DFS}(\CC)$ is \nver{similiar to $\textsc{explore-ce}(\CC)$}\oldver{also worse} in terms of memory consumption. The memory consumption of $\textsc{DFS}(\CC)$ is \oldver{$441$MB}\nver{$381$MB} in average, compared to \oldver{$317$MB}\nver{$508$MB} for $\textsc{explore-ce}(\CC)$ (JPF forces a minimum consumption of $256$MB).

To show the benefits of \emph{strong} optimality, we compare $\textsc{explore-ce}(\CC)$ which is strongly optimal with ``plain'' optimal algorithms $\textsc{explore-ce}^*(I_0,\CC)$ for different levels $I_0$. As shown in Figure~\ref{fig:results1}(a), $\textsc{explore-ce}(\CC)$ is more efficient time-wise than every ``plain'' optimal algorithm, and the difference in performance grows as $I_0$ becomes weaker. In the limit, when $I_0$ is the trivial isolation level $\texttt{true}$ where every history is consistent, $\textsc{explore-ce}^*(\texttt{true},\CC)$ timeouts for \nver{$20$}\oldver{$12$} out of the $25$ programs. The average speedup (average of individual speedups) of $\textsc{explore-ce}(\CC)$ w.r.t. $\textsc{explore-ce}^*(\RA,\CC)$, $\textsc{explore-ce}^*(\RC,\CC)$ and $\textsc{explore-ce}^*(\texttt{true},\CC)$ is \oldver{$2$, $31$, and $54$}\nver{$3$, $18$ and $15$.} respectively (we exclude timeout cases when computing speedups). All algorithms consume around \oldver{300 MB}\nver{$500$MB} of memory in average.


%\begin{table}[!ht]
%	\resizebox{\textwidth}{!}{
%    \centering
%
%	\begin{tabular}{c|c|c|c|c|c|c|c|}
%	\cline{2-8}
%	 & \CC     & \SI + \CC & \SER + \CC & \RA + \CC & \RC+ \CC   & \texttt{true} + \CC & \textsc{DFS}$(\CC)$  \\ \hline
%	\multicolumn{1}{|c|}{Avg. speedup}                        & 1      & 1     & 1      & 2       & 31       & 54        & 297      \\ \hline
%	\multicolumn{1}{|c|}{Avg. time (s)}    & 17     & 18      & 17       & 79      & 184      & 302       & 953      \\ \hline
%	\multicolumn{1}{|c|}{Avg. memory (MB)} & 317  & 335 & 332  & 339 & 332 & 341 & 441 \\ \hline
%	\multicolumn{1}{|c|}{Avg. histories ($\times 10^3$)} & 421.28 & 31.00   & 9.64     & 1746.52 & 25976.29 & 55789.54  & 68106.00 \\ \hline
%	\end{tabular}
%	}
%	\caption{Average speedup, time, memory and histories in the first experiment after excluding benchmarks that timeout.}
%\end{table}

For the $\SI$ and $\SER$ isolation levels that admit no strongly optimal $\textsc{explore}$ algorithm, we observe that the overhead of $\textsc{explore-ce}^*(\CC,\SI)$ or $\textsc{explore-ce}^*(\CC,\SER)$ relative to $\textsc{explore-ce}(\CC)$ is negligible (the corresponding lines in Figure~\ref{fig:results1} are essentially overlapping). This is due to the fact that the consistency checking algorithms of \citet{DBLP:journals/pacmpl/BiswasE19} are polynomial time when the number of sessions is fixed, which makes them fast at least on histories with few sessions.
 
%We test effective running time comparing $\textsc{explore-ce}$ under $\CC$ and $\textsc{explore-ce}^*$ under the pairs of isolation levels $\langle\CC, \SI\rangle$ and $\langle\CC, \SER\rangle$. In addition, we compare strong-optimality versus optimality running $\textsc{explore-ce}$ under $\CC$ and $\textsc{explore-ce}^*$ under the pairs of isolation levels $\langle\RA, \CC\rangle$, $\langle\RC, \CC\rangle$ and $\langle \texttt{true}, \CC\rangle$ (where $\texttt{true}$ is the isolation level under which every history is consistent). We compare both algorithms with a naive DFS algorithm that explores all possible transactions' interleavings under $\Rightarrow_I$ semantics, $\textsc{DFS}(\CC)$. It only allows a pending transaction at a time, all $\textsc{DFS}(\CC)$'s executions are $\CC$-consistent and there has not any incomplete execution (Theorem~\ref{theorem:causalExtensibleModels-CC-RA-RC}).
%The running times and number of histories are reported in Figure~\ref{fig:results1}. On one hand, the time complexity of $\textsc{explore-ce}^*$ is essentially determined by the underlying isolation level ($\CC$). On the other hand, the weaker the underlying with respect the tested isolation level, the worse the running time. In particular, $\textsc{explore-ce}$ under $\CC$ beats every competitor and no $\textsc{explore-ce}^*$ algorithm is beat by $\textsc{DFS}(\CC)$.

%As probably expected, $\textsc{explore-ce}^*$ under $(\RA, \CC)$ has a worse performance than $\textsc{explore-ce}$ under $\CC$ because of the time spent in enumerating histories which are $\RA$ but not $\CC$. As it can be seen in Figure~\ref{fig:results-histories} there is large gap between the number of $\RA$ and $\CC$ histories. 
%The time difference between $\textsc{explore-ce}(I_0)$ and $\textsc{explore-ce}^*(I_0,I)$ is insignificant. This is due to the fact that the consistency checking algorithms of \citet{DBLP:journals/pacmpl/BiswasE19} are polynomial time when the number of sessions is fixed, which makes them fast at least on histories with few sessions.

%We run $\textsc{explore-ce}$ for these programs under $\CC$, and $\textsc{explore-ce}^*$ under the pairs of isolation levels $\langle\CC, \SI\rangle$ and $\langle\CC, \SER\rangle$, $\langle\RA, \CC\rangle$, $\langle\RC, \CC\rangle$, $\langle \texttt{true}, \CC\rangle$ and DFS$(\CC)$. The running times and number of histories are reported in Figure~\ref{fig:results1}. As probably expected, $\textsc{explore-ce}^*$ under $(\RA, \CC)$ has a worse performance than $\textsc{explore-ce}$ under $\CC$ because of the time spent in enumerating histories which are $\RA$ but not $\CC$. As it can be seen in Figure~\ref{fig:results-histories} there is large gap between the number of $\RA$ and $\CC$ histories. The time difference between $\textsc{explore-ce}(I_0)$ and $\textsc{explore-ce}^*(I_0,I)$ is insignificant. This is due to the fact that the consistency checking algorithms of \citet{DBLP:journals/pacmpl/BiswasE19} are polynomial time when the number of sessions is fixed, which makes them fast at least on histories with few sessions.

%However, this is not anymore true for $\textsc{explore-ce}^*$ under $\langle\CC, \SI\rangle$ and $\langle\CC, \SER\rangle$. The difference w.r.t. $\textsc{explore-ce}$ under $\CC$ is insignificant. A possible explanation is that the difference between the number of $\RA$ histories and $\CC$ histories is significantly bigger than the difference between the number of $\CC$ histories and $\SI$/$\SER$ histories.

%number of $\CC$ histories is significantly smaller than $\RA$ histories, the cost of checking consistency with $\SI$ and $\SER$ in $\textsc{explore-ce}^*$ with $\langle\CC, \SI\rangle$ and $\langle\CC, \SER\rangle$. As $\CC$ is a causal-extensible model and it had a reasonable performance under this experiment, in the following we will work only with this isolation level.


%The results obtained in Figure~\ref{fig:results-ra-cc} show that an increment on the number of history a program may have under a concrete isolation level, obliges an increasing execution time. As expected, $\textsc{explore-ce}^*$ under $(\RA, \CC)$ have a worse performance than $\textsc{explore-ce}$ under $\CC$ by the cost of checking if a history satisfies $\CC$. However, as the number of $\CC$ histories is significantly smaller than $\RA$ histories, the cost of $\SI$ and $\SER$ checks is diluted. As $\CC$ is a causal-extensible model and it had a reasonable performance under this experiment, in the following we will work only with this isolation level.
% Moreover, it can be even worse than simply $\textsc{explore-ce}$ under $I_0$ if the $\evaluate$'s cost for isolation level $I$ is higher than the cost of checking if $h$ satisfies $I_0$. Moreover, as seen in Figure~\ref{fig:results-histories}, we notice that even for isolation levels with thousands of histories, the algorithm terminates in a reasonable time (no longer than one hour). As $\CC$ have a reasonable performance under this experiment, in the following we will work only with this isolation level.


% measures the algorithm's performance under $\CC$. We design three types of performance situations depending the number of shared variables a pair of transactions update; being ``Light'' a situation where every update is potentially read by only one thread, ``Heavy'' one where every update writes a variable every transaction reads and ``Medium'' something in between. For each of them, we describe five TPC-C programs, with a different number of threads each, between $1$ and $5$, with only one transaction per thread.

%writing transactions, and make them the same


%THREAD SCALABILITY




In our second experiment, we investigate the scalability of $\textsc{explore-ce}$ when increasing the number of sessions. For each $i\in [1,5]$, we consider 5 \nver{(independent)} client programs for TPC-C and 5 for Wikipedia\oldver{\footnote{We focus on these two applications because they are of similar complexity.}}
(10 in total) with $i$ sessions, each session containing 3 transactions. We start with 10 programs with 5 sessions, and remove sessions one by one to obtain programs with fewer sessions. We take $\CC$ as isolation level. 
%We take as benchmark five client programs for TPC-C and Wikipedia (10 in total) and $\CC$ as isolation level. 
%For each $i\in [1,5]$, we consider three clients per application with $i$ sessions, each containing three transactions. Starting with a client with $5$ sessions, we remove $5-i$ to obtain a client with $i$ sessions.
%Clients with less than five sessions are obtained by removing several sessions from a client with five sessions.  %Every client with $i$ sessions is obtained removing $5-i$ sessions satisfying every client with $i < 5$ sessions is a sub-client of a $i+1$ session client in our benchmark.
%of increasing levels of difficulty that we call light, medium, and heavy. For light clients, each session contains a different type of transaction, so the number of read/write interactions on the same variable is small. All sessions of a heavy client contain the same type of transaction in all sessions, and medium difficulty is an average of these two. 
The plot in Figure~\ref{fig:results-threads} shows average running time and memory consumption for each number $i\in [1,5]$ of sessions. 
As expected, increasing the number of sessions is a bottleneck running time wise because the number of histories increases significantly. However, memory consumption does not grow with the same trend, cf. the polynomial space bound.
%As expected, at least for ``heavy'' clients, increasing the number of sessions remains a bottleneck. This is expected also because the size of the output (number of histories) increases significantly as well.
%However, under the small-scope hypothesis, the systematic enumeration of \emph{all} executions of small clients enabled by our algorithms should suffice to uncover all potential bugs in an application. 

%In Figure~\ref{fig:results2} we can observe that, in general, the running time of this algorithm does not exceed the couple of minutes in almost every situation. Moreover, we point that the cost of swapping two events has a sensible impact on the overall performance.

\begin{figure}[t]
	\vspace{-4mm}
	\centering
	\begin{subfigure}[b]{0.322\linewidth}
		\centering
		\includegraphics[width=\textwidth]{figures/se-scala.eps}
		\vspace{-5mm}
		\caption{Increasing sessions.}
		%\caption{Execution time. For the last ``heavy'' client with 5 sessions, the running time  $20' 40''$ (out of the figure).}
		\label{fig:results-threads}
	\end{subfigure}
	\hspace{1cm}
	%\hfill
	\begin{subfigure}[b]{0.422\linewidth}
		\centering
		\includegraphics[width=0.76\textwidth]{figures/tr-scala.eps}
		\vspace{-1mm}
		\caption{Increasing transactions per session.}
		%\caption{Number of histories. For the last ``heavy'' client with 5 sessions, the number of histories $1296$.}
		\label{fig:results-transactions}
	\end{subfigure}
\vspace{-3.5mm}
	\caption{Evaluating the scalability of $\textsc{explore-ce}(\CC)$ for TPC-C and Wikipedia client programs when increasing their size. These plots include benchmarks that timeout ($30$ mins): $4$, $9$ and $10$ for $3$, $4$ and $5$ sessions respectively in Figure~\ref{fig:results-threads}, and $5$, $8$ and $10$ for $3$, $4$ and $5$ transactions per sessions respectively in Figure~\ref{fig:results-transactions}.}
	\label{fig:results2}
\vspace{-4mm}
\end{figure}

Finally, we evaluate the scalability of $\textsc{explore-ce}(\CC)$ when increasing the number of transactions per session. We consider 5 \nver{(independent)} TPC-C client programs and 5 \nver{(independent)} Wikipedia programs with $3$ sessions and $i$ transactions per session, for each $i\in [1,5]$. 
%As before, we remove $5-i$ transactions in each session of a client with $5$ transaction per thread to obtain our benchmarks. 
Figure~\ref{fig:results-transactions} shows average running time and memory consumption for each number $i\in [1,5]$ of transactions per session. Increasing the number of transactions per session is a bottleneck for the same reasons.
% consists on, fixed the number of threads per program, studying how the algorithm performance when those programs have different number of transactions. Analogously to the previous situation, we design three types of performance situations, ``Heavy'', ``Medium'' and ``Light''; and for each of them, we analyze five TPC-C programs with different number of transactions, from $1$ to $5$.

%The memory consumption in all these experiments fluctuates around $500$MB, taking into account that JPF forces a minimum consumption of $256$MB. There are no remarkable memory consumption variations between different isolation levels. There are slight grows in memory consumption when the number of histories increases. The particular implementation of each benchmark represent the most important source of memory consumption's variability.

%The results in Figure~\ref{fig:results3} supports our claims as the bigger the total space to explore, the greater the time it has to be consumed in the exploration.

==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/extending.tex <==
%!TEX root = main.tex
\subsection{Extending Histories According to An Oracle Order}\label{ssec:extensions}

%This order is encoded in the implementation of the NEXT function. For example, an oracle order could be defined by an order on session ids, so that whenever steps from multiple sessions are enabled, it prioritizes the session with the smaller id. The reorder steps in the algorithm will make it possible to explore interleavings that don't satisfy this order and ensure completeness. 

The function $\genericNext$ generates events representing database accesses to extend an execution, according to an \emph{arbitrary but fixed} order between the transactions in the program called \callout{oracle order}. 
%The version here presented employs as parameter the program to analyze along with a total order called \callout{oracle order} between its transactions. 
We assume that the oracle order, denoted by $<_{\ora}$, is consistent with the order between transactions in the same session of the program. The extension of $<_{\ora}$ to events is defined as expected. \nver{For example, assuming that each session has an id, an oracle order can be defined by an order on session ids along with the session order $\so$: transactions from sessions with smaller ids are considered first and the order between transactions in the same session follows $\so$.}

% and trivially extensible to events in a history, has to respect the order between transactions in the same session of the program. 
% order of the program (i.e. if $T \ [\so] \ T'$ then $T \leq_{\ora} T'$); forbidding executions any real processor would produce. This order will be constant during the whole algorithm's execution. 

$\genericNext$ returns a new event of the transaction that is not already completed and that is \emph{minimal} according to $<_{\ora}$. In more detail, if $j,e,\gamma$ is the output of $\genericNext(\prog, \hist_<, \locals)$, then either:
\vspace{-1mm}
\begin{itemize}
	\item the last transaction log $t$ of session $j$ (w.r.t. $\so$) in $\hist$ is pending, and $t$ is the smallest among pending transaction logs in $\hist$ w.r.t. $<_{\ora}$ 
	%(we assume a straightforward extension of the oracle order between transactions in the program to transaction logs in a history of the program),
	\item $\hist$ contains no pending transaction logs and the next transaction of sessions $j$ is the smallest among not yet started transactions in the program w.r.t. $<_{\ora}$.
	\vspace{-1mm}
\end{itemize}

%In addition, we assume the algorithm maintains a total order between the events in every history, called \callout{algorithm order} and denoted as $\leq_h$, as well as a function $\nextEvent$ that given a non-total history $h$ returns the next event to be added. In a nutshell, it returns the minimal event according to $\ora$ that is not in $h$, prioritizing those events in pending transactions. Formally:
%
%\begin{cframed}[pinegreen]
%	\begin{equation*}
%		\begin{array}{ccc}
%			\nextEvent(h) & \coloneqq & 
%			\left\{
%			\begin{array}{cc}
%				\min_{\ora}\{e \in \mathcal{E} \ | \ e \not\in h\} \cup \{\bot\} & \text{if } \not\exists T \text{ s.t. } \textsc{pending}_h(T) \\
%				\min_{\ora}\{e \in\mathcal{E} \setminus h \ | \ e \in \textsc{pending}_h(T) \} & \text{otherwise}
%			\end{array}
%			\right.
%		\end{array}
%	\end{equation*}
%\end{cframed}

%if there is an incomplete transaction, $\nextEvent(h)$ is the minimal event $e$ according to $\ora$ that is not in $h$ but $\ibegin(\tr(e)) \in h$.

%During this section we will present several approaches for finding a deterministic transactional model checker and we will show why STMC is the best among them. Every approach would be, in some particular sense, incremental; starting from an empty history and ``enlarging'' it, adding in each step new events and/or relations between them. For any fixed program, we will assume that no transaction enable/disable any other and that they are totally ordered by some relation $\ora$ called \textit{oracle order} that respects $\so$ (i.e. if $T \ [\so] \ T'$ then $T \ [\ora] \ T'$). Therefore, combining $\ora$ and $\po$ we can also say that the oracle order also enforces a total order between the events.

This implementation of $\genericNext$ is deterministic and it prioritizes the completion of pending transactions. The latter is useful to maintain the invariant that any history explored by the algorithm has at most one pending transaction. Preserving this invariant requires that the histories given as input to $\genericNext$ also have at most one pending transaction. This is discussed further when explaining the process of re-ordering events in Section~\ref{subsection:SwappingHistories}.
%Thanks to this function, we will be able to extend any history $h = \langle E, \so, \wro \rangle$ in a deterministic way. Moreover, by its definition, we observe that $\nextEvent$ always propose to complete pending transactions before starting new ones. Therefore, it is a reasonable candidate as $\genericNext$ function in a algorithm \ref{algorithm:algo-class} instance.

\begin{figure}[t]
	\centering
	\begin{subfigure}[b]{.32\textwidth}
\begin{adjustbox}{max width=\textwidth}
{
\begin{tabular}{c||c}
	\begin{lstlisting}[xleftmargin=5mm,basicstyle=\ttfamily\scriptsize,escapeinside={(*}{*)}, tabsize=1]
begin;
a = read((*x*));
if(a == 3)
	write((*$y$*),1);
commit
begin;
b = read((*x*));
c = read((*y*));
commit
\end{lstlisting} &
\begin{lstlisting}[xleftmargin=5mm,basicstyle=\ttfamily\scriptsize,escapeinside={(*}{*)}, tabsize=1]
begin;
d = read((*x*));
write((*$x$*),3);
commit
\end{lstlisting} 
\end{tabular}}
\end{adjustbox}
		
		
		\caption{Program \nver{(2 sessions)}.}
		\label{fig:oracle-order:prog}
	\end{subfigure}
\centering
\begin{subfigure}[b]{.31\textwidth}
	\resizebox{\textwidth}{!}{
		\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
			semithick, transform shape]
			\node[draw, rounded corners=2mm,outer sep=0] (t1) at (-3.5, 0) {\begin{tabular}{l} 
					\init
			\end{tabular}};
			
			\node[draw, rounded corners=2mm,outer sep=0, label={[font=\small]50:$t_1$}] (t2) at (-3.5, -2) {
				\begin{tabular}{l}
					$\rd{x}$\\
					{\pgfsetfillopacity{0.3}$\wrt{y}{1}$}						
			\end{tabular}};
			
			\node[draw, rounded corners=2mm,outer sep=0, label={[font=\small]50:$t_3$}] (t3) at (0, 0) {
				\begin{tabular}{l}
					$\rd{x}$ \\
					$\wrt{x}{3}$
			\end{tabular}};
			
			\node[draw, rounded corners=2mm,outer sep=0, opacity=0.3, label={[font=\small]50:$t_2$}] (t4) at (0, -2) {
				\begin{tabular}{l} 
					 $\rd{x}$ \\
					 $\rd{y}$
			\end{tabular}};
			
			\path (t1) edge[left] node[yshift=0,xshift=0] {$\ora$} (t2);
			\path (t4) edge[left] node[yshift=0,xshift=0] {$\ora$} (t3);
			\path (t1) edge[above] node[yshift=0,xshift=0] {$\wro$} (t3);
						
			\path (t2.north east) -- (t2.east) coordinate[pos=0.67] (t2or);
			\path (t2.south east) -- (t2.east) coordinate[pos=0.67] (t2so);
			\path (t4.south west) -- (t4.west) coordinate[pos=0.67] (t4so);
			\path (t4.north west) -- (t4.west) coordinate[pos=0.67] (t4or);
			
			
			\path (t2or) edge[above] node[yshift=0,xshift=0] {$\ora$} (t4or);
			\path [opacity=0.3](t2so) edge[below] node[yshift=0,xshift=0] {$\so$} (t4so);
			
			
			\path (t3.south west) edge[left] node[yshift=0,xshift=0] {$\wro$} (t2.north east);
			
			%\path (t3or) edge[left] node[yshift=0,xshift=0] {$\ora$} (t4or);
			%\path (t3so) edge[right] node[yshift=0,xshift=0] {$\wro$} (t4so);
		\end{tikzpicture}  
		
	}
	\caption{An incomplete history.}
	\label{fig:oracle_order:a}
\end{subfigure}
	\hspace{.5cm}
	\centering
	\begin{subfigure}[b]{.31\textwidth}
		\resizebox{\textwidth}{!}{
			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
				semithick, transform shape]
				\node[draw, rounded corners=2mm,outer sep=0] (t1) at (-3.5, 0) {\begin{tabular}{l} 
						\init
				\end{tabular}};
				
				\node[draw, rounded corners=2mm,outer sep=0, label={[font=\small]50:$t_1$}] (t2) at (-3.5, -2) {
					\begin{tabular}{l}
						$\rd{x}$\\
						$\wrt{y}{1}$					
				\end{tabular}};
				
				\node[draw, rounded corners=2mm,outer sep=0, label={[font=\small]50:$t_3$}] (t3) at (0, 0) {
					\begin{tabular}{l}
						$\rd{x}$ \\
						$\wrt{x}{3}$
				\end{tabular}};
				
				\node[draw, rounded corners=2mm,outer sep=0, opacity=0.3, label={[font=\small]50:$t_2$}] (t4) at (0, -2) {
					\begin{tabular}{l} 
						$\rd{x}$ \\
						$\rd{y}$
				\end{tabular}};
				
				\path (t1) edge[left] node[yshift=0,xshift=0] {$\ora$} (t2);
				\path (t4) edge[left] node[yshift=0,xshift=0] {$\ora$} (t3);
				\path (t1) edge[above] node[yshift=0,xshift=0] {$\wro$} (t3);
				
				\path (t2.north east) -- (t2.east) coordinate[pos=0.67] (t2or);
				\path (t2.south east) -- (t2.east) coordinate[pos=0.67] (t2so);
				\path (t4.south west) -- (t4.west) coordinate[pos=0.67] (t4so);
				\path (t4.north west) -- (t4.west) coordinate[pos=0.67] (t4or);
				
				
				\path (t2or) edge[above] node[yshift=0,xshift=0] {$\ora$} (t4or);
				\path [opacity=0.3](t2so) edge[below] node[yshift=0,xshift=0] {$\so$} (t4so);
				
				
				\path (t3.south west) edge[left] node[yshift=0,xshift=0] {$\wro$} (t2.north east);
				
				%\path (t3or) edge[left] node[yshift=0,xshift=0] {$\ora$} (t4or);
				%\path (t3so) edge[right] node[yshift=0,xshift=0] {$\wro$} (t4so);
			\end{tikzpicture}  
			
		}
		\caption{An extension.} % of a history using $\nextEvent$ function.}
		\label{fig:oracle_order:b}
	\end{subfigure}
	\vspace{-2mm}
	\caption{A program with two sessions (a), a history $h$ (b), and an extension of $h$ with an event returned by $\genericNext$ (c). 
%	and two histories, where $h$ is the former and the latter is $h \oplus \nextEvent(h)$. 
	The $\so$-edges from $\init$ to the other transactions are omitted for legibility. 
	We use edges labeled by $\ora$ to represent the oracle order $<_{\ora}$.
	Events in gray are not yet added to the history.}
	\label{fig:oracle_order}
	\vspace{-4mm}	
\end{figure}

For example, consider the program in Figure~\ref{fig:oracle-order:prog}, an oracle order which orders \oldver{all}\nver{the two} transactions \oldver{on}\nver{in} the left \nver{session} before the \nver{transaction in the} right \oldver{one}\nver{session}, and the history $h$ in Figure~\ref{fig:oracle_order:a}. Since the local state of the pending transaction on the left stores $3$ to the local variable $a$ (as a result of the previous $\erd{x}$ event) and the Boolean condition in \texttt{if} holds, $\genericNext$ will return the event $\wrt{y}{1}$ when called with $\hist$.
% history $h$ in Figure~\ref{fig:oracle_order:a}, as in the local state of the first thread, $d = 2$, the boolean condition in transaction $t_1$ is satisfied and the second database call ($\wrt{y}{1}$) can be executed. Thus, $\nextEvent(h)$ would return the event $\wrt{y}{1}$ as its transaction is pending.

\begin{figure}[t]

\begin{subfigure}[b]{.24\textwidth}
%	\resizebox{\textwidth}{!}{
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{c||c}
\begin{lstlisting}[xleftmargin=5mm,basicstyle=\ttfamily\scriptsize,escapeinside={(*}{*)}, tabsize=1]
begin;
write((*$x$*),1);
write((*$y$*),1);
commit
\end{lstlisting} & %a = read((*x*));
\begin{lstlisting}[xleftmargin=5mm,basicstyle=\ttfamily\scriptsize,escapeinside={(*}{*)}, tabsize=1]
begin;
a = read((*y*));
commit
begin;
b = read((*x*));
commit
\end{lstlisting} 
\end{tabular} 
\end{adjustbox}
%		}
\caption{Program \nver{(2 sessions)}.}
\label{fig:add_read:prog}
\end{subfigure}
\hspace{-2mm}
	\begin{subfigure}[b]{.253\textwidth}
		\resizebox{\textwidth}{!}{
			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
				semithick, transform shape]
				\node[draw, rounded corners=2mm,outer sep=0] (t1) at (-3, 0) {\begin{tabular}{l} $\init$\end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0] (t2) at (-3, -1.75) {\begin{tabular}{l} $\wrt{x}{1}$ \\ $\wrt{y}{1}$ \end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0] (t3) at (0, 0) {\begin{tabular}{l} $\rd{y}$\end{tabular}};
				\node[draw, rounded corners=2mm, outer sep=0, opacity=0.3] (t4) at (0, -1.75) {
					\begin{tabular}{l} 
					$\rd{x}$
				\end{tabular}};
				
				\path (t1.south east) -- (t1.east) coordinate[pos=0.67] (t1y);
				\path (t1.north east) -- (t1.east) coordinate[pos=0.67] (t1x);
				\path (t3.south west) -- (t3.west) coordinate[pos=0.67] (t3y);
				\path (t3.north west) -- (t3.west) coordinate[pos=0.67] (t3x);
				%\path (t1x) edge[above] node[yshift=0,xshift=0] {$\wro_x$} (t3x);
				\path (t1.east) edge[above] node[yshift=0,xshift=0] {$\so$} (t3.west);
				\path (t1.south) edge[above] node[left] {$\so$} (t2.north);
				\path (t2.north east) edge[above] node [yshift=2,xshift=0] {$\wro_y$} (t3.south west);
				\path[opacity=0.3] (t3.south) edge[below] node [right]{$\so$} (t4.north); %[yshift=0,xshift=0]
			\end{tikzpicture}  
			
		}
		\caption{Current history.}
		\label{fig:add_read:a}
	\end{subfigure}
	%\hspace{.5cm}
	\centering
	\begin{subfigure}[b]{.253\textwidth}
		\resizebox{\textwidth}{!}{
			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
				semithick, transform shape]
				\node[draw, rounded corners=2mm,outer sep=0] (t1) at (-3, 0) {\begin{tabular}{l} $\init$\end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0] (t2) at (-3, -1.75) {\begin{tabular}{l} $\wrt{x}{1}$ \\ $\wrt{y}{1}$ \end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0] (t3) at (0, 0) {\begin{tabular}{l} $\rd{y}$\end{tabular}};
				\node[draw, rounded corners=2mm, outer sep=0] (t4) at (0, -1.75) {
					\begin{tabular}{l} 
						$\rd{x}$
				\end{tabular}};
				
				\path (t1.south east) -- (t1.east) coordinate[pos=0.67] (t1y);
				\path (t1.north east) -- (t1.east) coordinate[pos=0.67] (t1x);
				\path (t3.south west) -- (t3.west) coordinate[pos=0.67] (t3y);
				\path (t3.north west) -- (t3.west) coordinate[pos=0.67] (t3x);
				%\path (t1x) edge[above] node[yshift=0,xshift=0] {$\wro_x$} (t3x);
				\path (t1.east) edge[above] node[yshift=0,xshift=0] {$\so$} (t3.west);
				\path (t1.south) edge[above] node[left] {$\so$} (t2.north);
				\path (t2.north east) edge[above] node [yshift=2,xshift=0] {$\wro_y$} (t3.south west);
				\path (t3.south) edge[below] node [right]{$\so$} (t4.north);
				\path (t2.east) edge[below] node [above]{$\wro_x$} (t4.west); %[yshift=0,xshift=0] %[yshift=0,xshift=0]
			\end{tikzpicture}  
			
		}
		\caption{One extension.}
		\label{fig:add_read:b}
	\end{subfigure}%\hspace{.5cm}
	\centering
	\begin{subfigure}[b]{.25\textwidth}
		\resizebox{\textwidth}{!}{
			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
				semithick, transform shape]
				\node[draw, rounded corners=2mm,outer sep=0] (t1) at (-3, 0) {\begin{tabular}{l} $\init$\end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0] (t2) at (-3, -1.75) {\begin{tabular}{l} $\wrt{x}{1}$ \\ $\wrt{y}{1}$ \end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0] (t3) at (0, 0) {\begin{tabular}{l} $\rd{y}$\end{tabular}};
				\node[draw, rounded corners=2mm, outer sep=0] (t4) at (0, -1.75) {
					\begin{tabular}{l} 
						$\rd{x}$
				\end{tabular}};
				
				\path (t1.south east) -- (t1.east) coordinate[pos=0.67] (t1y);
				\path (t1.north east) -- (t1.east) coordinate[pos=0.67] (t1x);
				\path (t3.south west) -- (t3.west) coordinate[pos=0.67] (t3y);
				\path (t3.north west) -- (t3.west) coordinate[pos=0.67] (t3x);
				%\path (t1x) edge[above] node[yshift=0,xshift=0] {$\wro_x$} (t3x);
				\path (t1.east) edge[above] node[yshift=0,xshift=0] {$\so$} (t3.west);
				\path (t1.south) edge[above] node[left] {$\so$} (t2.north);
				\path (t2.north east) edge[above] node [yshift=2,xshift=0] {$\wro_y$} (t3.south west);
				\path (t3.south) edge[below] node [right]{$\so$} (t4.north);
				\path (t1.south east) edge[below] node [yshift=6,xshift=-12]{$\wro_x$} (t4.north west); %[yshift=0,xshift=0] %[yshift=0,xshift=0]
			\end{tikzpicture}  
			
		}
		\caption{Another extension.}
		\label{fig:add_read:c}
	\end{subfigure}\hspace{.5cm}
	\vspace{-6mm}
	\caption{Extensions of a history by adding a $\iread$ event. Events in gray are not yet added to the history.}
	\label{fig:add_read}
	\vspace{-3mm}
	%\vspace{-3mm}
\end{figure}

%TODO REDO THE ABOVE FIGURE IN THE SPIRIT OF FIGURE \ref{fig:dead_branch}. MODIFY THE EXAMPLE SO ONE OF THE TWO CHOICES DOES NOT SATISFY SOME ISOLATION LEVEL, TO EXEMPLIFY THE USE OF $\genericValidWrites$.

According to Algorithm~\ref{algorithm:algo-class}, if the event returned by $\genericNext$ is not a read event, then it is simply added to the current history as the maximal element of the order $<$ (cf. the definition of $\oplus_j$ on ordered histories). If it is a read event, then adding this event may result in multiple histories depending on the chosen $\wro$ dependency. 
%
%The incremental process of obtaining histories with more information it is called \textit{extension}. In essence, given a history $h$ and an event $e \not\in h$, all possible graphs using these two elements must be constructed. 
%If $e$'s type is $\ibegin$ or $\iend$, there is only one possible way to extend it by the operator $\bullet$'s definition. When $e$ is a $\iread$, however, we have to explore multiple histories, one per $\wro$-dependency that can be generated with a $\iwrite$ event $w\in h$ and $e$. That is, all histories $h \bullet_w e$. 
For example, in Figure \ref{fig:add_read}, extending the history in Figure \ref{fig:add_read:a} with the $\erd{x}$ event could result in two different histories, pictured in Figure \ref{fig:add_read:b} and \ref{fig:add_read:c}, depending on the write with whom this read event is associated by $\wro$. However, under $\CC$, the latter history is inconsistent.
%we can obtain two different histories depending on the $\wro$ dependency created (figures \ref{fig:add_read:b} and \ref{fig:add_read:c}). In both three cases, we declare the algorithm order for this new history $h'$ by simply juxtaposing $e$ to all the previous ones: $\leq_{h'} = \leq_h \cup \{\langle e', e \rangle \ | \  e' \in h\}$.
The function $\genericValidWrites$ limits the choices to those that preserve consistency with the intended isolation level $I$, i.e.,
%However, we will only select those $\iwrite$ event such that the extended history $h \bullet_w e$ is consistent, as described by function $\validWrites$; which will eventually play the $\genericValidWrites$'s role in our algorithm.  
\begin{align*}
\genericValidWrites(h, e) \coloneqq  \{t \ \in \transC{h} \ | \ h \oplus_j e \oplus \wro(t,e) \mbox{ satisfies }I\}
\end{align*}
where $\transC{h}$ is the set of committed transactions in $h$.

%Finally, we declare the function $\evaluate$ that detects when a history is total.
%
%\begin{cframed}[pinegreen]
%	\begin{equation*}
%		\begin{array}{ccc}
%			\evaluate(h) & \coloneqq & \nextEvent(h) = \bot
%		\end{array}
%	\end{equation*}
%\end{cframed}

%Nevertheless, we will guarantee in both cases that every possible incomplete history will be $\so$-bounded, i.e. if $e \ [\so \cup \po]^+ e'$ and $e' \in h$ then $e \in h$; in order to easily avoid eventual inconsistencies. Therefore, the global order $\ora$ presented in Figure~\ref{fig:oracle_order:a} restrict in a simple but effective way the duplicity between histories: the order events are being added don't cause \textit{per se} redundancies.%In the second case, to avoid randomness, we will have a function $\nextEvent$ that given a history $h$ returns the first event $e$ according to $\ora$ that is not in $h$; to obtain the new history $h' = h \bullet e$. For example, given the history in Figure~\ref{fig:oracle_order:b}, the function $\nextEvent$ would return the event $\ibegin$ associated to the second transaction. Nevertheless, we will guarantee in both cases that every possible incomplete history will be $\so$-bounded, i.e. if $e \ [\so \cup \po]^+ e'$ and $e' \in h$ then $e \in h$; in order to easily avoid eventual inconsistencies. Therefore, the global order $\ora$ presented in Figure~\ref{fig:oracle_order:a} restrict in a simple but effective way the duplicity between histories: the order events are being added don't cause \textit{per se} redundancies.

%Thanks to $\so$ and $\ora$ order, we will be able to track every possible history, and therefore, have control over the amount of graphs generated. 

%Incomplete histories can be extended in two ways: either with the extern help of some guide that select beforehand which events and in which order will be executed or without it. For managing the second case in a deterministic way, we will have a function $\nextEvent$ that maps every $h$ to some event that is not in $h$ for obtaining a new history $h' = h \bullet e$. If $h$ is incomplete and $l = \last{h}$ then $e$ is the minimum event in $\po_T$ bigger than $l$; but if not, $e$ is the $\ibegin$ event belonging to the minimal transaction $T$ according to $\ora$ that is not in $h$. For example, the function $\nextEvent$ would the history in Figure~\ref{fig:oracle_order:b} to the event $d \gets \rd{y}$. Clearly, any coherent history can be extended using $\nextEvent$ function resulting in a coherent history (as $\ora$ extends $\so$, it only suffices defining the $\wro$ edge that an eventual free $\iread$ would require).
%Nevertheless, we will guarantee in both cases that every possible incomplete history will be $\so$-bounded, i.e. if $e \ [\so \cup \po]^+ e'$ and $e' \in h$ then $e \in h$; in order to easily avoid eventual inconsistencies. Therefore, the global order $\ora$ presented in Figure~\ref{fig:oracle_order:a} restrict in a simple but effective way the duplicity between histories: the order events are being added don't cause \textit{per se} redundancies.%In the second case, to avoid randomness, we will have a function $\nextEvent$ that given a history $h$ returns the first event $e$ according to $\ora$ that is not in $h$; to obtain the new history $h' = h \bullet e$. For example, given the history in Figure~\ref{fig:oracle_order:b}, the function $\nextEvent$ would return the event $\ibegin$ associated to the second transaction. Nevertheless, we will guarantee in both cases that every possible incomplete history will be $\so$-bounded, i.e. if $e \ [\so \cup \po]^+ e'$ and $e' \in h$ then $e \in h$; in order to easily avoid eventual inconsistencies. Therefore, the global order $\ora$ presented in Figure~\ref{fig:oracle_order:a} restrict in a simple but effective way the duplicity between histories: the order events are being added don't cause \textit{per se} redundancies.

==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/implementation.tex <==
\section{Implementation}

We implemented algorithm $\textsc{explore-ce}$ and $\textsc{explore-ce}^*$ on top of Java PathFinder (JPF) \textcolor{red}{cite JPF}, a verification tool for Java concurrent programs. We admit as input a Java program that (1) can be parsed and executed by JPF and (2) employs the API according to the specifications. Our tool is parametric in the isolation levels employed.

The API provided allow $\ibegin, \iwrite, \iread$ and $\icommit$ operations. Thanks to this API, we can maintain the database state separately from JPF's internal state and update the current history in each database call. We do not rely on any concrete database but store the information as a collection of String, one per write API call executed; along with the $\so$, $\wro$-dependencies between the events associated to them. Any time there is a need to connect data from the local state to the database one or viceversa we copy and store the concrete String value from one state to the other. %Altogether, we are able to simulate from simple variables to actual tables provided the client has proper methods to transform from one to the other representative.

Our implementation is compatible with JPF's standards, as both algorithm are instances of DFSearch; a JPF for DFS exploring algorithms. Moreover, we built consistency checkers based on the algorithm's presented in \textcolor{red}{Ranadeep and Enea's paper} for different isolation levels to ensure database's soundness. 

However, for performance issues, we developed an iterative version of the algorithm \ref{algorithm:algo-class} for reducing the actual memory consumption. We employ an annotated stack of database states that is modified in each $\textsc{explore-ce}$ call; and we consider the algorithm works with list instead of simply sets.
At every step where we execute a $\iread$, we annotate which $\iwrite$ event is reading from and  when the state pops from the stack, we change the $\wro$-dependency. Analogously, at every step we produce a swap, we annotate which tuple given by $\compute$ we used in the swap for selecting a different tuple when the state is popped out. % In addition, as JPF is not designed for supporting database operations, we developed an API that simulates every database instruction. operations, but they have been proved expressive enough both during our experiments and in real time applications. We admit any Java program that (1) can be parsed and executed by JPF and (2) has an equivalent translation into a program written with the syntax defined in Figure~\ref{fig:syntax}.



==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/intro.tex <==
%!TEX root = main.tex
\section{Introduction}
\label{sec:intro}

Data storage is no longer about writing data to a single
disk with a single point of access. Modern applications require not just data
reliability, but also high-throughput concurrent accesses. 
Applications concerning supply chains, banking, etc. use traditional relational databases
for storing and processing data, whereas applications such as social networking
software and e-commerce platforms 
use cloud-based storage systems (such as Azure Cosmos DB \cite{cosmosdb}, Amazon DynamoDB
\cite{decandia2007dynamo}, Facebook TAO \cite{facebook-tao}, etc.). 
%We use the term \textit{storage system} in this paper to refer to any such database system or service.


%As applications have moved from a single-box environment to the cloud, the notion of
%data persistence has also changed. It is no longer about storing data on a
%single disk with a single point of access. Rather, modern applications such as
%social networking software, e-commerce platforms, cloud micro-services, etc. are built using 
%high-scale storage systems, such as Azure CosmosDb \cite{cosmosdb}, Amazon DynamoDb \cite{amazon-dynamodb}, 
%Facebook TAO \cite{facebook-tao}. Applications such as 
 
%These storage systems, commonly offered by most major cloud providers (such as
%Azure CosmosDb \cite{cosmosdb}, Amazon DynamoDb \cite{amazon-dynamodb}, 
%Facebook TAO \cite{facebook-tao}, etc.)
%create and manage multiple replicas of data. Having multiple replicas offers reliability and prevents
%data loss, but it also offers availability and low-latency accesses by allowing
%different clients to connect with different replicas. 

Providing high-throughput processing, unfortunately, comes at an unavoidable cost of weakening 
the consistency guarantees offered to users:
Concurrently-connected clients may end up observing different versions of the same data. 
These ``anomalies'' can be prevented by using a strong \textit{isolation level} 
such as \textit{Serializability} \cite{DBLP:journals/jacm/Papadimitriou79b}, which essentially offers a single version of the data to all clients at any point in time. 
However, serializability requires expensive synchronization and incurs a high performance cost. As a
consequence, most storage systems use weaker isolation levels, such as 
{\it Causal Consistency}~\cite{DBLP:journals/cacm/Lamport78,DBLP:conf/sosp/LloydFKA11,antidote},
{\it Snapshot Isolation}~\cite{DBLP:conf/sigmod/BerensonBGMOO95}, {\it Read
Committed}~\cite{DBLP:conf/sigmod/BerensonBGMOO95}, etc. for better performance.
In a recent survey of
database administrators \cite{survey}, 86\% of the participants responded that
most or all of the transactions in their databases execute at Read Committed level.

A weaker isolation level allows for more possible behaviors than stronger
isolation levels. It is up to the developers then to ensure that their
application can tolerate this larger set of behaviors. Unfortunately, weak
isolation levels are hard to understand or reason about
\cite{DBLP:conf/popl/BrutschyD0V17,adya-thesis} and resulting application bugs
can cause loss of business \cite{acidrain}.

\vspace{.5mm}
\noindent
\textbf{Model Checking Database-Backed Applications.}
This paper addresses the problem of \textit{model checking} code for correctness against a given isolation level. %against weak behaviors: a developer should be able to write a test that runs
%their application and then asserts for correct behavior. 
%The main difficulty with testing today is getting coverage of weak behaviors.
\emph{Model checking}~\cite{DBLP:conf/popl/ClarkeES83,DBLP:conf/programm/QueilleS82} explores the state space of a given program in a systematic manner and it provides high coverage of program behavior. However, it faces the infamous state explosion problem, i.e., the number of executions grows exponentially in the number of concurrent clients. 
%In this paper, we consider shared-memory programs running on a sequentially consistent memory model, for which interleavings of atomic steps in different threads are a precise model of concrete executions.

%(called a Mazurkiewicz trace~\cite{DBLP:conf/ac/Mazurkiewicz86})

\emph{Partial order reduction} (POR)~\cite{DBLP:journals/sttt/ClarkeGMP99,DBLP:books/sp/Godefroid96,DBLP:conf/cav/Peled93,DBLP:conf/apn/Valmari89} is an approach that limits the number of explored executions without sacrificing coverage. POR relies on an equivalence relation between executions where e.g., two executions are equivalent if one can be obtained from the other by swapping consecutive independent (non-conflicting) execution steps. It guarantees that at least one execution from each equivalence class is explored. \emph{Optimal} POR techniques explore exactly one execution from each equivalence class. Beyond this classic notion of optimality, POR techniques may aim for optimality by avoiding visiting states from which \nver{the exploration is blocked}. 
%
{\em Dynamic} partial order reduction (DPOR)~\cite{DBLP:conf/popl/FlanaganG05} has been introduced to explore the execution space (and tracking the equivalence relation between executions) on-the-fly without relying on a-priori static analyses. This is typically coupled with \emph{stateless} model checking (SMC)~\cite{DBLP:conf/popl/Godefroid97} which explores executions of a program without storing visited states, thereby, avoiding excessive memory consumption. 

There is a large body of work on (D)POR techniques that address their soundness when checking a certain class of specifications for a certain class of programs, as well as their completeness and their theoretical optimality (see Section~\ref{sec:related}). Most often these works consider shared memory concurrent programs executing under a strongly consistent memory model. 
%The set of interleavings explored by some POR technique is defined by restricting the set of threads that are explored from each state (scheduling point). Depending on the class specifications, assumptions about programs, or optimality targets, there are various definitions for this set of processes, including stubborn sets~\cite{DBLP:conf/apn/Valmari89}, persistent sets~\cite{DBLP:books/sp/Godefroid96}, ample sets~\cite{DBLP:journals/sttt/ClarkeGMP99}, and source sets~\cite{DBLP:journals/jacm/AbdullaAJS17}.

In the last few years, some works have studied DPOR in the case of shared memory programs running under weak memory models such as TSO or Release-Acquire, e.g.~\cite{DBLP:conf/cav/AbdullaAJL16,DBLP:journals/acta/AbdullaAAJLS17,DBLP:journals/pacmpl/AbdullaAJN18,DBLP:conf/pldi/Kokologiannakis19}. While these algorithms are sound and complete, they have exponential space complexity when they are optimal. 
% In \cite{DBLP:journals/acta/AbdullaAAJLS17}, the authors define a DPOR algorithm for programs running under the TSO weak memory model. While this algorithm is sound, complete, and optimal, it has an exponential memory complexity. 
More recently, \citet{DBLP:journals/pacmpl/Kokologiannakis22} defined a DPOR algorithm that has a polynomial space complexity, in addition of being sound, complete and optimal. This algorithm can be applied for a range of shared memory models. % assuming that checking conformance for finite computations.   
%

While the works mentioned above concern shared memory programs, we are not aware of any published work addressing the case of database transactional programs running under weak isolation levels. In this paper, we address this case and propose new stateless model checking algorithms relying on DPOR techniques for database-backed applications.  \nver{We assume that all the transactions in an application execute under the \emph{same} isolation level, which happens quite frequently in practice (as mentioned above, most database applications are run on the default isolation level of the database).}
Our work generalizes the approach introduced by \cite{DBLP:journals/pacmpl/Kokologiannakis22}. However, this generalization to the transactional case, covering the most relevant isolation levels, is not a straightforward adaptation of \cite{DBLP:journals/pacmpl/Kokologiannakis22}. Ensuring optimality while preserving the other properties, e.g., completeness and polynomial memory complexity, is very challenging.
 %\nver{even under the assumption of a unique isolation level during the whole execution}. 
Next, we explain the main steps and features of our work.  

\vspace{.5mm}
\noindent
\textbf{Formalizing Isolation Levels.}
Our algorithms rely on the axiomatic definitions of isolation
levels introduced by \citet{DBLP:journals/pacmpl/BiswasE19}. These
definitions use logical constraints called \emph{axioms} to characterize the
set of executions of a database (e.g., key-value store) that conform to a particular isolation
level (extensible to SQL queries~\citep{DBLP:journals/pacmpl/BiswasKVEL21}). These constraints refer to a specific set of
relations between events/transactions in an execution that describe control-flow
or data-flow dependencies: a program order $\po$ between events in the same
transaction, a session order $\so$ between transactions in the same session\footnote{A
session is a sequential interface to the storage system. It corresponds to what
is also called a \textit{connection}.}, and a write-read $\wro$ (read-from) relation that
associates each read event with a transaction that writes the value returned by
the read. These relations along with the events in an
execution are called a \emph{history}. 
A history describes only the
interaction with the database, omitting application-side events (e.g., computing
values written to the database). 

\vspace{.5mm}
\noindent
\textbf{Execution Equivalence.} DPOR algorithms are parametrized by an equivalence relation on executions, most often, Mazurkiewicz equivalence~\cite{DBLP:conf/ac/Mazurkiewicz86}. In this work, we consider a weaker equivalence relation, also known as \emph{read-from equivalence}~\cite{DBLP:journals/pacmpl/ChalupaCPSV18,DBLP:journals/pacmpl/AbdullaAJN18,DBLP:journals/pacmpl/AbdullaAJLNS19,DBLP:conf/pldi/Kokologiannakis19,DBLP:conf/asplos/Kokologiannakis20,DBLP:journals/pacmpl/Kokologiannakis22}, which considers that two executions are equivalent when their histories are precisely the same (they contain the same set of events, and the relations $\po$, $\so$, and $\wro$ are the same). 
In general, reads-from equivalence is coarser than Mazurkiewicz equivalence, and its equivalence classes can be exponentially-smaller than Mazurkiewicz traces in certain cases~\cite{DBLP:journals/pacmpl/ChalupaCPSV18}.

\vspace{.5mm}
\noindent
\textbf{SMC Algorithms.}
Our SMC algorithms enumerate executions of a given program under a given isolation level $I$. They are \emph{sound}, i.e., enumerate only \emph{feasible} executions (admitted by the program under $I$), \emph{complete}, i.e., they output a representative of each read-from equivalence class, and \emph{optimal}, i.e., they output \emph{exactly one} complete execution from each read-from equivalence class.
%producing \emph{exactly one} representative from each read-from equivalence class. 
For isolation levels weaker than and including Causal Consistency, they satisfy a notion of \emph{strong optimality} which says that additionally, the enumeration avoids states from which the execution is ``blocked'', i.e., it cannot be extended to a complete execution of the program. 
%This goes beyond the more standard notion of optimality which requires that the algorithm produces exactly one \emph{complete} execution from each equivalence class.
For Snapshot Isolation and Serializability, we show that \emph{there exists} no algorithm in the same class (to be discussed below) that can ensure such a strong notion of optimality. All the algorithms that we propose are polynomial space, as opposed to many DPOR algorithms introduced in the literature.

As a starting point, we define a generic class of SMC algorithms, called \emph{swapping based}, generalizing the approach adopted by \citep{DBLP:conf/pldi/Kokologiannakis19,DBLP:journals/pacmpl/Kokologiannakis22}, which enumerate histories of program executions. These algorithms focus on the interaction with the database assuming that 
%track the history of an execution, i.e., the interaction with the database. We assume that 
the other steps in a transaction concern local variables visible only within the scope of the enclosing session.  Executions are extended according to a generic scheduler function $\genericNext$ and every read event produces several exploration branches, one for every write executed in the past that it can read from. Events in an execution can be swapped to produce new exploration ``roots'' that lead to different histories. Swapping events is required for completeness, to enumerate histories where a read $r$ reads from a write $w$ that is scheduled by $\genericNext$ after $r$. To ensure soundness, we restrict the definition of swapping so that it produces a history that is feasible by construction (extending an execution which is possibly infeasible may violate soundness). Such an algorithm is optimal w.r.t. the read-from equivalence when it enumerates each history exactly once. 

We define a concrete algorithm in this class that in particular, satisfies the stronger notion of optimality mentioned above for every isolation level $I$ which is \emph{prefix-closed} and \emph{causally-extensible}, e.g.,  {\it Read Committed} and \textit{Causal Consistency}. Prefix-closure means that every prefix of a history that satisfies $I$, i.e., a subset of transactions and all their predecessors in the causal relation, i.e., $(\so\cup\wro)^+$, is also consistent with $I$, and causal extensibility means that any pending transaction in a history that satisfies $I$ can be extended with one more event to still satisfy $I$, and if this is a read event, then, it can read-from a transaction that precedes it in the causal relation. To ensure strong optimality, this algorithm uses a carefully chosen condition for restricting the application of event swaps, which makes the proof of completeness in particular, quite non-trivial.

We show that isolation levels such as Snapshot Isolation and Serializability are \emph{not} causally-extensible and that there exists no swapping based SMC algorithm which is sound, complete, and strongly optimal at the same time (independent of memory consumption bounds). This impossibility proof uses a program to show that any $\genericNext$ scheduler and any restriction on swaps would violate either completeness or strong optimality. However, we define an extension of the previous algorithm which satisfies the weaker notion of optimality, while preserving soundness, completeness, and polynomial space complexity. This algorithm will simply enumerate executions according to a weaker prefix-closed and causally-extensible isolation level, and filter executions according to the stronger isolation levels Snapshot Isolation and Serializability at the end, before outputting.

We implemented these algorithms in the Java Pathfinder (JPF) model checker~\cite{DBLP:conf/issta/VisserPK04}, and evaluated them on a number of challenging database-backed applications drawn from the literature of distributed systems and databases.  

Our contributions and outline are summarized as follows:
\vspace{-1mm}
\begin{itemize}
	\item[\S~\ref{sec:props}] identifies a class of isolation levels called prefix-closed and causally-extensible that admit efficient SMC.
	\item[\S~\ref{sec:algs}] defines a generic class of swapping based SMC algorithms based on DPOR which are parametrized by a given isolation level.
	\item[\S~\ref{sec:CC-algorithm}] defines a swapping based SMC algorithm which is sound, complete, strongly-optimal, and polynomial space, for any isolation level that is prefix-closed and causally-extensible.
	\item[\S~\ref{sec:ser}] shows that there exists no swapping based algorithm for Snapshot Isolation and Serializability, which is sound, complete, and strongly-optimal at the same time, and proposes a swapping based algorithm which satisfies ``plain'' optimality. % (along with soundness, completeness, and polynomial space complexity bounds).
	\item[\S~\ref{sec:exp}] reports on an implementation and evaluation of these algorithms. % in the context of a number of interesting case studies.
\vspace{-1mm}
\end{itemize}

Section~\ref{sec:prelims} recalls the formalization of isolation levels of Biswas and Enea~\cite{DBLP:journals/pacmpl/BiswasE19,DBLP:journals/pacmpl/BiswasKVEL21}, while Sections~\ref{sec:related} and~\ref{sec:conc} conclude with a discussion of related work and concluding remarks. \nver{Additional formalization, proofs, and experimental data can be found in the technical report~\cite{bouajjani2023dynamic}.}


%========
%
%
%Programming paradigm is in constant evolution, sequential programs tend to easily become obsolete because of its slow performance and even concurrent programs can also be inefficient when the memory requirements increase. The current state-of-the-art tries to overcome those problems by developing parallel programs along with distributed storage systems. However, not every type of application has the same data reliability requirements and therefore developers may want to relax the \textit{isolation level}, i.e. the restrictions imposed to the information stored for guaranteeing consistency, from the database in order to increase performance.
%
%Allowing multiple behaviors in these contexts hinder the already difficult task of verifying concurrent programs. Studying every alternative is something unrealistic, as the number of possible scenarios grows exponentially with the length of the programs. In general, formal methods such as \textcolor{red}{cite examples} are a reasonable approach as they provide certificate of correctness and explainability of the bugs otherwise. Among them, \textit{stateless model checking} (SMC) and \textit{dynamic partial order reduction} (DPOR) \textcolor{red}{cite papers} stand out as the most promising techniques for verifying current programs during the recent years \textcolor{red}{cite papers}.
%
%On one hand, for a given length-bounded program, SMC explores systematically every possible execution without storing at any point the set of already visited ones. On the other hand, DPOR resumes every possible behavior in a more succinct way, reducing the number of executions that have to be explored for covering those behaviors. Henceforth, combining both techniques to obtaining sound, complete and efficient algorithms has been one of the aimed goals in this field and it has been successfully done for concurrent programs with shared memory \textcolor{red}{cite papers}.
%
%Despite their popularity, there is no application of such techniques in parallel programming with distributed memory's literature so far, hence the relevance of filling this gap. Nevertheless, part of the path this paper wants to create is already explored, as shared memory models are not that unrelated with distributed database's. For example, we can mention the relation between \textit{sequential consistency} and \textit{serializability} or \textit{strong release-acquire} and \textit{causal consistency}; where both database isolation level cases are nothing but a generalization of their shared memory counterparts \textcolor{red}{cite papers}.
%
%In this paper, we present STMC, a \textit{sound}, \textit{complete}, \textit{optimal} DPOR algorithm with \textit{linear memory requirements} that employs SMC techniques for verifying some isolation levels. We describe the models that can guarantee those properties, show that \textit{causal consistency} ($\CC$), \textit{read atomic} ($\RA$) and \textit{read committed} ($\RC$) satisfy them and present an example of why more complex models such as \textit{serializability} ($\SER$) cannot be verified with our algorithm. We also present a formal semantics for STMC and exhibit how it evolves from the base algorithm to its current state; requiring executing transactions in isolation and swapping complete blocks of transactions. In addition, we provide some proofs to help the reader having a better understanding of STMC.
%
%On top of this theoretical development, we also furnish this work with an implementation using Java and several benchmarks that study its re. In a nutshell, our software is an extension of JPF \textcolor{red}{cite tool}, a Java-built software analysis framework for Java (parallel) programs. It provides control to DFS traversal of executions, which along its modularity, makes it an ideal tool for developing and extending a database concurrent programs' verifier. In particular, we highlight the easiness for splitting the program memory and database's management and providing an API for writing the programs to analyze. 
%%Our work doesn't finish with the theoretical aspects, as we also furnish this paper with an implementation in Java. In a nutshell, it is an extension of JPF \textcolor{red}{cite tool}, a Java 

%we start from the base algorithm presented in \textcolor{red}{cite Viktor's algorithm} and adapt it to some concrete isolation levels while maintaining its properties  In particular, we describe the properties any model has to ensure for 

%Data storage is no longer about writing data to a single disk with a single point of access. Modern applications require not just data reliability, but also high-throughput concurrent accesses. Applications concerning supply chains, banking, etc. use traditional relational databases for storing and processing data, whereas applications such as social networking software and e-commerce platforms use cloud-based storage systems (such as Azure Cosmos DB \cite{cosmosdb}, Amazon DynamoDB \cite{decandia2007dynamo}, Facebook TAO \cite{facebook-tao}, etc.). We use the term \textit{storage system} in this paper to refer to any such database system or service.

%Providing high-throughput processing, unfortunately, comes at an unavoidable cost of weakening the guarantees offered to users. Concurrently-connected clients may end up observing different views of the same data. These ``anomalies'' can be prevented by using a strong \textit{isolation level} such as \textit{serializability} \cite{DBLP:journals/jacm/Papadimitriou79b}, which essentially offers a single view of the data. However, serializability requires expensive synchronization and incurs a high performance cost. As a consequence, most storage systems use weaker isolation levels, such as {\it Causal Consistency}~\cite{DBLP:journals/cacm/Lamport78,DBLP:conf/sosp/LloydFKA11,antidote}, {\it Snapshot Isolation}~\cite{DBLP:conf/sigmod/BerensonBGMOO95}, {\it Read Committed}~\cite{DBLP:conf/sigmod/BerensonBGMOO95}, etc. for better performance. In a recent survey of database administrators \cite{survey}, 86\% of the participants responded that most or all of the transactions in their databases execute at Read Committed isolation level.


==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/programs.tex <==
%!TEX root = main.tex
\section{Transactional Programs}\label{sec:prelims}

\subsection{Program Syntax}
\begin{figure}
\vspace{-4mm}
\small
\begin{align*}
\key\in \Vars\quad \xvar\in\LVars
\end{align*}
\begin{minipage}[t]{.4\textwidth}
\vspace{-4mm}
\begin{align*}
\mathsf{Prog} &  \eqdef  \mathsf{Sess} \ \mid\  \mathsf{Sess}\,||\,\mathsf{Prog} \\
\mathsf{Sess} & \eqdef  \mathsf{Trans} \ \mid\  \mathsf{Trans}; \mathsf{Sess} \\
\mathsf{Trans} & \eqdef  \ibegin; \mathsf{Body}; \icommit\\
\end{align*}
\end{minipage}
\begin{minipage}[t]{.4\textwidth}
\vspace{-4mm}
\begin{align*}
\mathsf{Body} & \eqdef  \mathsf{Instr} \ \mid\  \mathsf{Instr}; \mathsf{Body} \\
\mathsf{Instr} & \eqdef  \mathsf{InstrDB} \ \mid\  a := e \mid\ \iif{\phi(\vec{a})}{\mathsf{Instr}} \\
\mathsf{InstrDB} & \eqdef \xvar := \iread(\key)  \ \mid\  \iwrite(\key,\xvar) \ \mid \ \iabort
%\mathsf{Local} & \eqdef  x := e
\end{align*}
\end{minipage}
\vspace{-7mm}
\caption{Program syntax. The set of global variables is denoted by $\Vars$ while $\LVars$ denotes the set of local variables.
We use $\phi$ to denote Boolean expressions over local variables, and $e$ to denote expressions over local variables interpreted as values. We use $\vec{\cdot}$ to denote vectors of elements.}
\label{fig:syntax}
\vspace{-8mm}
\end{figure}

Figure~\ref{fig:syntax} lists the definition of a simple programming language
that we use to represent applications running on top of a database. A program is a set of \emph{sessions} running in parallel, each
session being composed of a sequence of \emph{transactions}. Each transaction is
delimited by $\ibegin$ and either $\icommit$ or $\iabort$ instructions, 
%\footnote{We do not consider involuntary aborts, i.e. aborts caused by the particular implementation of the database.},
 and its body contains instructions that access the
database and manipulate a set $\LVars$ of local variables. 
We use symbols $a$, $b$, etc. to denote elements of $\LVars$.

For simplicity, we abstract the database state as a valuation to a set $\Vars$ of \emph{global} variables\footnote{In the context of a relational database, global variables correspond to fields/rows of a table while in the context of a key-value store, they correspond to keys.}, ranged over using $x$, $y$, etc. The instructions accessing the database correspond to reading the value of a global variable and storing it into a local variable $a$ ($a := \iread(x)$) , writing the value of a local variable $a$ to a global variable $x$ ($\iwrite(x,a)$), or an assignment to a local variable $a$ ($a := e$). The set of values of global or local variables is denoted by $\Vals$. Assignments to local variables use expressions $e$ over local variables, which are interpreted as values and whose syntax is left unspecified. Each of these instructions can be guarded by a Boolean condition $\phi(\vec{a})$ over a set of local variables $\vec{a}$ (their syntax is not important). Our results assume bounded programs, as usual in SMC algorithms, and therefore, we omit other constructs like $\mathtt{while}$ loops. 
SQL statements (SELECT, JOIN, UPDATE) manipulating relational tables can be compiled to reads or writes of variables representing rows in a table (see for instance,~\cite{DBLP:journals/pacmpl/RahmaniNDJ19,DBLP:journals/pacmpl/BiswasKVEL21}). 
%\nver{Our work focuses on the problem of enumerating interleavings of reads and write "effects" from different transactions, modeled as reads and write of a set of global variables, and the issue of translating SQL statements to such reads and writes (which is prevalent in concurrency control mechanisms as well) is beyond the scope of our paper.} 
%\nver{SQL tables are modelled by a ``set'' variable whose content is the set of ids (primary keys) of the rows present in the table. SQL statements such as INSERT and DELETE statements are modelled as writes on that set variable while SQL statements with a WHERE clause (SELECT, JOIN, UPDATE) can be compiled to reads or writes of variables that represent fields or rows in a table following a starting read of the table's set variable.} (see~\cite{DBLP:journals/pacmpl/RahmaniNDJ19,DBLP:journals/pacmpl/BiswasKVEL21}).
% \nver{All SQL instructions are translated to key-value paradigm by adding a ``set'' variable per table whose content is the set of  ids (primary keys) of the rows present in the table. The translation of every SQL instruction with a WHERE clause starts reading this variable while INSERT and DELETE are modelled as writes on it.}

%Other constructs like $\mathtt{while}$ loops can be defined in a similar way. 
%Let $\KVProgs$ denote the set of programs where a transaction body can contain only such instructions.

\subsection{Isolation Levels}

We present the axiomatic framework introduced
by \citet{DBLP:journals/pacmpl/BiswasE19} for defining isolation levels. %\footnote{Isolation levels are called consistency models by \citet{DBLP:journals/pacmpl/BiswasE19}.}.
Isolation levels are defined as logical constraints, called \emph{axioms}, over \emph{histories}, which are an abstract representation of the interaction between a program and the database in an execution. 
% that record the sequence of reads and writes executed in each transaction, the order between transactions in each session, and a write-read relation (also called read-from) that ``justifies'' read values by associating each read to a write that wrote the value returned by the read.

%TODO SOME INTRO EXPLAINING THAT ISOLATION LEVELS ARE DEFINED AS AXIOMS OVER HISTORIES, WHICH REPRESENT THE INTERACTION BETWEEN A PROGRAM AND A STORE. 
\vspace{-2mm}
\subsubsection{Histories}

Programs interact with a database by issuing transactions formed of $\ibegin$, $\icommit$, $\iabort$, $\textsf{read}$ and $\textsf{write}$ instructions. The effect of executing one such instruction is represented using an \emph{event} $\langle e, \mathit{type} \rangle$ where $e$ is an \textit{identifier} and $\mathit{type} $ is a \textit{type}. There are five types of events: $\ebegin$, $\ecommit$, $\eabort$, $\erd{x}$ for reading the global variable $x$, and $\ewrt{x,v}$ for writing value $v$ to $x$. $\Events$ denotes the set of events.
For a read/write event $e$, we use $\mathit{var}(e)$ to denote the variable $x$. % and $\mathit{val}(e)$ the value $v$.

A \emph{transaction log} $\tup{t,E, \po_t}$ is an identifier $t$ and a finite set of events $E$ along with a strict total order $\po_t$ on $E$, called \emph{program order} (representing the order between instructions in the body of a transaction).
%$T$  is a finite sequence of events ordered by a strict total order $\po_T$ called \emph{program order}. 
The minimal element of $\po_t$ is a $\ebegin$ event. A transaction log without neither a $\ecommit$ nor an $\eabort$ event is called \emph{pending}. Otherwise, it is called \emph{complete}. A complete transaction log with a $\ecommit$ event is called \textit{committed} and \textit{aborted} otherwise. If a $\ecommit$ or an $\eabort$ event occurs, then it is maximal in $\po_t$; $\ecommit$ and $\eabort$ cannot occur in the same log. The set $E$ of events in a transaction log $t$ is denoted by $\events{t}$. Note that a transaction is aborted because it executed an $\iabort$ instruction. Histories do not include transactions aborted by the database because their effect should not be visible to other transactions and the abort is not under the control of the program. For simplicity, we may use the term \emph{transaction} instead of transaction log.

Isolation levels differ in the values returned by read events which are not preceded by a write on the same variable in the same transaction. \nver{We assume in the following that every transaction in a program is executed under the same isolation level.} For every isolation level that we are aware of, 
%
%The program order $\po_t$ represents the order between instructions in the body of a transaction. 
%We assume that %each transaction log is well-formed in the sense that 
if a read of a global variable $x$ is preceded by a write to $x$ in $\po_t$, then it should return the value written by the last write to $x$ before the read (w.r.t. $\po_t$). 
%This property is implicit in the definition of every isolation level that we are aware of.  Therefore, %The  set of all transaction logs is denoted by $\mathsf{Tlogs}$.

%For every transaction $T$, we denote $\po_T$ the total order existing between the events in $T$.
%During the whole paper we will assume that every pair of transactions are disjoint and that both $\mathcal{E}$ and $\mathcal{T}$ are finite. Therefore, we denote the function $tr: \mathcal{E} \to \mathcal{T}$ that associates every event to the unique transaction it belongs to. %Moreover, we will assume there is a special transaction called \callout{initial} that contains exactly one write event for every possible variable.

The set of $\erd{x}$ events in a transaction log $t$ that are \textit{not} preceded by a write to $x$ in $\po_t$, for some $x$, is denoted by $\readOp{t}$. 
%As mentioned above, the other read events take their values from writes in the same transaction and their behavior is independent of other transactions. 
Also, if $t$ does \textit{not} contain an $\eabort$ event, the set of $\ewrt{x,\_}$ events in $t$ that are \textit{not} followed by other writes to $x$ in $\po_t$, for some $x$, is denoted by $\writeOp{t}$. If a transaction contains multiple writes to the same variable, then only the last one (w.r.t. $\po_t$) can be visible to other transactions (w.r.t. any isolation level that we are aware of). If $t$ contains an abort event, then we define $\writeOp{t}$ to be the empty set. This is because the effect of aborted transactions (its set of writes) should not be visible to other transactions.
The extension to sets of transaction logs is defined as usual. 
Also, we say that a transaction log $t$ \emph{writes} $x$, denoted by $\writeVar{t}{x}$, when $\writeOp{t}$ contains some $\ewrt{x,\_}$ event. 

A \emph{history} contains a set of transaction logs (with distinct identifiers)
ordered by a (partial) \emph{session order} $\so$ that represents the order
between transactions in the same session. %\footnote{For our programming language, $\so$ would be a union of total orders. This constraint is not important for defining isolation levels.}. 
It also includes a
%ordering constraints imposed by the applications using the database. Most often, $\so$ is a union of sequences, each sequence being called a \emph{session}. 
\emph{write-read} relation (also called read-from) that defines read values by associating each read to a transaction that wrote that value. Read events do \emph{not} contain a value, and their return value is defined as the value written by the transaction associated by the write-read relation.
%
\nver{Let $T$ be a set of transaction logs.}
For a write-read relation \oldver{$\wro\subseteq T\times \readOp{T}$}\nver{$\wro\subseteq \writeOp{T}\times \readOp{T}$} and variable $\key$, $\wro_\key$ is the restriction of $\wro$ to reads of $\key$, \oldver{$\wro_\key=\wro\cap (T\times \{ e\ |\ e \mbox{ is a }\erd{\key} \mbox{ event}\})$}\nver{$\wro_\key=\wro\cap (\writeOp{T}\times \{ e\ |\ e \mbox{ is a }\erd{\key} \mbox{ event}\})$}. We extend the relations $\wro$ and $\wro_\key$ to pairs of transactions by $\tup{t_1,t_2}\in \wro$, resp., $\tup{t_1,t_2}\in \wro_\key$, iff there exists \nver{a $\wrt{x}{\_}$ event $w$ in $t_1$ and} a $\rd{\key}$ event $r$ in $t_2$  s.t. \oldver{$\tup{t_1,e}\in \wro$, resp., $\tup{t_1,e}\in \wro_\key$}\nver{$\tup{w,r}\in \wro$, resp., $\tup{w, r}\in \wro_\key$.} \nver{Analogously, $\wro$ and $\wro_\key$ can be extended to tuples formed of a transaction (containing a write) and a read event.} We say that the transaction log $t_1$ is \emph{read} by the transaction log $t_2$ when $\tup{t_1,t_2}\in \wro$. 

\vspace{-1mm}
\begin{definition}
A \emph{history} $\tup{T, \so, \wro}$ is a set of transaction logs $T$ along with a strict partial \emph{session order} $\so$, and a 
\emph{write-read} relation \oldver{$\wro\subseteq T\times \readOp{T}$}\nver{$\wro\subseteq \writeOp{T}\times \readOp{T}$} such that
\vspace{-1mm}
\begin{itemize}
	\item the inverse of $\wro$ is a total function, 
	\item \oldver{if $(t,e)\in \wro$, where $e$ is a $\erd{x}$ event, then $\writeOp{t}$ contains a $\ewrt{x,\_}$ event,}\nver{if $(w,r)\in \wro$, then $w$ and $r$ are a write and respectively, a read, of the same variable,} and
	\item $\so\cup\wro$ is acyclic (here we use the extension of $\wro$ to pairs of transactions).
\end{itemize}
\vspace{-2mm}
\end{definition}

Every history includes a distinguished transaction writing the initial values of all global variables. This transaction precedes all the other transactions in $\so$. We use $\hist$, $\hist_1$, $\hist_2$, $\ldots$ to range over histories. 

The set of transaction logs $T$ in a history $\hist=\tup{T, \so, \wro}$ is denoted by $\tlogs{\hist}$, and $\events{\hist}$ is the union of $\events{t}$ for $t\in T$. For a history $\hist$ and an event $e$ in $\hist$, $\trans{h}{e}$ is the transaction $t$ in $\hist$ that contains $e$. Also, $\writeOp{\hist}=\bigcup_{t\in \tlogs{h}}\writeOp{t}$ and $\readOp{\hist}=\bigcup_{t\in \tlogs{h}}\readOp{t}$.

We extend $\so$\oldver{ and $\wro$} to pairs of events by $(e_1,e_2)\in \so$ if $(\trans{h}{e_1},\trans{h}{e_2})\in\so$. Also, $\po=\bigcup_{t\in T} \po_t$.


%TODO NOT SURE THAT THE FOLLOWING DEFINITION IS NEEDED
%
%\begin{definition}
%Let $h$ be a history:
%\begin{itemize}
%\item $h$ is called \callout{complete} if every transaction is non-pending and \callout{incomplete} otherwise;
%\item $h$ is \callout{executed in isolation} if it contains at most one pending transaction;
%\item $h$ is called \callout{total} if it is complete and contains every transaction $T \in \mathcal{T}$.
%\end{itemize}
%\end{definition}
%
%\textcolor{red}{\sout{If the event $e =\nextEvent(h)$ is $\ibegin, \iwrite$ or $\iend$, we will denote by $h \bullet e$ the history $h' = \langle E', \so', \wro\rangle$ where $E' = \events{h} \cup \{e\}$ and $\so' = \so \cup \{\langle e', e \rangle \ | \ e' \in h \land \thread{e} = \thread{e'}\}$. On the other hand, if $e$ is a $\iread$ event, we will define the history $h_w' = h \bullet_w e$ for some $\iwrite$ event $w \in h$ as $\langle E', \so', \wro \cup \{\langle w, r \rangle\} \rangle$; where $E'$ and $\so'$ defined as before.}: Not well defined, just cut-pasted from below}. 
%
%\textcolor{red}{EXTENSIONS, $\mathcal{H}^<$ AND $\bullet$ OPERATOR NOT (yet) DEFINED IN THIS SECTION!!!!!!!}

\vspace{-1mm}
\subsubsection{Axiomatic Framework}

\begin{figure}[t]
	\resizebox{\textwidth}{!}{
		\footnotesize
		\begin{tabular}{|c|c|c|c|}
			\hline & & & \\ [-2mm]
			\begin{subfigure}[b]{.24\textwidth}
				\centering
				\begin{tikzpicture}[->,>=stealth,shorten >=1pt,auto,node distance=4cm,
					semithick, transform shape]
					\node[transaction state, text=black] at (0,0)       (t_1)           {$t_1$};
					\node[transaction state] at (2,0)       (t_3)           {$t_3$};
					\node[transaction state, text=black,label={above:\textcolor{black}{$\writeVar{ }{\key}$}}] at (-.5,1.5) (t_2) {$t_2$};
					\path (t_1) edge[wrColor] node {$\wro_x$} (t_3);
					% \path (t_2) edge[blue] node {$\CO$} (t_1);
					\path (t_2) edge[bend left] node {$(\so \cup \wro)^+$} (t_3);
					%   \path [->, decoration={snake}] (t_2) edge[decorate] node[auto] {F} (t_3);
					\path (t_2) edge[left,double equal sign distance,coColor] node {$\co$} (t_1);
				\end{tikzpicture}
				\parbox{\textwidth}{
					$ $ \\

					$t_1\neq t_2\ \land \tup{t_1,t_3}\in \wro_x \ \land $
					
					\hspace{2mm}$\writeVar{t_2}{x}\ \land$ 

					\hspace{2mm}$\tup{t_2,t_3}\in(\so \cup \wro)^+$
					
					\hspace{4mm}$\implies \tup{t_2,t_1}\in\co$
				}
				
				\caption{$\mathsf{Causal\ Consistency}$}
				\label{cc_def}
			\end{subfigure}
			
			&     
			\begin{subfigure}[b]{.24\textwidth}
				\centering
				\begin{tikzpicture}[->,>=stealth,shorten >=1pt,auto,node distance=4cm,
				 semithick, transform shape]
				\node[transaction state, text=black] at (0,0)       (t_1)           {$t_1$};
				\node[transaction state] at (2,0)       (t_3)           {$t_3$};
				\node[transaction state, text=black,label={above:\textcolor{black}{$\writeVar{ }{x}$}}] at (-0.5,1.5) (t_2) {$t_2$};
				\node[transaction state] at (1.5,1.5) (t_4) {$t_4$};
				\path (t_1) edge[wrColor] node {$\wro_x$} (t_3);
				% \path (t_2) edge[blue] node {$\CO$} (t_1);
				\path (t_2) edge[] node {$\co^*$} (t_4);
				\path (t_4) edge[left] node {$(\so \cup \wro)$} (t_3);
				\path (t_2) edge[left,double, coColor] node {$\co$} (t_1);
				\end{tikzpicture}
				\parbox{\textwidth}{
				
				$ $ \\

				$t_1\neq t_2\ \land \tup{t_1,t_3}\in \wro_x \ \land $
				
				\hspace{2mm}$\writeVar{t_2}{x}\ \land$ 
				
				\hspace{2mm}$\tup{t_2,t_3}\in\co^*\circ\,(\wro\cup\so)$
				
				\hspace{4mm}$\implies \tup{t_2,t_1}\in\co$
				}
				
				\caption{$\mathsf{Prefix}$}
				\label{pre_def}
				\end{subfigure}
			&
			\hspace{-1mm}

			\begin{subfigure}[b]{.24\textwidth}
			    \centering
			    \begin{tikzpicture}[->,>=stealth,shorten >=1pt,auto,node distance=4cm,
			      semithick, transform shape]
			     \node[transaction state, text=black] at (0,0)       (t_1)           {$t_1$};
			     \node[transaction state, label={[xshift=-5]below:$\writeVar{ }{\yvar}$}] at (2,0)       (t_3)           {$t_3$};
			     \node[transaction state, text=black,label={above:$\writeVar{}{x}$}] at (-.5,1.5) (t_2) {$t_2$};
			     \node[transaction state, label={[yshift=-2]above:{$\writeVar{}{\yvar}$}}] at (1.5,1.5) (t_4) {$t_4$};
			     \path (t_1) edge[wrColor] node {$\wro_x$} (t_3);
			     % \path (t_2) edge[blue] node {$\CO$} (t_1);
			     \path (t_2) edge node {$\co^*$} (t_4);
			     \path (t_4) edge node {$\co$} (t_3);
			     \path (t_2) edge[left,double, coColor] node {$\co$} (t_1);
			    \end{tikzpicture}
			    \parbox{\textwidth}{

			     $t_1\neq t_2\ \land \ \tup{t_1,t_3}\in \wro_x \ \land$
			     
			     \hspace{2mm}$ \writeVar{t_2}{\xvar}\ \land \ \writeVar{t_3}{\yvar}\ \land$ 
			     
			     \hspace{2mm}$ \writeVar{t_4}{\yvar} \land  \tup{t_2,t_4}\in\co^*$ 
			     
			     \hspace{2mm}$\land \ \tup{t_4,t_3}\in\co$
			     
			     \hspace{4mm}$\implies \tup{t_2,t_1}\in\co$
			    }
			    
			    \caption{$\mathsf{Conflict}$}
			    \label{confl_def}
			   \end{subfigure}
			
			   & 
    
			\begin{subfigure}[b]{.24\textwidth}
				\centering
				\begin{tikzpicture}[->,>=stealth,shorten >=1pt,auto,node distance=4cm,
					semithick, transform shape]
					\node[transaction state, text=black] at (0,0)       (t_1)           {$t_1$};
					\node[transaction state] at (2,0)       (t_3)           {$t_3$};
					\node[transaction state, text=black, label={above:\textcolor{black}{$\writeVar{ }{x}$}}] at (-.5,1.5) (t_2) {$t_2$};
					\path (t_1) edge[wrColor] node {$\wro_x$} (t_3);
					% \path (t_2) edge[blue] node {$\CO$} (t_1);
					\path (t_2) edge[bend left] node {$\co$} (t_3);
					\path (t_2) edge[left,double, coColor] node {$\co$} (t_1);
				\end{tikzpicture}
				\parbox{\textwidth}{
					$ $ \\
					$ $ \\


					$t_1\neq t_2\ \land \ \tup{t_1,t_3}\in \wro_x \land$
					
					\hspace{2mm}$ \writeVar{t_2}{x}\ \land \ \tup{t_2,t_3}\in\co$ 
										
					\hspace{4mm}$\implies \tup{t_2,t_1}\in\co$
				}
				
				\caption{$\mathsf{Serializability}$}
				\label{ser_def}
			\end{subfigure}
			
			\\ \hline			  
		\end{tabular}
	}
	\vspace{-2mm}
	\caption{Axioms defining isolations levels (all logical variables representing transactions, e.g., $t_1$, are universally quantified). The reflexive and transitive, resp., transitive, closure of a relation $rel$ is denoted by $rel^*$, resp., $rel^+$. Also, $\circ$ denotes the composition of two relations, i.e., $rel_1 \circ rel_2 = \{\tup{a, b} | \exists c. \tup{a, c} \in rel_1 \land \tup{c, b} \in rel_2\}$.}
	\label{fig:consistency_defs}
	\vspace{-4mm}
\end{figure}

A history satisfies a certain isolation level if there is a strict total order $\co$ on its transactions, called \emph{commit order}, which extends the write-read relation and the session order, and which satisfies certain properties. These properties, called \emph{axioms}, relate the commit order with the $\so$ and $\wro$ relations in a history and are
%the session-order and the write-read relation in the history. 
%The axioms define mandatory $\co$ predecessors $\tr_2$ of a transaction $\tr_1$ that is read in the history. 
%They are 
defined as 
first-order formulas of the form:
\label{eq:axioms}
\vspace{-1mm}
\begin{align}
  & \forall \key,\ \forall \tr_1\neq \tr_2,\ \forall \tr_3.\ \nonumber\\
  & \hspace{3mm}  \tup{\tr_1,t_3}\in \wro_\key \land \writeVar{\tr_2}{\key} \land \phi(\tr_2,\tr_3) \implies \tup{\tr_2,\tr_1}\in\co \label{eq:axiom}
%  & \hspace{5.4cm} \implies \tup{\tr_2,\tr_1}\in\co \nonumber
\end{align}
\vspace{-5mm}

where $\phi$ is a property relating $\tr_2$ and $\tau$ (i.e., the read or the
transaction reading from $\tr_1$) that varies from one axiom to another.\footnote{These formulas are interpreted on tuples $\tup{\hist,\co}$ of a history $\hist$ and a commit order $\co$ on the transactions in $\hist$ as usual.} Note that an aborted transaction $t$ cannot take the role of $\tr_1$ nor $\tr_2$ in equation \ref{eq:axiom} as the set $\writeOp{t}$ is empty. Intuitively, this axiom schema states the following: in order for $\tau$ to read specifically $t_1$'s write on $k$, it must be the case that every $t_2$ that also writes $k$ and satisfies $\phi(t_2,\tau)$ was committed before $t_1$. 
%Note that in all cases we consider, $\phi(t_2,\tau)$ already ensures that $t_2$ is committed before the read $\tau$, so this axiom schema ensures that $t_2$ is furthermore committed before $t_1$'s write.
The property $\phi$ relates $\tr_2$ and $\tau$ using the relations in a history and the commit order. 
Figure~\ref{fig:consistency_defs} shows two axioms which correspond to their homonymous isolation levels: \textit{Causal Consistency} ($\CC$) and \textit{Serializability} ($\SER$). The conjunction of the other two axioms Conflict and Prefix defines \textit{Snapshot Isolation} ($\SI$). \textit{Read Atomic} ($\RA$) is a weakening of $\CC$ where $(\so \cup \wro)^+$ is replaced with $\so \cup \wro$. \textit{Read Committed} ($\RC$) is defined similarly\appendixver{(see Appendix~\ref{sec:def:RA-RC})}.
%Analogously, some isolation levels such as \textit{Read Committed} ($\RC$), \textit{Read Atomic} ($\RA$) can be defined in the same way (Appendix~\ref{sec:def:RA-RC}).
Note that $\SER$ is stronger than $\SI$ (i.e., every history satisfying $\SER$ satisfies $\SI$ as well), $\SI$ is stronger than $\CC$, $\CC$ is stronger than $\RA$, and $\RA$ is stronger than $\RC$.
% as the model where prefix and conflict axioms both hold. 
%We say a history $h$ satisfies an isolation level $I$ if there is a total order called \callout{commit order} $\co$ that extend $\so \cup \wro$ and satisfies its axioms. However, by the definition of $\RC, \RA$ and $\CC$, it is clear that for every history $h$ s.t. the relation $\co$ deduced from $\so \cup \wro$ is acyclic exists a commit order for those isolation levels.
%Figure~\ref{fig:consistency_defs} shows the axioms defining Read Committed, Causal Consistency, and Serializability (see \citet{DBLP:journals/pacmpl/BiswasE19} for axioms defining Read Atomic, Prefix, and Snapshot Isolation). 




%For instance, $\mathsf{Read\ Committed}$~\cite{DBLP:conf/sigmod/BerensonBGMOO95} requires that every read returns a value written in a committed transaction, and also, that the reads in the same transaction are ``monotonic'', i.e., they do not return values that are older, w.r.t. the commit order, than values read in the past.
%%\footnote{This monotonicity property corresponds to the fact that in the original formulation of $\mathsf{Read\ Committed}$~\cite{DBLP:conf/sigmod/BerensonBGMOO95}, every write is guarded by the acquisition of a lock on the written key, that is held until the end of the transaction.}. 
%While the first condition holds for every history (because of the surjectivity of $\wro$), the second condition is expressed by the axiom $\mathsf{Read\ Committed}$ in Figure~\ref{lock_rc_def}, which states that for any transaction $\tr_1$ writing a key $\key$ that is read at an operaion $\alpha$ in a transaction, the set of transactions $\tr_2$ writing $\key$ and read previously in the same transaction (these reads may concern other keys) must precede $\tr_1$ in commit order. 
%For instance, Figure~\ref{rc_example:1} shows a history and a (partial) commit order that does not satisfy this axiom because $\rd{\key_1}{1}$ returns the value written in a transaction ``older'' than the transaction read in the previous $\rd{\key_2}{2}$. %An exa

\begin{wrapfigure}{r}{0.4\textwidth}
\vspace{-5mm}
%\vspace{0.5mm}
   \centering
%   \begin{subfigure}{.3\textwidth}
%  \resizebox{\textwidth}{!}{
%\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
%    semithick, transform shape]
%    \node[draw, rounded corners=2mm] (t1) at (0, 0) {\begin{tabular}{l} $\wrt{\key_1}{1}$ \end{tabular}};
%   \node[draw, rounded corners=2mm,outer sep=0] (t2) at (0, -1.5) {\begin{tabular}{l} $\wrt{\key_1}{2}$ \\ $\wrt{\key_2}{2}$\end{tabular}};
%   \node[draw, rounded corners=2mm, minimum width=1.8cm, minimum height=2.5cm] (t3) at (3, -0.75) {};
%   \node[style={inner sep=0,outer sep=0}] (t3_1) at (3, 0) {\begin{tabular}{l} $\rd{\key_2}{2}$ \end{tabular}};
%   \node[style={inner sep=0,outer sep=0}] (t3_2) at (3, -1.5) {\begin{tabular}{l} $\rd{\key_1}{1}$ \end{tabular}};
%   % \path (t1) edge node {} (t3_2);
%   % \path (t2) edge node {} (t3_1);
%   \path (t1) edge node {$\co$} (t2);
%   \path (t3_1) edge node {$\po$} (t3_2);
%   \path (t1) edge[below] node[yshift=-4,xshift=4] {$\wro$} (t3_2);
%   \path (t2) edge node[yshift=-2,xshift=7] {$\wro$} (t3_1);
%  \end{tikzpicture}  
%    }
%    \caption{$\mathsf{Read\ Committed}$ violation.}
%    \label{rc_example:1}
%\end{subfigure}
%\hspace{1cm}
%\begin{subfigure}{.4\textwidth}
\resizebox{0.38\textwidth}{!}{
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
 semithick, transform shape]
 \node[draw, rounded corners=2mm,outer sep=0, label={[font=\small]180:$t_1$}] (t1) at (0, 1.4) {$\ewrt{x,1}$};
\node[draw, rounded corners=2mm,outer sep=0,label={[font=\small]0:$t_2$}] (t2) at (3, 1.4) {\begin{tabular}{l} $\erd{x}$ \\ $\ewrt{x,2}$ \end{tabular}};
\node[draw, rounded corners=2mm,outer sep=0,label={[font=\small]0:$t_3$}] (t3) at (3, 0) {\begin{tabular}{l} $\erd{x}$ \\ $\erd{y}$ \end{tabular}};
\node[draw, rounded corners=2mm,outer sep=0,label={[font=\small]180:$t_4$}] (t4) at (0, 0) {\begin{tabular}{l} $\erd{x}$ \\ $\ewrt{y,1}$\end{tabular}};

\path (t1) edge[above] node[yshift=0,xshift=0] {$\wro_x$} (t2);

\path (t1) edge[below] node[yshift=-3,xshift=3] {$\wro_x$} (t3);

\path (t2) edge[above] node[yshift=-6,xshift=-18] {$\wro_x$} (0,0.58);

\path (t4) edge[below] node[yshift=0,xshift=0] {$\wro_y$} (t3);
\end{tikzpicture}  
}
% \caption{Causal C violation.}
% \label{cc_example:1}
%\end{subfigure}
\vspace{-2mm}
  \caption{Causal Consistency violation. Boxes group events from the same transaction.}
  \label{counter_example:1}
\vspace{-4mm}
\end{wrapfigure}
For instance, the axiom defining Causal Consistency~\cite{DBLP:journals/cacm/Lamport78} states that for any transaction $\tr_1$ writing a variable $x$ that is read in a transaction $\tr_3$, the set of $(\wro\cup \so)^+$ predecessors of $\tr_3$ writing $x$ must precede $\tr_1$ in commit order ($(\wro\cup \so)^+$ is usually called the \emph{causal} order). A violation of this axiom can be found in Figure~\ref{counter_example:1}: the transaction $\tr_2$ writing 2 to $x$ is a $(\wro\cup \so)^+$ predecessor of the transaction $\tr_3$ reading 1 from $x$ because the transaction $\tr_4$, writing 1 to $y$, reads $x$ from $\tr_2$ and $\tr_3$ reads $y$ from $\tr_4$. This implies that $\tr_2$ should precede in commit order the transaction $\tr_1$ writing 1 to $x$, which is inconsistent with the write-read relation ($\tr_2$ reads from $\tr_1$).

The $\mathsf{Serializability}$ axiom requires that for any transaction $\tr_1$ writing to a variable $x$ that is read in a transaction $\tr_3$, the set of $\co$ predecessors of $\tr_3$ writing $x$ must precede $\tr_1$ in commit order. This ensures that each transaction observes the effects of all the $\co$ predecessors. 

%It was shown in~\cite{DBLP:journals/pacmpl/BiswasE19} that as expected, $\mathsf{Serializability}$ implies $\mathsf{Causal}$, which implies $\mathsf{Read\ Committed}$ (when interpreted as first-order formulas).

\begin{definition}
For an isolation level $I$ defined by a set of axioms $X$, a history
$\hist=\tup{T, \so, \wro}$ \emph{satisfies} $I$ iff there is a strict total
order $\co$ s.t. $\wro\cup\so\subseteq \co$ and $\tup{h,\co}$ satisfies $X$. %\footnote{Isolation levels like Snapshot Isolation require more than one axiom.}
 % Given a $\CO$(\textit{commit order}), a total order on $T$ which extends $\wro \cup \so$, we can define consistency axioms from table \ref{consistency_defs}. For each axiom, the situation in the table implies, $\Path{\tr_2}{\CO}{\tr_1}$.
 \label{axiom-criterion}
\end{definition}

A history that satisfies an isolation level $I$ is called $I$-consistent. For two isolation levels $I_1$ and $I_2$, $I_1$ is \emph{weaker than} $I_2$ when every $I_1$-consistent history is also $I_2$-consistent.

%=====
%
%To fully model any behavior of a transactional concurrent program we are obliged to formally describe the database section. This notion will be depicted as the concept of \textit{model}:
%
%%Those notions are generic enough to only describe a possible set of instructions that a parallel program may execute along with the $\wr$ relations that exist between them.
%
%\begin{comment}
%\begin{definition}
%An axiomatic \callout{model} $\mathcal{M}$ over histories is a collection of rules that enforce a \callout{consistency criterion} over them. The histories that satisfy those criteria are called \callout{consistent} while the rest are simply denoted inconsistent. 
%\end{definition}
%\end{comment}
%
%\begin{definition}
%An axiomatic \callout{model} $\mathcal{M}$ over histories is a collection of rules that enforce a \callout{consistency criterion} over them. The histories that satisfy those criteria are called \callout{$\mathcal{M}$-consistent} while the rest are simply denoted $\mathcal{M}$-inconsistent. If there is no ambiguity on the model, we will simply denote them consistent or inconsistent.%
%
%\end{definition}
%
%
%
%In figure \ref{fig:consistency_defs} it is depicted five axioms which correspond to their homonymous isolation levels: \textit{Read Committed} ($\RC$), \textit{Read Atomic} ($\RA$), \textit{Causal Consistency} ($\CC$)  \textit{Prefix Consistency} ($\PRE$) and \textit{Serializability} ($\SER$); along with the conflict axiom. Conflict and Prefix allow us to define \textit{Snapshot Isolation} ($\SI$) as the model where prefix and conflict axioms both hold. We say a history $h$ satisfies an isolation level $I$ if there is a total order called \callout{commit order} $\co$ that extend $\so \cup \wro$ and satisfies its axioms. However, by the definition of $\RC, \RA$ and $\CC$, it is clear that for every history $h$ s.t. the relation $\co$ deduced from $\so \cup \wro$ is acyclic exists a commit order for those isolation levels.
%
%TODO DEFINE $I$-consistent histories

\subsection{Program Semantics}\label{ssec:semantics}

We define a small-step operational semantics for transactional programs, which is parametrized by an isolation level $I$. The semantics keeps a history of previously executed database accesses in order to maintain consistency with $I$. 

For readability, we define a program as a partial function $\prog:\mathsf{SessId}\rightharpoonup \mathsf{Sess}$ that associates session identifiers in $\mathsf{SessId}$ with concrete code as defined in Figure~\ref{fig:syntax} (i.e., sequences of transactions). Similarly, the session order $\so$ in a history is defined as a partial function $\so:\mathsf{SessId}\rightharpoonup \mathsf{Tlogs}^*$ that associates session identifiers with sequences of transaction logs. Two transaction logs are ordered by $\so$ if one occurs before the other in some sequence $\so(j)$ with 
$j\in \mathsf{SessId}$.

The operational semantics is defined as a transition relation $\Rightarrow_I$ between \emph{configurations}, which are defined as tuples containing the following:
\begin{itemize}
	\item history $\hist$ storing the events generated by database accesses executed in the past, 
	\item a valuation map $\vec{\gamma}$ that records local variable values in the current transaction of each session ($\vec{\gamma}$ associates identifiers of sessions with valuations of local variables),
	\item a map $\vec{B}$ that stores the code of each live transaction (mapping session identifiers to code), 
	\item sessions/transactions $\prog$ that remain to be executed from the original program.
\end{itemize}

The relation $\Rightarrow_I$ is defined using a set of rules as expected\appendixver{(their precise definition can be found in Appendix~\ref{app:rules})}. %(the others can be defined in a similar manner). 
Starting a new transaction in a session $j$ is enabled as long as this session has no live transactions ($\vec{\mathsf{B}}(j) = \epsilon$) and results in adding a transaction log with a single $\ebegin$ event to the history and scheduling the body of the transaction (adding it to $\vec{\mathsf{B}}(j)$). Local steps, i.e., checking a Boolean condition or computation with local variables, use the local variable valuations and advance the code as expected. Read instructions of some global variable $x$ can have two possible behaviors: (1) if the read follows a write on $x$ in the same transaction, then it returns the value written by the last write on $x$ in that transaction, and (2) otherwise, the read reads from another transaction $\tr'$ which is chosen non-deterministically as long as extending the current history with the write-read dependency associated to this choice leads to a history that still satisfies $I$. \nver{Depending on the isolation level, there may not exist a transaction $\tr'$ the read can read from\appendixver{(see Appendix~\ref{app:impossibility} for a concrete example)}.} For other instructions, e.g., $\icommit$ and $\iabort$, the history is simply extended with the corresponding events while ending the transaction execution in the case of $\iabort$.

%\textsc{spawn} starts a new transaction in a session $j$ provided that this session has no live transaction ($\vec{\mathsf{B}}(j) = \epsilon$). It adds a transaction log with a single $\ebegin$ event to the history and schedules the body of the transaction. \textsc{if-true} and \textsc{if-false} check the truth value of a Boolean condition of an $\mathtt{if}$ conditional. \textsc{local} models the execution of an assignment to a local variable which does not impact the stored history. \textsc{read-local} and \textsc{read-extern} concern read instructions. \textsc{read-local} handles the case where the read follows a write on the variable $x$ in the same transaction: the read returns the value written by the last write on $x$ in that transaction. Otherwise, \textsc{read-extern} corresponds to reading a value written in another transaction $\tr'$. The transaction $\tr'$ is chosen non-deterministically as long as extending the current history with the write-read dependency associated to this choice leads to a history that still satisfies $I$. \textsc{read-extern} applies only when the executing transaction contains no write on the same variable. \textsc{commit} confirms the end of a transaction making its writes visible while \textsc{abort} ends the transaction's execution immediately.

An \emph{initial} configuration for program $\prog$ contains the program $\prog$, a history $\hist=\tup{\{\tr_0\},\emptyset,\emptyset}$ where $\tr_0$ is a transaction log containing writes that write the initial value for all variables, and empty current transaction code ($\mathsf{B}=\epsilon$). 
An execution of a program $\prog$ under an isolation level $I$ is a sequence of configurations $c_0 c_1\ldots c_n$ where $c_0$ is an initial configuration for $\prog$, and $c_m\Rightarrow_I c_{m+1}$, for every $0\leq m < n$. We say that $c_n$ is \emph{$I$-reachable} from $c_0$.
The history of such an execution is the history $\hist$ in the last configuration $c_n$. 
A configuration is called \emph{final} if it contains the empty program ($\prog=\emptyset$).
Let $\histOf[I]{\prog}$ denote the set of all histories of an execution of $\prog$ under $I$ that ends in a final configuration.



==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/related.tex <==
%!TEX root = main.tex
\section{Related Work}\label{sec:related}

\noindent
\textbf{Checking Correctness of Database-Backed Applications.}
%There here have been several directions of work addressing the correctness of database-backed applications. 
One line of work is concerned with the logical formalization
of isolation levels 
\cite{ansi,DBLP:conf/icde/AdyaLO00,DBLP:conf/sigmod/BerensonBGMOO95,DBLP:conf/concur/Cerone0G15,DBLP:journals/pacmpl/BiswasE19}.
Our work relies on the axiomatic definitions of isolation levels introduced by \citet{DBLP:journals/pacmpl/BiswasE19}, which have also investigated
the problem of checking whether a given history satisfies a certain isolation
level. Our SMC algorithms rely on these algorithms to check consistency of a history with a given isolation level. 
%the validity of the values returned by read operations. Working with a
%logical formalization allowed us to avoid implementing an actual database with replication or
%sophisticated synchronization.

Another line of work focuses on the problem of finding ``anomalies'': 
behaviors that are not possible under serializability. This is typically done
via a static analysis of the application code that builds a static dependency graph that
over-approximates the data dependencies in all possible
executions of the application~\cite{DBLP:journals/jacm/CeroneG18,DBLP:conf/concur/0002G16,DBLP:journals/tods/FeketeLOOS05,DBLP:conf/vldb/JorwekarFRS07,acidrain,isodiff}.
Anomalies with respect to a given isolation level then correspond to a
particular class of cycles in this graph. Static dependency graphs turn out to
be highly imprecise in representing feasible executions, leading to false
positives. Another source of false positives is that an anomaly might not be a
bug because the application may already be designed to handle the
non-serializable behavior \cite{DBLP:conf/pldi/BrutschyD0V18,isodiff}. 
Recent work has tried to address these issues by using more precise 
logical encodings of the application~\cite{DBLP:conf/popl/BrutschyD0V17,DBLP:conf/pldi/BrutschyD0V18}, or
by using user-guided heuristics~\cite{isodiff}. 
Another approach consists of modeling the application
logic and the isolation level in first-order logic and relying on SMT solvers to
search for anomalies~\cite{DBLP:journals/pacmpl/KakiESJ18,DBLP:conf/concur/NagarJ18,burcu-netys},
or defining specialized reductions to assertion
checking~\cite{DBLP:conf/concur/BeillahiBE19,DBLP:conf/cav/BeillahiBE19}.
Our approach, based on SMC, does not generate false positives because we systematically
enumerate only valid executions of a program which allows to check for user-defined assertions.

Several works have looked at the problem of reasoning about the correctness of
applications executing under weak isolation and introducing additional
synchronization when
necessary~\cite{DBLP:conf/eurosys/BalegasDFRPNS15,DBLP:conf/popl/GotsmanYFNS16,DBLP:conf/esop/NairP020,DBLP:conf/usenix/0001LCPRV14}.
These are based on static analysis or logical proof arguments. 
The issue of repairing applications is orthogonal to our work. 

MonkeyDB~\cite{DBLP:journals/pacmpl/BiswasKVEL21} is a mock storage system for testing storage-backed applications. 
While being able to scale to larger code, it has the inherent incompleteness of testing. As opposed to MonkeyDB, our algorithms perform a systematic and complete exploration of executions and can establish correctness at least in some bounded context, and they avoid redundancy, enumerating equivalent executions multiple times. Such guarantees are beyond the scope of MonkeyDB.


%The \textsc{Clotho} tool \cite{clotho}, for instance, uses a static analysis of the application to
%generate test cases with plausible anomalies, which are deployed in a concrete
%testing environment for generating actual executions. 
%
%
%Our approach, based on testing with MonkeyDB, has several practical advantages.
%There is no need for analyzing application code; we can work with any
%application. There are no false positives because we directly run the
%application and check for user-defined assertions, instead of looking for
%application-agnostic anomalies. The limitation, however, of the MonkeyDB approach is 
%the inherent incompleteness of testing.
%
%
%As in the previous case, our work based on testing has the advantage that it can
%scale to real sized applications (as opposed to these techniques which are based
%on static analysis or logical proof arguments), but it cannot prove that an
%application is correct. Moreover, the issue of repairing applications is
%orthogonal to our work. 
%
%MonkeyDB~\cite{DBLP:journals/pacmpl/BiswasKVEL21}

%\vspace{1mm}
%\noindent
%\textbf{Model Checking Concurrent Programs.}
%Over the years various different techniques have been introduced to deal with the state explosion problem in model checking. For concurrent programs specifically, depth bounding \cite{DBLP:conf/popl/Godefroid97}, delay bounding \cite{DBLP:conf/popl/EmmiQR11}, context bounding (bounding the number of context switches) \cite{DBLP:conf/tacas/QadeerR05}, preemption bounding \cite{DBLP:conf/pldi/MusuvathiQ07} and phase bounding \cite{DBLP:conf/tacas/BouajjaniE12} bring tractability to the model checking problem and have been shown to be effective for bug finding. These techniques are all {\em incomplete}, in the sense that lack of bugs does not guarantee the correctness of the system.

%\vspace{1mm}
%\noindent
%\textbf{Partial Order Reduction.}
%POR techniques deal with the state explosion problem in model checking by not exploring multiple executions from the same equivalence class, and are {\em complete}. Early techniques like {\em ample sets} \cite{DBLP:conf/popl/ClarkeES83,DBLP:conf/forte/HolzmannP94} and {\em stubborn sets} \cite{DBLP:journals/fmsd/GodefroidW93,DBLP:conf/dimacs/Godefroid90} were based on static analysis. {\em Sleep sets} \cite{DBLP:conf/dimacs/Godefroid90} were the first to  guarantee optimality (one execution from each Mazurkiewicz trace) \cite{DBLP:journals/fmsd/GodefroidHP95} by keeping track of information from the history of the exploration. %However, they only prune transitions and cannot eliminate any state when used alone. 
%Persistent sets \cite{DBLP:conf/cav/GodefroidP93,DBLP:journals/dc/KatzP92} generalized stubborn and ample sets and enabled development of dynamic POR (DPOR) methods.

\vspace{.5mm}
\noindent
\textbf{Dynamic Partial Order Reduction.}
%DPOR~\cite{DBLP:conf/popl/FlanaganG05} algorithms explore the execution space (and tracking the equivalence relation) on-the-fly without relying on a-priori static analyses. This is typically coupled with SMC~\cite{DBLP:conf/popl/Godefroid97} which explores executions of a program without storing visited states, thereby, avoiding excessive memory consumption. 
\citet{DBLP:journals/jacm/AbdullaAJS17} introduced the concept of \emph{source sets} which provided the first strongly optimal DPOR algorithm for Mazurkiewicz trace equivalence. Other works study DPOR techniques for coarser equivalence relations, e.g.,~\cite{DBLP:journals/pacmpl/AbdullaAJLNS19,DBLP:conf/cav/AgarwalCPPT21,DBLP:conf/tacas/AronisJLS18,DBLP:journals/pacmpl/ChalupaCPSV18,DBLP:journals/pacmpl/ChatterjeePT19}. In all cases, the space complexity is exponential when strong optimality is ensured. % but consumes exponential memory.

%First, many techniques aim to combat the state-space explosion problem by introducing coarser equivalence partitioning\cite{DBLP:journals/pacmpl/AbdullaAJLNS19,DBLP:conf/cav/AgarwalCPPT21,DBLP:conf/tacas/AronisJLS18,DBLP:journals/pacmpl/ChalupaCPSV18,DBLP:journals/pacmpl/ChatterjeePT19}. Among these, only Nidhugg~\cite{DBLP:conf/tacas/AronisJLS18,DBLP:journals/pacmpl/AbdullaAJLNS19} is optimal w.r.t. to its equivalence partitioning(s), although, as demonstrated in 6.1, can suffer from exponential memory consumption.

Other works focus on extending DPOR to weak memory models either by targeting a specific memory model~\cite{DBLP:conf/cav/AbdullaAJL16,DBLP:journals/acta/AbdullaAAJLS17,DBLP:journals/pacmpl/AbdullaAJN18,DBLP:conf/oopsla/NorrisD13} or by being parametric with respect to an axiomatically-defined memory model~\cite{DBLP:conf/pldi/Kokologiannakis19,DBLP:conf/asplos/Kokologiannakis20,DBLP:journals/pacmpl/Kokologiannakis22}. Some of these works can deal with the coarser reads-from equivalence, e.g.,~\cite{DBLP:journals/pacmpl/AbdullaAJN18,DBLP:conf/pldi/Kokologiannakis19,DBLP:conf/asplos/Kokologiannakis20,DBLP:journals/pacmpl/Kokologiannakis22}. Our algorithms build on the work of \citet{DBLP:journals/pacmpl/Kokologiannakis22} which for the first time, proposes a DPOR algorithm which is both strongly optimal and polynomial space. The definitions of database isolation levels are quite different with respect to weak memory models, which makes these previous works not extensible in a direct manner. These definitions include a semantics for \emph{transactions} which are collections of reads and writes, and this poses new difficult challenges. 
For instance, reasoning about the completeness and the (strong) optimality of existing DPOR algorithms for shared-memory is agnostic to the scheduler ($\genericNext$ function) while the strong optimality of our $\textsc{explore-ce}$ algorithm relies on the scheduler keeping at most one transaction pending at a time. \nver{In addition, unlike TruSt, \textsc{explore-ce} ensures that no swapped events can be swapped again and that the history order $<$ is an extension of $\so \cup \wro$.} This makes our completeness and optimality proofs radically different. %\nver{Also, while $\textsc{explore-ce}$ only does consistency checks over partial histories in $\genericValidWrites$, TruSt do additional checks on $\genericNext$ function as their study case involves non-causally extensible weak memory models such as SC.} 
\nver{Moreover, even for transactional programs with one access per transaction, where $\SER$ and $\SC$ are equivalent, TruSt under $\SC$ and $\textsc{explore-ce}^*(I_0,\SER)$ do not coincide, for any $I_0 \in \{\RC, \RA, \CC\}$. In this case, TruSt enumerates only $\SC$-consistent histories at the cost of solving an NP-complete problem at each step while the $\textsc{explore-ce}^*$ step cost is polynomial time at the price of not being strongly-optimal.}
Furthermore, we identify isolation levels ($\SI$ and $\SER$) for which it is impossible to ensure both strong optimality and polynomial space bounds with a swapping-based algorithm, a type of question that has not been investigated in previous work. 

%They do not coincide in the SC case. For Serializability, our work proposes the algorithm EXPLORE(I0, SER) which enumerates histories under an isolation level I0 for which EXPLORE(I0) is strongly optimal, e.g., I0=CC, and filters histories before outputting to be SER-consistent. The version of TruSt that enumerates read-from equivalence classes under SC (Section 4.2 in Kokologiannakis et al. [37]) enumerates only SC-consistent histories, but it needs to check SC consistency at every step in the execution and this check is NP-complete in general.

%CC with singleton transactions corresponds to Strong Release-Acquire (SRA). Even in this case, the two algorithms are not the same. For instance, TruSt allows swapping events that have been already swapped. Also, our algorithm satisfies some invariants, e.g., if (t,r)∈wr then t < r, which are not true for TruSt. We introduced these differences while building the extension to transaction


%investigate the question of whether it is possible to ensure both strong optimality and polynomial space bounds for certain isolation levels ($\SI$ and $\SER$)
%
%In general, completeness and optimality proofs are very sensitive 


%TruSt builds on the foundations laid by GenMC~\cite{DBLP:conf/pldi/Kokologiannakis19} in order to achieve memory-model parametricity; however, it adapts the extensibility requirement on the underlying memory model to a more precise łmaximal extensibility requirement (see 3.1)


%In \cite{DBLP:conf/popl/FlanaganG05}, an efficient stateful algorithm is proposed for computing persistent sets dynamically by considering  currently explored parts of the state space. This algorithm needed large memory for keeping discovered states and the happens-before relation. The algorithm is improved in \cite{DBLP:conf/spin/YangCGK08} with a more efficient state representation, and in \cite{DBLP:conf/icfem/YiWY06} with a summary-based representation of the happens before. % relation is represented more efficiently by introducing summaries. 
%
%In \cite{DBLP:conf/fase/LauterburgKMA10,DBLP:conf/forte/TasharofiKLLMA12}, stateless dynamic POR techniques were introduced. {\em Source sets} \cite{DBLP:journals/jacm/AbdullaAJS17} were introduced in the context of dynamic POR techniques such that the state space can be reduced up to the limit that is theoretically possible. They are generalizations of persistent sets and their relation with persistent sets are investigated in \cite{DBLP:conf/birthday/AbdullaAJS17}. Our eager and lazy algorithms are relying on source sets but operate in the context of stateful model checking. The technique from \cite{DBLP:conf/atva/NeeleWBP16} is similar to our ample algorithm for the GPU setting, but their choice of invisible actions is different than ours.
%While we focus on shared-memory programs running on top of a sequential consistency memory model, POR techniques have been also investigated in the context of weak memory models such as TSO or C11, e.g.,~\cite{DBLP:conf/cav/Kokologiannakis21,DBLP:conf/asplos/Kokologiannakis20,DBLP:journals/acta/AbdullaAAJLS17,DBLP:journals/pacmpl/AbdullaAJN18}.


%AZADEH: WE NEED SOMETHING MORE SOLID ABOUT STATELESS POR. IT CANNOT BE MENTIONED IN A SENTENCE AS A FLEETING THOUGHT ONLY. I WROTE SOMETHING BUT I AM NOT SURE IT IS ACCURATE. I TRIED TO TAKE A FEW RANDOM SENTENCES AND MAKE A THEME OUT OF THEM. READ BELOW AND CORRECT ANY INACCURACIES.


%After seminal works like Verisoft~\cite{DBLP:conf/popl/Godefroid97} and Chess [Musuvathi et al. 2008] paved the way for stateless model checking, there has been a large body of work on SMC and DPOR~\cite{DBLP:conf/popl/FlanaganG05}. A major breakthrough in this line of work was made by Abdulla et al.~\cite{DBLP:journals/jacm/AbdullaAJS17}, who provided the first optimal DPOR algorithm for Mazurkiewicz trace equivalence for sequential consistency. This algorithm, as described in 2.3, avoids blocked explorations at the cost of exponential memory consumption. We can broadly classify the more recent works in this area into two main categories depending on their primary focus.
%First, many techniques aim to combat the state-space explosion problem by introducing coarser equivalence partitionings\cite{DBLP:journals/pacmpl/AbdullaAJLNS19,DBLP:conf/cav/AgarwalCPPT21,DBLP:conf/tacas/AronisJLS18,DBLP:journals/pacmpl/ChalupaCPSV18,DBLP:journals/pacmpl/ChatterjeePT19}. Among these, only Nidhugg~\cite{DBLP:conf/tacas/AronisJLS18,DBLP:journals/pacmpl/AbdullaAJLNS19} is optimal w.r.t. to its equivalence partitioning(s), although, as demonstrated in 6.1, can suffer from exponential memory consumption.
%
%Second, other techniques focus on extending DPOR to weak memory models either by targeting a specific weak memory model~\cite{DBLP:conf/cav/AbdullaAJL16,DBLP:journals/acta/AbdullaAAJLS17,DBLP:journals/pacmpl/AbdullaAJN18,DBLP:conf/oopsla/NorrisD13} or by being parametric with respect to an axiomatically-defined memory model~\cite{DBLP:conf/pldi/Kokologiannakis19,DBLP:conf/asplos/Kokologiannakis20}. In addition, a number of these works can operate under the coarser reads-from equivalence partitioning, including~\cite{DBLP:journals/pacmpl/AbdullaAJN18} and ~\cite{DBLP:conf/pldi/Kokologiannakis19,DBLP:conf/asplos/Kokologiannakis20}, which do so while maintaining optimality. TruSt builds on the foundations laid by GenMC~\cite{DBLP:conf/pldi/Kokologiannakis19} in order to achieve memory-model parametricity; however, it adapts the extensibility requirement on the underlying memory model to a more precise łmaximal extensibility requirement (see 3.1)

==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/si-ser.tex <==
%!TEX root = main.tex
\section{Swapping-based model checking for Snapshot Isolation and Serializability}\label{sec:ser}

%As show in section \ref{sec:proofs-algorithm}, algorithm \ref{algorithm:optimal-instantiated}'s completeness proof (theorem \ref{theorem:completeness}) is model-depending, as it heavily relies on its causal-extensibility. Immediately, the question of the algorithm's extensibility to stricter isolation levels arise. For understanding the difference between the formers and $\SI$ or $\SER$, let's analyze how algorithm \ref{algorithm:optimal-instantiated} behaves for the program depicted in figure \ref{fig:ser-non-optimal:a} under them. We study this example as it has exactly two consistent executions but a dead-lock one under $\SI$ and $\SER$.
For $\textsc{explore-ce}$, the part of strong optimality concerning \emph{not} engaging in fruitless explorations was a direct consequence of causal extensibility (of the isolation level). However, isolation levels such as SI and SER are \emph{not} causally extensible (see Section~\ref{ssec:causal_ext}). Therefore, the question we investigate in this section is whether there exists another implementation of $\textsc{explore}$ that can ensure strong optimality along with $I$-soundness and $I$-completeness for $I$ being SI or SER. We answer this question in the negative, and as a result, propose an SMC algorithm that extends $\textsc{explore-ce}$ by just filtering histories before outputting to be consistent with SI or SER.

\vspace{-1mm}
\begin{restatable}{theorem}{impossibility}
\label{th:impos}
If $I$ is \textit{Snapshot Isolation} or \textit{Serializability}, there exists no $\textsc{explore}$ algorithm that is $I$-sound, $I$-complete, and strongly optimal.
\vspace{-1mm}
\end{restatable}

The proof of Theorem~\ref{th:impos} \appendixver{given in App.~\ref{proof:impossibility} }defines a program with two transactions and shows that 
%We consider the program in Figure~\ref{fig:ser-non-optimal:prog}, and show that 
any concrete instance of $\textsc{explore}$ in Alg.~\ref{algorithm:algo-class} \emph{cannot be both} $I$-complete and strongly optimal.
%This program contains two transactions, where only the first 3 instructions in each transaction are important.


%As $\mathcal{P}$ is symmetric and every computed partial execution have at most one pending transaction, we can assume, without loss of generality, the oracle order where $T_1$ precedes $T_2$. In this setting, when $A$ execute the read event $r_1 \coloneqq a \gets \rd{x}$, it will only be able to read from $\init$. After completing $T_1$, it executes the read-event $r_2 \coloneqq b \gets \rd{x}$ from $T_2$. One one hand, if $r_2$ reads from $T_1$, then we obtain a consistent history that can be extended to a total consistent one, $h$. However, from $h$ we cannot swap any two transactions as $T_2$ depends on $T_1$, which also depends on $\init$. On the other hand, if $r_2$ reads from $\init$ we will obtain a history $h'$ that leads to a deadlock (figure \ref{fig:ser-non-optimal:c}) and cannot be swapped before $T_2$'s completion; otherwise we would obtain a partial history $h''$ with two pending transaction. To sum up, algorithm \ref{algorithm:optimal-instantiated} is incomplete for $\SI$ and $\SER$.
%
%This show that our proposal is not flexible enough to satisfy the constraints that new models may require. Therefore, we want to analyze what properties shall we weak for still obtaining a $\mathcal{M}$-sound, complete and optimal while employing polynomial memory; for $\SI$ and $\SER$ models. Let's suppose then that there exists such an algorithm $A \in \mathcal{S}_{\mathcal{M}}$ and see how it behaves under the same program $\mathcal{P}$. As $A$ is complete, whenever a $\iread$ event $r$ reading from some $\iwrite$ $w$ does not lead to an inconsistency, it will explore that possible history (the algorithm cannot deduce in advance if a dead-lock/inconsistency will appear later on). In particular, a consistent extension of the history shown in \ref{fig:ser-non-optimal:b} will be computed with either $\wrt{y}{1}$ or $\wrt{x}{2}$ in it. Without loss of generality, let's assume $w_2 \coloneqq \wrt{x}{2} \not \in h$. By definition of $\genericNext$ function, $a = \genericNext(h) \in h$, and as stated in lines \ref{algorithm:algo-class:exploreRead}, \ref{algorithm:algo-class:exploreStd}, the history $h \bullet a$ is an extension of $h$ that will always be explored. Moreover, as $A$ is $\mathcal{M}$-sound, $\texttt{N}(h')$ cannot return $w_2$ as $\lnot \ \textsc{IsConsistent}_{\mathcal{M}}(h' \bullet w_2)$ for any extension $h'$ of $h$. Therefore, there is a history $h'$ that extends $h$ where all events but those in $T_2$ $\po$-after $w_2$ will be executed. In conclusion, $\texttt{N}(h') = \bot$ but $h'$ is not total, so it must be a blocking execution. That contradicts $A$ is an optimal algorithm.


%Let's suppose on the contrary that such algorithm $A$ exists. As $A$ is complete, whenever a $\iread$ event $r$ reading from some $\iwrite$ $w$ does not lead to an inconsistency, it will explore that possible history. In particular, a consistent extension of the history shown in \ref{fig:ser-non-optimal:b} will be computed  with either $\wrt{y}{1}$ or $\wrt{x}{2}$ in it. Without loss of generality, let's assume $w_x \coloneqq \wrt{x}{2} \not \in h$. \textcolor{red}{Shall I develop this a bit more? how?}. As $A$ is weakly optimal, for every $a = \texttt{N}(h)$, $a \not\in h $ (otherwise $A$ will compute $h$ and $h \bullet a = h$); and as stated in lines \ref{algorithm:algo-class:exploreRead}, \ref{algorithm:algo-class:exploreStd}, the history $h \bullet a$ will always be explored. Moreover, as $A$ is $\mathcal{M}$-sound, $\texttt{N}(h')$ cannot return $w_x$ as $\lnot \ \textsc{IsConsistent}_{\mathcal{M}}(h' \bullet w_x)$, for any history $h'$ extending $h$. Therefore, there is an extension $h'$ of $h$ where all events but those in $T_2$ $\po$ after $w_x$ will be executed. In conclusion, $\texttt{N}(h') = \bot$ but $h'$ is not total, so it must be a blocking execution. That contradicts $A$ is an optimal algorithm.

%\begin{theorem}
%There is no algorithm in $\mathcal{S}_{\mathcal{M}} \cap \mathcal{O}^n_{\mathcal{M}}$, $n$ in $\mathbb{N}$, for neither SI nor SER.
%\label{theorem:si-ser-bad-models}
%\begin{comment}
%\begin{proof}
%
%\textcolor{red}{
%During this proof let's call $\mathcal{P}$ to the program depicted in \ref{fig:ser-non-optimal:a}. Let's suppose on the contrary that such algorithm $A$ exists. As $A$ is complete, whenever a $\iread$ event $r$ reading from some $\iwrite$ $w$ does not lead to an inconsistency, it will explore that possible history. In particular, a consistent extension of the history shown in \ref{fig:ser-non-optimal:b} will be computed  with either $\wrt{y}{1}$ or $\wrt{x}{2}$ in it. Without loss of generality, let's assume $w_x \coloneqq \wrt{x}{2} \not \in h$. \textcolor{red}{Shall I develop this a bit more? how?}. As $A$ is weakly optimal, for every $a = \texttt{N}(h)$, $a \not\in h $ (otherwise $A$ will compute $h$ and $h \bullet a = h$); and as stated in lines \ref{algorithm:algo-class:exploreRead}, \ref{algorithm:algo-class:exploreStd}, the history $h \bullet a$ will always be explored. Moreover, as $A$ is $\mathcal{M}$-sound, $\texttt{N}(h')$ cannot return $w_x$ as $\lnot \ \textsc{IsConsistent}_{\mathcal{M}}(h' \bullet w_x)$, for any history $h'$ extending $h$. Therefore, there is an extension $h'$ of $h$ where all events but those in $T_2$ $\po$ after $w_x$ will be executed. In conclusion, $\texttt{N}(h') = \bot$ but $h'$ is not total, so it must be a blocking execution. That contradicts $A$ is an optimal algorithm.
%}

%\underline{$S_{\mathcal{M}} \cap \mathcal{L}^1_{\mathcal{M}} = \emptyset$}. 

%Let's suppose on the contrary that such algorithm $A$ exists. As $A$ is in $\mathcal{L}^1_{\mathcal{M}}$ and $\mathcal{P}$ is symmetric, with out loss of generality we can assume $A$ execute first $T_1$ and then $T_2$. Then, it will execute the read event $r_1 \coloneqq a \gets \rd{x}$, which can only read from $\init$. After $T_1$, it executes the first event of $T_2$: $r_2 \coloneqq b \gets \rd{x}$. If $r_2$ reads from $T_1$, then we obtain a consistent history that can be extended to a total consistent one, $h$. However, from $h$ we cannot swap any two transactions as $T_2$ depends on $T_1$, which also depends on $\init$. On the other hand, if $r_2$ reads from $\init$, we will obtain a history $h'$ that leads to a deadlock and cannot be swapped before $T_2$'s completion; otherwise $A$ would have two pending transaction. Therefore, $A$ would only explore exactly one execution, so it is incomplete. This contradicts $A$ is in $\mathcal{L}^1_{\mathcal{M}}$.

%from this history, there %only has two transactions, $A$ can either execute the first or the second transaction at a time. As $A$ is complete and the history depicted in \ref{fig:ser-non-optimal:b} is consistent, there is an execution $h$ extending that history
%As after executing any event, $A$ has no information on the future events' availability, it will explore any possible consistent history. 

%\textcolor{red}{The first case is due to the non-$\wro \cup \so$-maximality of SI, SER (second example we discussed). The second one is the example when there is only one branch computed (first example we discussed).}
%\end{proof}
%\end{comment}
%\end{theorem}
%
%In particular, the program in figure \ref{fig:ser-non-optimal} shows that both $\SI$ and $\SER$ are actually not causally-extensible. Nevertheless, we present a swapping-based $\mathcal{M}$-sound, complete, weakly optimal algorithm employing polynomial memory based on \ref{algorithm:optimal-instantiated}:

Given this negative result, we define an implementation of $\textsc{explore}$ for an isolation level $I\in\{SI,SER\}$ that ensures optimality instead of strong optimality, along with soundness, completeness, and polynomial space bound. Thus, let $\textsc{explore-ce}(I_0)$ be an instance of $\textsc{explore-ce}$ parametrized by $I_0\in \{\RC,\RA,\CC\}$. We define an implementation of $\textsc{explore}$ for $I$, denoted by $\textsc{explore-ce}^*(I_0,I)$, which is exactly $\textsc{explore-ce}(I_0)$ except that 
% extension of any instance of $\textsc{explore-ce}$ parametrized by a prefix-closed and causally-extensible isolation level $I$ which is weaker than SI, which is only optimal and not strongly optimal.
% that for isolation levels $I$ like SI and SER has the same guarantees except that it is only optimal and not strongly optimal.
%any $\textsc{explore-ce}$ parametrized isolation level $I$, which 
instead of $\genericEvaluate(\hist) ::= true$, it uses 
\vspace{-1mm}
\begin{equation*}
	\begin{array}{ccc}
		\genericEvaluate(\hist) & \coloneqq & \hist \mbox{ satisfies }I
	\end{array}
\vspace{-1mm}
\end{equation*}
$\textsc{explore-ce}^*(I_0,I)$ enumerates exactly the same histories as $\textsc{explore-ce}(I_0)$ except that it outputs only histories consistent with $I$. The following is a direct consequence of Theorem~\ref{th:corr}.
%because the set of histories admitted by a program under $I\in\{SI,SER\}$ is a subset of the set of histories admitted under $I_0\in \{\RC,\RA,\CC\}$.

\vspace{-1mm}
\begin{corollary}
%For any $I_0\in \{\RC,\RA,\CC\}$ and $I\in\{SI,SER\}$, $\textsc{explore-ce}^*(I_0,I)$ is $I$-sound, $I$-complete, optimal, and polynomial space.
For any isolation levels $I_0$ and $I$ such that $I_0$ is prefix-closed and causally extensible, and $I_0$ is weaker than $I$, $\textsc{explore-ce}^*(I_0,I)$ is $I$-sound, $I$-complete, optimal, and polynomial space.
\end{corollary}

%Note that the corollary above extends to any isolation level $I_0$ which is prefix closed and causally extensible and any isolation level $I$ which is stronger than $I_0$.

%\textcolor{red}{Discuss the exponential total branches ditched}
%The reason why theorem \ref{theorem:si-ser-bad-models} holds for $\SI$ and $\SER$ but not for the rest of isolation levels described in \ref{fig:consistency_defs} is due to the lack of causal-extensibility. Nevertheless, weakening

% Under any of them the event $\wrt{x}{2}$ would always be eligible to be added to the aforementioned history $h$, and therefore any final dead-lock would be reached.



==> CausalCons.-DPOR/CausalCons.-DPOR-Paper/swaps.tex <==
%!TEX root = main.tex
\subsection{Re-Ordering Events in Histories}
\label{subsection:SwappingHistories} %Provisional

After extending the current history with one more event, $\textsc{explore}$ may be called recursively on other histories obtained by re-ordering events in the current one (and dropping some other events).
%Besides sound and complete, we would also seek for an optimal algorithm, i.e. that avoids computing a history $h$ whose extensions are all inconsistent; also called a \textit{blocking} execution. If this is not achieved, our search would employ more resources such as time or memory than it actually needs for doing its purpose.

\begin{figure}[t]
\vspace{-1mm}

	\centering
	\begin{subfigure}[b]{.25\textwidth}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{c||c}
\begin{lstlisting}[xleftmargin=5mm,basicstyle=\ttfamily\scriptsize,escapeinside={(*}{*)}, tabsize=1]
begin;
a = read((*x*));
b = read((*y*));
commit
\end{lstlisting} &
\begin{lstlisting}[xleftmargin=5mm,basicstyle=\ttfamily\scriptsize,escapeinside={(*}{*)}, tabsize=1]
begin;
write((*$x$*),2);
write((*$y$*),2);
commit
\end{lstlisting} 
\end{tabular} 
\end{adjustbox}
\vspace{1.2cm}
%		}
		\caption{Program \nver{(2 sessions)}.}
		\label{fig:dead_branch:prog}
	\end{subfigure}
\centering
	\begin{subfigure}[b]{.125\textwidth}
		\resizebox{\textwidth}{!}{
			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
				semithick, transform shape]
				
				%\\ \multicolumn{1}{c}{ \ldots}
				\node[draw, rounded corners=2mm,outer sep=0] (t1) at (-3.25, 0) {\begin{tabular}{l} $\init$ \end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]50:$t_1$}] (t2) at (-3.25, -1.6) {\begin{tabular}{l} 
						$\rd{x}$ \\ $\rd{y}$
				\end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]50:$t_2$}] (t3) at (-3.25, -3.2) {\begin{tabular}{l} 
						$\wrt{x}{2}$\pgfsetfillopacity{0.3}\\
						$\wrt{y}{2}$
				\end{tabular}};			
				
				\path (t1.south west) -- (t1.south) coordinate[pos=0.67] (t1x);
				\path (t1.south east) -- (t1.south) coordinate[pos=0.67] (t1y);
				\path (t2.north west) -- (t2.north) coordinate[pos=0.67] (t2x);
				\path (t2.north east) -- (t2.north) coordinate[pos=0.67] (t2y);
				
				\path (t1.south) edge [left] node {$\wro$} (t2.north);

				%\path (t2) edge [right] node {$\wro_x$} (t3);
			\end{tikzpicture}  
			
		}
		\caption{Current.}
		\label{fig:dead_branch:a}
	\end{subfigure}
	\hspace{.175cm}
	\centering
	\begin{subfigure}[b]{.125\textwidth}
		\resizebox{\textwidth}{!}{
			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
				semithick, transform shape]
				\node[draw, rounded corners=2mm,outer sep=0] (t1) at (-3.25, 0) {\begin{tabular}{l} $\init$ \end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]50:$t_2$}] (t2) at (-3.25, -3.2) {\begin{tabular}{l} 
						$\rd{x}$ \pgfsetfillopacity{0.3}\\ $\rd{y}$
				\end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]50:$t_1$}] (t3) at (-3.25, -1.6) {\begin{tabular}{l} 
						$\wrt{x}{2}$\pgfsetfillopacity{0.3}\\
						$\wrt{y}{2}$
				\end{tabular}};			
				
				\path (t1.south west) -- (t1.south) coordinate[pos=0.67] (t1x);
				\path (t2.north west) -- (t2.north) coordinate[pos=0.67] (t2x);
				\path (t3.north west) -- (t3.west) coordinate[pos=0.67] (t3x);
				
				\path (t3.south) edge [left] node {$\wro_x$} (t2.north); %[yshift=8,xshift=0]
				%\path (t1x) edge [right] node {$\wro_y$} (t2x);
			\end{tikzpicture}  
			
		}
		\caption{Reorder.}
		\label{fig:dead_branch:b}
	\end{subfigure}
	\hspace{.175cm}
	\centering
		\begin{subfigure}[b]{.177\textwidth}
		\resizebox{\textwidth}{!}{
			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
				semithick, transform shape]
				\node[draw, rounded corners=2mm,outer sep=0] (t1) at (-3.25, 0) {\begin{tabular}{l} $\init$ \end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]50:$t_2$}] (t2) at (-3.25, -3.2) {\begin{tabular}{l} 
						$\rd{x}$ \\ $\rd{y}$
				\end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]50:$t_1$}] (t3) at (-3.25, -1.6) {\begin{tabular}{l} 
						$\wrt{x}{2}$\pgfsetfillopacity{0.3}\\
						$\wrt{y}{2}$
				\end{tabular}};			
				
				\path (t1.south west) -- (t1.south) coordinate[pos=0.67] (t1x);
				\path (t2.north west) -- (t2.north) coordinate[pos=0.67] (t2x);
				\path (t3.north west) -- (t3.west) coordinate[pos=0.67] (t3x);
				
				%\path (t3x) edge [above] node[yshift=8,xshift=0] {$\wro_x$} (t2.north east);
				\path (t3.south) edge [left] node {$\wro_x$} (t2.north);
				\path (t1.south west) edge [bend right=40] node[left] {$\wro_y$} (t2.north west);
			\end{tikzpicture}
		}
		\caption{Extended.}
		\label{fig:dead_branch:c}
	\end{subfigure}
	\hspace{.175cm}
	\centering
	\begin{subfigure}[b]{.177\textwidth}
		\resizebox{\textwidth}{!}{
			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
				semithick, transform shape]
				\node[draw, rounded corners=2mm,outer sep=0] (t1) at (-3.25, 0) {\begin{tabular}{l} $\init$ \end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]50:$t_2$}] (t2) at (-3.25, -3.2) {\begin{tabular}{l} 
						$\rd{x}$ \\ $\rd{y}$
				\end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]50:$t_1$}] (t3) at (-3.25, -1.6) {\begin{tabular}{l} 
						$\wrt{x}{2}$\\
						$\wrt{y}{2}$
				\end{tabular}};			
				
				\path (t1.south west) -- (t1.south) coordinate[pos=0.67] (t1x);
				\path (t2.north west) -- (t2.north) coordinate[pos=0.67] (t2x);
				\path (t3.north west) -- (t3.west) coordinate[pos=0.67] (t3x);
				
				%\path (t3x) edge [above] node[yshift=8,xshift=0] {$\wro_x$} (t2.north east);
				\path (t3.south) edge [left] node {$\wro_x$} (t2.north);
				\path (t1.south west) edge [bend right=40] node[left] {$\wro_y$} (t2.north west);
			\end{tikzpicture}
			
		}
		\caption{Inconsistent.}
		\label{fig:dead_branch:d}
	\end{subfigure}
	\vspace{-2.5mm}
	\caption{Example of inconsistency after swapping two events. All $\so$-edges from $\init$ to the other transactions are omitted for legibility. The history order $<$ is represented by the top to bottom order in each figure.
	%All transaction logs are history-ordered top to bottom according to their position in the figure. 
	Events in gray are not yet added to the history. }
	\label{fig:dead_branch}
	\vspace{-4mm}
\end{figure}
%\vspace{-2mm}

%Proceeding this way we can ensure that every complete history is not inconsistent, but we cannot yet ensure every incomplete consistent history lead to a complete and consistent one. Guaranteeing it would mean that every step done in the algorithm is meaningful; that any explored branch would lead to a dead end. 
%The process of re-ordering events must maintain the invariant that the algorithm explores histories with at most one pending transaction, 
Re-ordering events must preserve the invariant of producing histories with at most one pending transaction.
To explain the use of this invariant in avoiding fruitless explorations, let us consider the program in Figure~\ref{fig:dead_branch:prog} assuming an exploration under Read Committed. The oracle order gives priority to the transaction on the left.
Assume that the current history reached by the exploration is the one pictured in Figure~\ref{fig:dead_branch:a} (the last added event is $\wrt{x}{2}$). Swapping $\wrt{x}{2}$ with $\rd{x}$ would result in the history pictured in Figure~\ref{fig:dead_branch:b}. To ensure that this swap produces a new history which was not explored in the past, the $\wro_x$ dependency of $\rd{x}$ is changed towards the $\wrt{x}{2}$ transaction (we detail this later).
By the definition of $\nextEvent$ (and the oracle order), this history shall be extended with $\rd{y}$, and this read event will be associated by $\wro_y$ to the only available $\iwrite(y,\_)$ event from $\init$. This is pictured in 
Figure~\ref{fig:dead_branch:c}. The next exploration step will extend the history with $\ewrt{y,2}$ (the only extension possible) which however, results in a history that does \emph{not} satisfy Read Committed, thereby, the recursive exploration branch being blocked.
%as there is only one $\iwrite(y,\_)$ event, the $\wro$ dependncy for this
%that writes $y$, $r_b$ must read from the very first transaction; as seen in Figure~\ref{fig:dead_branch:c}. However, when completing the third transaction we must inexorably admit that our history in Figure~\ref{fig:dead_branch:d} is inconsistent. Therefore, all the computation required to complete the unfinished transactions after the swap was in vain; we couldn't detect after computing $h_2$ the dead end.
% As $\nextEvent$ function always prioritize pending transactions
The core issue is related to the history in Figure \ref{fig:dead_branch:c} which has a pending transaction that is \emph{not} $(\so \cup \wro)^+$-maximal. Being able to extend such a transaction while maintaining consistency is not guaranteed by Read Committed (and any other isolation level we consider). Nevertheless, causal extensibility guarantees the existence of an extension for pending transactions that are $(\so \cup \wro)^+$-maximal. We enforce this requirement by restricting the explored histories to have at most one pending transaction. This pending transaction will necessarily be $(\so \cup \wro)^+$-maximal.

%
%Hence, for being always able to extend a history by invoking the model's causally-extensibility, we have to never produce pending transactions that are non $\so \cup \wro$-maximal. A simple solution is always executing histories in isolation, i.e. having exactly one pending transaction; thus, $\so \cup \wro$-maximal,  otherwise there would be a previous point where two pending transactions coexisted. To sum up, we are not going to swap just after executing a $\iwrite$ event but when its transaction is completed.

%TODO EXPLAIN THE DEFINITIONS BELOW

To enforce histories with at most one pending transaction, the function $\genericCompute$, which identifies events to reorder, has a non-empty return value only when the last added event is $\ecommit$ (the end of a transaction)\footnote{\nver{Aborted transactions have no visible effect on the state of the database so swapping an aborted transaction cannot produce a new meaningful history.}}. Therefore, in such a case, it returns pairs \oldver{ that contain some read $r$ and the last completed transaction log $t$}\nver{of some transaction log prefix ending in a read $r$ and the last completed transaction log $t$}, such that the transaction log containing $r$ and $t$ are \emph{not} causally dependent (i.e., related by $(\so \cup \wro)^*$) \nver{(the transaction log prefix ending in $r$ and $t$ play the role of the subsequences $\alpha$ and respectively, $\beta$ in the description of $\genericCompute$ from Section~\ref{sec:algs}). To simplify the notation, we will assume that $\genericCompute$ returns pairs $(r,t)$.}
%In particular, given $r$ and $t$, we define the subsequences $\alpha_{r,t} = \{r\}$ and $\beta_{r,t} = \{t' \ | \ (t', t) \in (\so \cup \wro)^* \land r < t' \}$ that represent the minimal information required for $\alpha, \beta$ comply with $\genericSwap$'s specifications. To simplify notation, we will assume $\genericCompute$ simply returns the pairs $(r,t)$.
%\begin{equation*}
%	\begin{array}{lcl}
\vspace{-0.5mm}
\begin{align*}
& \genericCompute(h_<)  \coloneqq  \{(r,t) \in \Events \times T \ | \ r \in \readOp{T} \land \writeVar{t}{\variable{r}}\land \trans{h}{r} < t\\ %[.5mm]
		%&& \hspace{1.9cm} \land\  \\ [1mm]
& \hspace{2.7cm} \land\ (\trans{h}{r},t)\not\in (\so \cup \wro)^*\land \mbox{$t$ is complete and it includes the last event in $<$}\} \\
%& \hspace{1.7cm} \land\ \mbox{$t$ is complete}   \} 
%			&& \mbox{where $t$ is the transaction log of the last event in $<$}
\end{align*}
\vspace{-9mm}
%	\end{array}
%\end{equation*}
\begin{figure}[t]
\centering
\begin{subfigure}[b]{.25\textwidth}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{c||c}
\begin{lstlisting}[xleftmargin=5mm,basicstyle=\ttfamily\scriptsize,escapeinside={(*}{*)}, tabsize=1]
begin;
a = read((*x*));
if(a == 0){
	abort
}
write((*$y$*),1)
commit
begin;
b = read((*x*));
commit		
\end{lstlisting} &
\begin{lstlisting}[xleftmargin=5mm,basicstyle=\ttfamily\scriptsize,escapeinside={(*}{*)}, tabsize=1]
begin;
write((*$y$*),3);
commit
begin;
write((*$x$*),4);
commit
	\end{lstlisting} 
\end{tabular} 
\end{adjustbox}
	
	\caption{Program \nver{(2 sessions)}.}
	\label{fig:compute-reordering:prog}
\end{subfigure} 
\hspace{.15cm}%\pgfsetfillopacity{0.3}\\
	\centering
	\begin{subfigure}[b]{.21\textwidth}
		\resizebox{.76\textwidth}{!}{
			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
				semithick, transform shape]
				
				%\\ \multicolumn{1}{c}{ \ldots}
				\node[draw, rounded corners=2mm,outer sep=0] (t0) at (0, 0) {\begin{tabular}{l} $\init$ \end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]65:$t_1$}] (t1) at (0, -1.3) {\begin{tabular}{l} 
					$\rd{x}$ \\ $\iabort$
				\end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]50:$t_2$}] (t2) at (0, -2.6) {\begin{tabular}{l} 
					$\rd{x}$
				\end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]50:$t_3$}] (t3) at (0, -3.6) {\begin{tabular}{l} 
					$\wrt{y}{3}$
				\end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]50:$t_4$}] (t4) at (0, -4.6) {\begin{tabular}{l} 
					$\wrt{x}{4}$
				\end{tabular}};			
				
				\path (t1.south west) -- (t1.south) coordinate[pos=0.67] (t1x);
				\path (t1.south east) -- (t1.south) coordinate[pos=0.67] (t1y);
				\path (t2.north west) -- (t2.north) coordinate[pos=0.67] (t2x);
				\path (t2.north east) -- (t2.north) coordinate[pos=0.67] (t2y);
				
				\path (t1.south) edge [left] node {$\so$} (t2.north);
				\path (t3.south) edge [left] node {$\so$} (t4.north);
				\path (t0.south) edge [left] node {$\wro_x$} (t1.north);\\
				\path (t0.south east) edge [bend left] node[right, pos=0.2] {$\wro_x$} (t2.north east);
				
				%\path (t2) edge [right] node {$\wro_x$} (t3);
			\end{tikzpicture}  
			
		}
		\caption{Current.}
		\label{fig:compute-reordering:a}
	\end{subfigure}
	\hspace{.15cm}
	\centering
	\begin{subfigure}[b]{.23\textwidth}

		\resizebox{.685\textwidth}{!}{
			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
				semithick, transform shape]
				\node[draw, rounded corners=2mm,outer sep=0] (t0) at (0, 0) {\begin{tabular}{l} $\init$ \end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]65:$t_1$}] (t1) at (0, -1.22) {\begin{tabular}{l} 
						$\rd{x}$ \\ $\iabort$
				\end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]50:$t_2$}] (t2) at (0, -4.6) {\begin{tabular}{l} 
						$\rd{x}$
				\end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]50:$t_3$}] (t3) at (0, -2.4) {\begin{tabular}{l} 
						$\wrt{y}{3}$
				\end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]50:$t_4$}] (t4) at (0, -3.6) {\begin{tabular}{l} 
						$\wrt{x}{4}$
				\end{tabular}};			
				
				\path (t1.south west) -- (t1.south) coordinate[pos=0.67] (t1x);
				\path (t1.south east) -- (t1.south) coordinate[pos=0.67] (t1y);
				\path (t2.north west) -- (t2.north) coordinate[pos=0.67] (t2x);
				\path (t2.north east) -- (t2.north) coordinate[pos=0.67] (t2y);
				
				\path (t1.south east) edge [bend left] node [right, pos=0.2] {$\so$} (t2.north east);
				\path (t3.south) edge [left] node {$\so$} (t4.north);
				\path (t0.south) edge [left] node {$\wro_x$} (t1.north);\\
				\path (t4.south) edge [left] node{$\wro_x$} (t2.north);
				 %[yshift=8,xshift=0]
				%\path (t1x) edge [right] node {$\wro_y$} (t2x);
			\end{tikzpicture}  

		}
		
				\caption{Swap $t_2$ and $t_4$.}
	
		\label{fig:compute-reordering:b}
	\end{subfigure}
	\hspace{.15cm}
	\centering
	\begin{subfigure}[b]{.21\textwidth}
		\resizebox{.58\textwidth}{!}{
				\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
				semithick, transform shape]
				\node[draw, rounded corners=2mm,outer sep=0] (t0) at (0, 0) {\begin{tabular}{l} $\init$ \end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]65:$t_1$}] (t1) at (0, -3.5) {\begin{tabular}{l} 
						$\rd{x}$ \\ \pgfsetfillopacity{0.3}$\wrt{y}{1}$ 
				\end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, opacity=0.3, label={[font=\small]50:$t_2$}] (t2) at (0, -4.7) {\begin{tabular}{l} 
						$\rd{x}$
				\end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]50:$t_3$}] (t3) at (0, -1.05) {\begin{tabular}{l} 
						$\wrt{y}{3}$
				\end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]50:$t_4$}] (t4) at (0, -2.2) {\begin{tabular}{l} 
						$\wrt{x}{4}$
				\end{tabular}};			
				
				\path (t1.south west) -- (t1.south) coordinate[pos=0.67] (t1x);
				\path (t1.south east) -- (t1.south) coordinate[pos=0.67] (t1y);
				\path (t2.north west) -- (t2.north) coordinate[pos=0.67] (t2x);
				\path (t2.north east) -- (t2.north) coordinate[pos=0.67] (t2y);
				
				\path[opacity=0.3] (t1.south) edge [left] node [left] {$\so$} (t2.north);
				\path (t3.south) edge [left] node {$\so$} (t4.north);
				\path (t4.south) edge [left] node {$\wro_x$} (t1.north);\\
				%\path (t4.south) edge [left] node{$\wro_x$} (t2.north);
				%[yshift=8,xshift=0]
				%\path (t1x) edge [right] node {$\wro_y$} (t2x);
			\end{tikzpicture}  
			
		}
		\caption{Swap $t_1$ and $t_4$.}
		\label{fig:compute-reordering:c}
	\end{subfigure}
	\vspace{-2mm}
	\caption{Re-ordering events. All $\so$-edges from $\init$ to other transactions are omitted for legibility. The history order $<$ is represented by the top to bottom order in each figure. Events in gray are deleted from the history.}
	\label{fig:compute-reordering}
	\vspace{-2mm}
\end{figure}

%\vspace{-6mm}
For example, for the program in Figure~\ref{fig:compute-reordering:prog} and history $h$ in Figure~\ref{fig:compute-reordering:a}, $\genericCompute(h)$ would return $(r_1, t_4)$ and $(r_2, t_4)$ where $r_1$ and $r_2$ are the $\rd{x}$ events in $t_1$ and $t_2$ respectively. 

For a pair $(r,t)$, the function $\genericSwap$ produces a new history $\hist'$ which contains all the events ordered before $r$ (w.r.t. $<$), the transaction $t$ and all its $(\so \cup \wro)^*$ predecessors, and the event $r$ reading from $t$. All the other events are removed. Note that the $\po$ predecessors of $r$ from the same transaction are ordered before $r$ by $<$ and they will be also included in $\hist'$. The history $\hist'$ without $r$ is a prefix of the input history $\hist$. By definition, the only pending transaction in $\hist'$ is the one containing the read $r$. The order relation is updated by moving the transaction containing the read $r$ to be the last; it remains unchanged for the rest of the events.
%
\begin{align*}
\genericSwap(h_<, r, t, \locals) \coloneqq \big( (h' = (h \setminus D) \oplus \wro(t,r), <'), \locals' \big), \text{where $\locals' = \locals \downarrow \events{h'}$} \\
 D = \{e |  r < e \land (\trans{h}{e},t)\not\in (\so \cup \wro)^*\} \mbox{ and }
<' = \big( < \downarrow (\events{h'}\setminus \events{\trans{h'}{r}}) \big) \cdot \trans{h'}{r} %\\[1mm]
%& \hspace{1cm}\mbox{.}
\end{align*}

Above, $h \setminus D$ is the prefix of $\hist$ obtained by deleting all the events in $D$ from its transaction logs; a transaction log is removed altogether if it becomes empty. Also, $\hist'' \oplus \wro(t,r)$ denotes an \emph{update} of the $\wro$ relation of $\hist''$ where any pair $(\_,r)$ is replaced by $(t,r)$. Finally, $<'' \cdot\ \trans{h'}{r}$ is an extension of the total order $<''$ obtained by appending the events in $\trans{h'}{r}$ according to program order.

%and $\wrt{y}{1}$ in $t_1$ 
Continuing with the example of Figure~\ref{fig:compute-reordering}, when swapping $r_1$ and $t_4$, all the events in transaction $t_2$ belong to $D$ and they will be removed. This is shown in Figure~\ref{fig:compute-reordering:c}. Note that transaction $t_1$ aborted in Figure~\ref{fig:compute-reordering:a} while it will commit in Figure~\ref{fig:compute-reordering:c} (because the value read from $x$ changed). When swapping $r_2$ and $t_4$, no event but the commit in $t_2$ will be deleted (Figure~\ref{fig:compute-reordering:b}).

%Following algorithm \ref{algorithm:algo-class}'s schema, we define two functions $\compute, \swap$ that plays the role of $\genericCompute, \genericSwap$ respectively. In addition, for the history $h' = \swap(h, r, w)$ we declare the algorithm order of $h'$, $\leq_{h'}$ as $\leq_{h'} = \leq_{(h \setminus \tr(r) ) \restriction_{h'}} \cup \{\langle e, e' \rangle \ | \ e \in h' \setminus \tr(r), e' \in \tr(r)\} \cup \po_{\tr(r) \restriction_{h'}}$.
%
%\begin{cframed}[pinegreen]
%	\begin{equation*}
%		\begin{array}{ccc}
%			\compute(h) & \coloneqq & \{(r,w) \in h^2 \ | \ r <_h w \land \variable{r} = \variable{w} \land w \in \tr(\last{h}) \} \\
%			\swap(h, r, w) & \coloneqq & (h \setminus D) \bullet_w r \\
%			& \text{where} & D = \{e \ | \ r \leq_h e \land \lnot (\tr(e) \ (\so \cup \wro)^* \ \tr(w))\}
%		\end{array}
%	\end{equation*}
%\end{cframed}


\subsection{Ensuring Optimality}\label{ssec:optimality}

%Conversely, adding a $\iwrite$ $w$ is more complicated, multiple events may read this new event; specifically. the number of possible histories is exponential, $2^{|\iread(h)|}$. Moreover, after changing a $\wro$-edge from a $\iread$ $r$, we have no knowledge of the rest of the event's presence: some conditional instruction may be executed after $r$ and it may be meaningless talking about them. Thus, checking for every possible set of $\iread$ events if reading from $w$ leads to something consistent is no reasonable. Therefore, we have to define a criterion to determine whose sets of read events shall be analyzed. One hand, the history $h \bullet w$ where no $\iread$ reads from $w$ has to be explored, with an algorithm order defined in an analogously as for any other aforementioned history. On the other hand, we select one $\iread$ $r$ that will be the first event in $h$ reading from $w$ while the ones that follow $r$ will have to be re-executed. As $r$ had already been executed, what at the end we produce is a swap between the relative orders of $r$ and $w$; so $r$ would be thereinafter called \textit{swapped}.

%As in a more formal way definition \ref{def:swapped} states, this read $r$ would be thereinafter called \textit{swapped}

%Moreover, after changing a $\wro$-edge, we have no knowledge of the rest of the event's presence: some conditional instruction may be executed after that $\iread$ and it may be meaningless talking about the rest of the events. Moreover, by the prefix-closedness of our model, an inconsistent history only leads to inconsistent ones; so there is no reasonable reason for exploring those. Thus, instead of generating every single one of them and check afterwards if they are consistent, we prefer to generate a small subset and only extends those ones that are consistent; by the prefix-closedness of our model, an inconsistent history only leads to inconsistent ones. %Therefore, we can detect inconsistencies early on.

%Our protocol is defined as follows: we will select one $\iread$ event that will be the first event in $h$ reading from $w$ while the ones that proceed $r$ will be marked as postponed; they will have to be re-executed. As in a more formal way definition \ref{def:swapped} states, This read $r$ would be thereinafter called \textit{swapped}:

%, and we will enforce the following properties: no event before $r$ will read from $w$, $r$ reads from $w$, every read after $r$ may or may not read from $w$. 
Simply extending histories according to $\genericNext$ and making recursive calls on re-ordered histories whenever they are $I$-consistent guarantees soundness and completeness, but it does not guarantee optimality. Intuitively, the source of redundancy is related to the fact that applying $\genericSwap$ on different histories may give the same result. 

\begin{figure}[t]
	\begin{subfigure}[b]{.25\textwidth}
\begin{adjustbox}{max width=.9\textwidth}
\begin{tabular}{c||c}
\begin{lstlisting}[xleftmargin=5mm,basicstyle=\ttfamily\footnotesize,escapeinside={(*}{*)}, tabsize=1]
begin;
write((*$x$*),2)
commit
\end{lstlisting} &
\begin{lstlisting}[xleftmargin=5mm,basicstyle=\ttfamily\footnotesize,escapeinside={(*}{*)}, tabsize=1]
begin;
a=read((*$x$*));
commit
\end{lstlisting} 
				
\\
\multicolumn{1}{c}{} & \multicolumn{1}{c}{}
\\
\begin{lstlisting}[xleftmargin=5mm,basicstyle=\ttfamily\footnotesize,escapeinside={(*}{*)}, tabsize=1]
begin;
b=read((*$x$*));
commit
\end{lstlisting} &
\begin{lstlisting}[xleftmargin=5mm,basicstyle=\ttfamily\footnotesize,escapeinside={(*}{*)}, tabsize=1]
begin;
write((*$x$*),4);
commit
\end{lstlisting}
\end{tabular} 
\end{adjustbox}
		
		\caption{Program \nver{(4 sessions)}}
		\label{fig:non-optimality:prog}
	\end{subfigure}
	\begin{subfigure}[b]{.17\textwidth}
		\resizebox{0.785\textwidth}{!}{
			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
				semithick, transform shape]
				\node[draw, rounded corners=2mm,outer sep=0] (t1) at (-3, 0) {\begin{tabular}{l} $\init$ \end{tabular}};
				
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]30:$t_1$}] (t2) at (-3, -1.0) {\begin{tabular}{l} $\wrt{x}{2}$ \end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]30:$t_2$}] (t3) at (-3, -2.0) {\begin{tabular}{l} $\rd{x}$ \end{tabular}};
				
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, opacity=0.3, label={[font=\small]30:$t_3$}] (t4) at (-3, -3.0) {\begin{tabular}{l} $\rd{x}$ \end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, opacity=0.3, label={[font=\small]30:$t_4$}] (t5) at (-3, -4.0) {\begin{tabular}{l} $\wrt{x}{2}$ \end{tabular}};
				
				\path (t1.south west) edge[above, bend right=50] node[left, pos=0.1] {$\wro$} (t3.north west);
				%\path (-4.5,-3.75) edge[-,dashed] (-1,-3.75);
			\end{tikzpicture}  
			
		}
		\caption{Before reading}
		\label{fig:non_optimality:a}
	\end{subfigure}
	\centering	
	\begin{subfigure}[b]{.17\textwidth}
		\resizebox{0.925\textwidth}{!}{
			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
				semithick, transform shape]
				\node[draw, rounded corners=2mm,outer sep=0] (t1) at (-3, 0) {\begin{tabular}{l} $\init$ \end{tabular}};
				
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]40:$t_1$}] (t2) at (-3, -1.0) {\begin{tabular}{l} $\wrt{x}{2}$ \end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]30:$t_2$}] (t3) at (-3, -2.0) {\begin{tabular}{l} $\rd{x}$ \end{tabular}};
				
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]35:$t_3$}] (t4) at (-3, -3.0) {\begin{tabular}{l} $\rd{x}$ \end{tabular}};
				
				\node[draw, rounded corners=2mm, label={[font=\small]30:$t_4$}] (t5) at (-3, -4.0) {\begin{tabular}{l} \textbf{\textcolor{blue}{$\wrt{x}{4}$}} \end{tabular}};
				
				%\path (t3) edge node {$\so$} (t5);
				%\path (t3) edge node {$\po$} (t3);
				%\path (t1) edge[below] node[yshift=-4,xshift=-4] {$\wro$} (t3_2);
				%\path (t2) edge[below] node[yshift=-4,xshift=4] {$\wro$} (t4_2);
%				\path (t1) edge[above] node[yshift=0,xshift=0] {$\wro$} (t3);
%				\path (t1) edge[below] node[yshift=-2,xshift=-2] {$\wro$} (t4);
				\path (t1.south west) edge[above, bend right=50] node[left, pos=0.1] {$\wro$} (t3.north west);
				\path (t1.south east) edge[below, bend left=50] node[right, pos=0.1] {$\wro$} (t4.north east);
				%\path (-4.5,-5.25) edge[-,dashed] (-1,-5.25);
			\end{tikzpicture}  
			
		}
		\caption{$t_3$ reads $\init$}
		\label{fig:non_optimality:b}
	\end{subfigure}
	\centering
	\begin{subfigure}[b]{.17\textwidth}
		\resizebox{1.\textwidth}{!}{
			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
				semithick, transform shape]
				\node[draw, rounded corners=2mm,outer sep=0] (t1) at (-3, 0) {\begin{tabular}{l} $\init$ \end{tabular}};
				
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]30:$t_1$}] (t2) at (-3, -1.0) {\begin{tabular}{l} $\wrt{x}{2}$ \end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]30:$t_2$}] (t3) at (-3, -2.0) {\begin{tabular}{l} $\rd{x}$ \end{tabular}};
				
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]35:$t_3$}] (t4) at (-3, -3.0) {\begin{tabular}{l} $\rd{x}$ \end{tabular}};
				
				\node[draw, rounded corners=2mm, label={[font=\small]30:$t_4$}] (t5) at (-3, -4.0) {\begin{tabular}{l} \textbf{\textcolor{blue}{$\wrt{x}{4}$}} \end{tabular}};
				
				
				\path (t1.south west) edge[above, bend right=50] node[left, pos=0.1] {$\wro$} (t3.north west);
				\path (t2.south east) edge[below, bend left=50] node[right, pos=0.1] {$\wro$} (t4.north east);
				%yshift=16, xshift=-2,
				%\path (-4.5,-5.25) edge[-,dashed] (-1,-5.25);
			\end{tikzpicture}  
			
		}
		\caption{$t_3$ reads $t_1$}
		\label{fig:non_optimality:c}
	\end{subfigure}
	\centering
	\begin{subfigure}[b]{.18\textwidth}
		\resizebox{.615\textwidth}{!}{
			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
				semithick, transform shape]
				\node[draw, rounded corners=2mm,outer sep=0] (t1) at (-3, 0) {\begin{tabular}{l} $\init$ \end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]30:$t_1$}] (t2) at (-3, -1.1) {\begin{tabular}{l} $\wrt{x}{2}$ \end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]30:$t_2$}] (t3) at (-3, -3.3) {\begin{tabular}{l} $\rd{x}$ \end{tabular}};
				
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, opacity=0.3, label={[font=\small]30:$t_3$}] (t4) at (-3, -4.4) {\begin{tabular}{l} $\rd{x}$ \end{tabular}};
				
				\node[draw, rounded corners=2mm, label={[font=\small]30:$t_4$}] (t5) at (-3, -2.2) {\begin{tabular}{l} $\wrt{x}{4}$ \end{tabular}};				
				
				\path (t5) edge[left] node {$\wro$} (t3);
				
			\end{tikzpicture}  
			
		}
		\caption{After swap.}
		\label{fig:non_optimality:d}
	\end{subfigure}
	\vspace{-2mm}	
	\caption{Re-ordering events versus optimality. We assume an oracle order orders transaction from left to right, top to bottom in the program. All transaction logs are history-ordered top to bottom according to their position in the figure. Events in gray are not yet added to the history.}
	\label{fig:non_optimality}	
	\vspace{-5mm}
\end{figure}


As a first example, consider the program in Figure~\ref{fig:non-optimality:prog} with 2 transactions that only read some variable $x$ and 2 transactions that only write to $x$, each transaction in a different session. Assume that $\textsc{explore}$ reaches the ordered history in Figure~\ref{fig:non_optimality:a} and $\genericNext$ is about to return the second reading transaction. $\textsc{explore}$ will be called recursively on the two histories in Figure~\ref{fig:non_optimality:b} and Figure~\ref{fig:non_optimality:c} that differ in the write that this last read is reading from (the initial write or the first write transaction). On both branches of the recursion, $\genericNext$ will extend the history with the last write transaction written in blue bold font. For both histories, swapping this last write with the first read on $x$ will result in the history in Figure~\ref{fig:non_optimality:d} (cf. the definition of $\genericCompute$ and $\genericSwap$). Thus, both branches of the recursion will continue extending the same history and optimality is violated. The source of non-optimality is related to $\wro$ dependencies that are \emph{removed} during the $\genericSwap$ computation. The histories in Figure~\ref{fig:non_optimality:b} and Figure~\ref{fig:non_optimality:c} differ in the $\wro$ dependency involving the last read, but this difference was discarded during the $\genericSwap$ computation. To avoid this behavior, $\genericSwap$ is enabled only on histories where the discarded $\wro$ dependencies relate to some ``fixed'' set of writes, i.e., latest\footnote{\nver{We use latest writes because they are uniquely defined. In principle, other ways of identifying some unique set of writes could be used.}} writes w.r.t. $<$ that \oldver{preserve consistency}\nver{guarantee consistency by causal extensibility} (see the definition of $\isMaximallyAdded{\_}{\_}$ below). 
%\nver{from their ``causal past'' (i.e., predecessors in $(\so \cup \wro)^+$)}, i.e., latest\footnote{\nver{We use latest writes because they are uniquely defined. In principle, other ways of identifying some unique set of writes could be used.}} writes w.r.t. $<$ that preserve consistency (see the definition of $\isMaximallyAdded{\_}{\_}$ below). 
\nver{By causal extensibility, a read $r$ can always read from a write which already belongs to its ``causal past'', i.e., predecessors in $(\so \cup \wro)^*$ excluding the $\wro$ dependency for $r$. For every discarded $\wro$ dependency, it is required that the read reads from the latest such write w.r.t. $<$.} In this example, re-ordering is enabled only when the second $\rd{x}$ reads from \oldver{$\ewrt{x,2}$}\nver{the initial write; $\ewrt{x,2}$ does not belong to its ``causal past'' (when the $\wro$ dependency of the read itself is excluded)}.


%Different branches of the recursion may lead to the same history also because $\genericSwap$ may give the same result on 
%thereby, violating optimality. 
\begin{figure}[t]
	
\begin{subfigure}[b]{.23\textwidth}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{c||c}
\begin{lstlisting}[xleftmargin=5mm,basicstyle=\ttfamily\scriptsize,escapeinside={(*}{*)}, tabsize=1]
begin;
a=read((*$x$*));
commit
\end{lstlisting} &
\begin{lstlisting}[xleftmargin=5mm,basicstyle=\ttfamily\scriptsize,escapeinside={(*}{*)}, tabsize=1]
begin;
b=read((*$y$*));
commit
\end{lstlisting} 
\\
\multicolumn{1}{c}{} & \multicolumn{1}{c}{}
\\
\begin{lstlisting}[xleftmargin=5mm,basicstyle=\ttfamily\scriptsize,escapeinside={(*}{*)}, tabsize=1]
begin;
write((*$y$*),3);
commit
\end{lstlisting} &
\begin{lstlisting}[xleftmargin=5mm,basicstyle=\ttfamily\scriptsize,escapeinside={(*}{*)}, tabsize=1]
begin;
write((*$x$*),4);
commit
\end{lstlisting}
\end{tabular} 
\end{adjustbox}

\caption{Program \nver{(4 sessions)}.}
\label{fig:redundant_Swap:prog}
\end{subfigure}
	\centering
	\begin{subfigure}[b]{.225\textwidth}
		\resizebox{.65\textwidth}{!}{
			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
				semithick, transform shape]
				\node[draw, rounded corners=2mm,outer sep=0] (t0) at (-3, 0) {\begin{tabular}{l} $\init$ \end{tabular}};
				
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]50:$t_1$}] (t1) at (-3, -1.075) {\begin{tabular}{l} $\rd{x}$\end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]50:$t_2$}] (t2) at (-3, -2.15) {\begin{tabular}{l} $\rd{y}$  \end{tabular}};
				
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]50:$t_3$}] (t3) at (-3, -3.225) {\begin{tabular}{l} $\wrt{y}{3}$ \end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]50:$t_4$}] (t4) at (-3, -4.3) {\begin{tabular}{l} $\wrt{x}{4}$ \end{tabular}};
				
				%\path (t0.south west) edge[above, bend right] node[left] {$\wro$} (t3.north west);
				\path (t0.south west) edge[above, bend right] node[left] {$\wro$} (t2.north west);
				\path (t0.south) edge node[left] {$\wro$} (t1.north);
				%\path (t0.south east) edge[above, bend left] node[left] {$\wro$} (t4.north east);
			\end{tikzpicture}  
		}
		\caption{Current history.}
		\label{fig:redundant_swap:a}
	\end{subfigure}
	\hspace{.25cm}
	\centering
	\begin{subfigure}[b]{.17\textwidth}
		\resizebox{.68\textwidth}{!}{
			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
				semithick, transform shape]
				\node[draw, rounded corners=2mm,outer sep=0] (t0) at (-3, 0) {\begin{tabular}{l} $\init$ \end{tabular}};
				
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]50:$t_1$}] (t1) at (-3, -1.1) {\begin{tabular}{l} $\rd{x}$ \end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]50:$t_2$}] (t2) at (-3, -3.3) {\begin{tabular}{l} $\rd{y}$ \end{tabular}};
				
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]50:$t_3$}] (t3) at (-3, -2.2) {\begin{tabular}{l} $\wrt{y}{3}$ \end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]50:$t_4$}] (t4) at (-3, -4.4) {\begin{tabular}{l} $\wrt{x}{4}$ \end{tabular}};
				
%				\path (t0.south west) edge[above, bend right] node[left] {$\wro$} (t3.north west);
				\path (t3.south) edge node[left] {$\wro$} (t2.north);
				\path (t0.south) edge node[left] {$\wro$} (t1.north);
				%\path (t0.south east) edge[above, bend left] node[left] {$\wro$} (t4.north east);
			\end{tikzpicture}  
		}
		
		\caption{Swap $t_2$ and $t_3$.}
		\label{fig:redundant_swap:b}
	\end{subfigure}
	\hspace{.25cm}
	\centering
	\begin{subfigure}[b]{.17\textwidth}
		\resizebox{.72\textwidth}{!}{
			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
				semithick, transform shape]
				\node[draw, rounded corners=2mm,outer sep=0] (t0) at (-3, 0) {\begin{tabular}{l} $\init$ \end{tabular}};
				
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]50:$t_1$}] (t1) at (-3, -2.2) {\begin{tabular}{l} $\rd{x}$ \end{tabular}};
%				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]50:$t_2$}] (t2) at (-3, -4.5) {\begin{tabular}{l} $\rd{y}$ \end{tabular}};
				
%				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]50:$t_3$}] (t3) at (-3, -6) {\begin{tabular}{l} $\wrt{y}{3}$ \end{tabular}};
				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, label={[font=\small]50:$t_4$}] (t4) at (-3, -1.1) {\begin{tabular}{l} $\wrt{x}{4}$ \end{tabular}};
				
				%\path (t0.south west) edge[above, bend right] node[left] {$\wro$} (t3.north west);
%				\path (t0.south west) edge[above, bend right] node[left] {$\wro$} (t2.north west);
				\path (t4.south) edge node[left] {$\wro$} (t1.north);
				%\path (t0.south) edge node[left] {$\wro$} (t4.north);
			\end{tikzpicture}  
		}
		
		\caption{Swap $t_1$ and $t_4$.}
		\label{fig:redundant_swap:c}
	\end{subfigure}
	%\hspace{.5cm}
\vspace{-2mm}
	\caption{Re-ordering the same read on different branches of the recursion.}
	\label{fig:redundant_swap}
	\vspace{-5mm}
\end{figure}

%there are two sources of redundancy in this case: (1) re-ordering the same read on different branches of the recursion, and (2) applying $\genericSwap$ on different histories may give the same result.
%TODO GIVE AN EXAMPLE FOR THE 1ST ISSUE. JUSTIFYING THE SWAPPED CONDITION. 
The restriction above is not sufficient, because the two histories for which $\genericSwap$ gives the same result may not be generated during the same recursive call (for different $\wro$ choices when adding a read).
For example, consider the program in Figure~\ref{fig:redundant_Swap:prog} that has four sessions each containing a single transaction. $\textsc{explore}$ may compute the history $h$ pictured in Figure~\ref{fig:redundant_swap:a}. Before adding transaction $t_4$, $\textsc{explore}$ can re-order $t_3$ and $t_2$ and then extend with $t_4$ and arrive at the history $h_1$ in Figure~\ref{fig:redundant_swap:b}. Also, after adding $t_4$, it can re-order $t_1$ and $t_4$ and arrive at the history $h_2$ in Figure~\ref{fig:redundant_swap:c}. However, swapping the same $t_1$ and $t_4$ in $h_1$ leads to the same history $h_2$, thereby, having two recursive branches that end up with the same input and violate optimality. Swapping $t_1$ and $t_4$ in $h_1$ should not be enabled because the $\erd{y}$ to be removed by $\genericSwap$ has been swapped in the past. Removing it makes it possible that this recursive branch explores that $\wro$ choice for $\erd{y}$ again.
%Therefore, two different histories will also be computed via swapping two transactions: $h_2$ if we swap $t_2$ and $t_3$  (Figure~\ref{fig:redundant_swap:b}) and $h_3$ if we swap $t_1$ and $t_4$(Figure~\ref{fig:redundant_swap:c}). However, from $h_2$ we can also swap $t_1$ and $t_4$ to produce a history that can be extended to $h_3$; obtaining twice the same history.

%Let's suppose we have a program $\mathcal{P}$ as depicted in figure \ref{fig:non_optimality}, assuming $\leq_{\ora}$ order transactions as presented from left to right, top to bottom. Then, the algorithm computes histories \ref{fig:non_optimality:a}, $h$, and \ref{fig:non_optimality:b}, $h'$. After adding $T_4$ in both $h,h'$ we can produce a swap between $r_a \coloneqq a \gets \rd{x}$ and $w_4 \coloneqq \wrt{x}{4}$; deleting the event $r_b \coloneqq b \gets \rd{x}$ as $\lnot(\tr(r_b) \ [\wro \cup \so]^+ \ \tr(w_4)) $. Therefore, after the swap in both cases we arrive to the history depicted in Figure~\ref{fig:non_optimality:c}; obtaining a non-optimal situation. 

%In conclusion, we cannot swap transactions without any restriction. As the example in figure \ref{fig:non_optimality} shows, the key of redundancy lies in every $\wro$ edge that is going to be modified or erased: if two histories only differ on those, the resultant history is the same.

The $\genericProtocol$ condition restricting re-orderings requires that the re-ordered history be $I$- consistent and that every read deleted by $\genericSwap$ or the re-ordered read $r$ (whose $\wro$ dependency is modified) reads from a latest valid write, \nver{cf. the example in Figure~\ref{fig:non_optimality},} and it is not already swapped, \nver{cf. the example in Figure~\ref{fig:redundant_swap}} (the set $D$ is defined as in $\genericSwap$):

\vspace{-5mm}
\begin{align*}
& \genericProtocol(h_<, r, t, \locals) \coloneqq \mbox{the history returned by }\genericSwap(h_<, r, t, \locals) \mbox{ satisfies }I\\
&\hspace{3.5cm}\land\ \forall r'\in \readOp{h}\cap (D\cup\{r\}).\ \lnot \swapped{h_<}{r'}\land \isMaximallyAdded{h_<}{r'}{t} 
%			\hspace{2cm}\text{where }  D = \{e \ | \ r < e \land (\trans{h}{e},\trans{h}{w})\not\in (\so \cup \wro)^*\} %  \\ \multicolumn{3}{c}{
\end{align*}
\vspace{-5mm}


%\vspace{-1mm}


%\nver{The $\genericProtocol$ condition restricting re-orderings requires that the re-ordered history be $I$-consistent and that every read deleted by $\genericSwap$ or the re-ordered read $r$ (whose $\wro$ dependency is modified) reads from the latest causal valid write.}

\begin{comment}
\begin{align*}
& \genericProtocol(h_<, r, t, \locals) \coloneqq \mbox{the history returned by }\genericSwap(h_<, r, t, \locals) \mbox{ satisfies }I\\
&\hspace{3.5cm}\land h = \isMaximallyAdded{h_<}{h \setminus (\{t' \ | \ r < t' \land (t', t) \not\in (\so \cup \wro)^*\} \cup r)} 
%			\hspace{2cm}\text{where }  D = \{e \ | \ r < e \land (\trans{h}{e},\trans{h}{w})\not\in (\so \cup \wro)^*\} %  \\ \multicolumn{3}{c}{
\end{align*}
\end{comment}

%\nver{The \textit{$(r,t)$-alternative history to $h$} $\alter{r}{t}{h}$ is a history that would have been obtained by an alternative swapping-based algorithm that, after adding $r$ in the same order than $\textsc{explore-sc}$, firstly it would have added every transaction causally dependent with $t$ in $h$ and then, every missing event following $\ora$. However, every event in $h_<$ whose $\wro$ differs from $\alter{r}{t}{h}_{\hat{<}}$ will differ because it does not read the latest causal value (according to $\hat{<}$). $\genericProtocol(h_<, r, t, \locals)$ is satisfied whenever $h$ coincide with its $(r,t)$-alternative history.}

%\nver{A history $h_<$ reads all causal latest values }

%A read $r$ reads from a latest valid transaction, denoted as $\isMaximallyAdded{h_<}{r}$, if reading from any other later transaction w.r.t. $<$ violates the isolation level $I$. Formally, assuming that $t$ is the transaction such that $(t,r)\in\wro$,

A read $r$ reads from a \nver{causally} latest valid transaction, denoted as $\isMaximallyAdded{h_<}{r}$, if reading from any other later transaction $t'$ w.r.t. $<$ \nver{which is in the ``causal past'' of $\trans{h_<}{r}$} violates the isolation level $I$. Formally, assuming that $t_r$ is the transaction such that $(t_r,r)\in\wro$ in $h$,

\vspace*{-3.5mm}
\begin{equation*}
\isMaximallyAdded{h_<}{r}{t} \coloneqq 
t_r = \max_{<} \left\{\begin{array}{ccc}
	\writeVar{t'}{\mathit{var}(r)} \land (t', \trans{h_<}{r}) \in (\so \cup \wro)^* \text{ in } h' \\
	\land \ h' \oplus r\oplus \wro(t',r) \models I 
	\end{array}
	\right\} \\
 %\forall t' \in \tlogs{\hist}. (t'\mbox{writes }\mathit{var}(r)\land t < t' < r) \implies (h \setminus \{e | r < e\}) \oplus \wro(t',r)\not\models I 
\end{equation*}
where $h' = h \setminus \{e \ | \ r \leq e \land (\trans{h}{e}, t) \not\in (\so \cup \wro)^* \}$.

%\nver{A read $r$ reads from a causally latest valid transaction, denoted as $\readsCasuallyLatest{h_<}{r}{t}$, if reading from any other later transaction $t'$ w.r.t. $<$ such that $\trans{h_<}{r}$ causally depends on violates the isolation level $I$. Formally, assuming that $t$ is the transaction such that $(t,r)\in\wro$ in $h$,} 

\begin{comment}
\begin{equation*}
\readsCasuallyLatest{h_<}{r}{t} \coloneqq 
\max_{<} \{\writeVar{t'}{\mathit{var}(r)} \land (t', \trans{h_<}{r}) \in (\so \cup \wro)^* \land h_< \oplus_j r \oplus \wro(t',r) \models I \}
%\forall t' \in \tlogs{\hist}. (t'\mbox{writes }\mathit{var}(r)\land t < t' < r) \implies (h \setminus \{e | r < e\}) \oplus \wro(t',r)\not\models I 
\end{equation*}
\end{comment}


We say that a read $r$ is \emph{swapped} in $\hist_<$ when (1) $r$ reads from a transaction $t$ that is a successor in the oracle order $<_{\ora}$ (the transaction was added by $\genericNext$ after the read), which is now a predecessor\footnote{The $\textsc{explore}$ maintains the invariant that every read follows the transaction it reads from in the history order $<$.} in the history order $<$, (2) there is no transaction \nver{$t'$} that is before $r$ in both $<_{\ora}$ and $<$, and which is a $(\so \cup \wro)^+$ successor of $t$, and (3) $r$ is the first read in its transaction to read from $t$. Formally, assuming that $t$ is the transaction such that $(t,r)\in\wro$, 
% of $r$ is the first in oracle order to be after transaction containing $w$ in $(\so \cup \wro)^+$, and 
%\begin{definition}
%	A $\iread$ event $r$ is \callout{swapped} if the following conditions hold:
%	\begin{itemize}
%		\item For $w= h.\wro(r)$, $w <_h r$ and $w >_{\ora} r$.
%		\item $\tr(r)$ is the first transaction that depends on $\tr(w)$: $\nexists T <_{\ora} \tr(r)$ s $T <_h \tr(r)$ and $\tr(w) \ (\so \cup \wro)^+ \ T$. %\textcolor{red}{Note: I changed $T \neq \tr(r)$ to $T <_{\ora} \tr(r)$ for the proof as by $\ora$-respectfulness (defined in proof's section), we obtain both are equivalent.}
%		\item $r$ is the first $\iread$ event that reads from $\tr(w)$: $\nexists r'\in \tr(r), r' \leq_{\ora} r$ such that $\tr(h.\wro(r')) = \tr(w)$
%	\end{itemize}
%	\label{def:swapped}
%\end{definition}
%
\vspace{-0.5mm}
\begin{align*}
& \swapped{h_<}{r}  \coloneqq t < r \land t >_{\ora} r 
\land \forall t' \in h.\ t' <_{\ora} \trans{h}{r} \implies (r < t'  \lor (t,t')\not\in (\so \cup \wro)^+) \\
&\hspace{2.5cm} \land\ \forall r' \in \readOp{h}.\ (t,r')\in\wro \implies (r',r)\not\in \po  %\trans{h}{w'} \neq \trans{h}{w}
\end{align*}

\nver{Condition (1) states a quite straightforward fact about swaps: $r$ could not have been involved in a swap if it reads from a predecessor in the oracle order which means that it was added by $\genericNext$ after the transaction it reads from. Conditions (2) and (3) are used to exclude spurious classifications as swapped reads. Concerning condition (2), suppose that in a history $h$ we swap a transaction $t$ with respect a
(previous) read event $r$. Later on, the algorithm may add a read $r'$ reading also from $t$. Condition (2) forbids $r'$ to be declared as swapped.
Indeed, taking $tr(h, r)$ as an instantiation of $t'$, $tr(h, r)$ is before $r'$ in both
$<_{or}$ and $<$ and it reads from the same transaction as $r'$, thereby, being a $(\so \cup \wro)^+$ successor of the transaction read by $r'$.
Condition (3) forbids that, after swapping $r$ and $t$ in $h$, later
read events from the same transaction as $r$ can be considered as swapped.}

\nver{
Showing that $I$-completeness holds despite discarding re-orderings is quite challenging. Intuitively, it can be shown that if some $\genericSwap$ is \emph{not} enabled in some history $h_<$ for some pair $(r,t)$ although the result would be $I$-consistent (i.e., $\genericProtocol(h_<, r, t, \locals)$ does not hold because some deleted read is swapped or does not read from a causally latest transaction), then the algorithm explores another history $h'$ which coincides with $h$ except for those deleted reads who are now reading from causally latest transactions. Then, $h'$ would satisfy $\genericProtocol(h_<, r, t, \locals)$, and moreover applying $\genericSwap$ on $h'$ for the pair $(r,t)$ would lead to the same result as applying $\genericSwap$ on $h$, thereby, ensuring completeness. 
}


%\nver{Intuitively, swapped events correspond to calls to $\genericSwap$ function. More concretly, a read $r$ from a history $h_<$ satisfies $\swapped{h_<}{r}$ if and only if there is a reachable history $h^p_{<^p}$ along with a transaction $t$ and a mapping $\locals$ such that $h^s = \genericSwap(h^p_{<^p}, r, t, \locals)$ and $\textsc{explore}(h^s_{<^s})$ can reach $h_{<}$. }

%\nver{Intuitively, there is a correpondance between an event $r$ being swapped in a history $\hist_<$, and existing a previous history $(h_p, <_p)$ that leads to $\hist_<$ after several recursive calls which one them is $\genericSwap((h_p, <_p), \alpha, r)$ for some $\alpha$.} 

%\nver{One should note that the strict definition of $\genericProtocol$ does not contradict with the $I$- completeness of the algorithm. Indeed, if a $\genericSwap$ call is not effectued (i.e. for a pair $(r,t)$ that belongs to $\genericCompute(h_<)$, the history $\hat{h}$ returned by $\genericSwap(h_<, r, t, \locals)$ is $I$-consistent but $\genericProtocol(h_<, r, t, \locals)$ does not hold), by definition of $\genericProtocol$ there must be a read event $r'$ in $\readOp{h}$ that is either swapped or not satisfying $\isMaximallyAdded{h_<}{r'}$. Briefly, there is a reachable history $h'$ where every deleted event reads from causal valid value and every non-deleted value read the same value it reads in $h$. This history always exists by causal-extensibility. Moreover, by construction $h'$ satisfies $\genericProtocol$. Thus, as $h$ and $h'$ coincide in the non-deleted values, $\genericSwap(h_<, r, t, \locals)$ can be obtained by calling to $\genericSwap(h'_{r'}, r, t, \locals')$.}
%for those events that will be deleted after swapping, 
%one can take slightly different branches when multiple $\wro$ alternatives arise, reaching another history $h'_{<'}$ where $\genericProtocol(h'_{<'}, r, t, \locals)$ holds. Note that causally-extensibility guarantees that for every read event $r'$, if $(t',r') \in \wro$ and $\tr(h_<,r) \in (\so \cup \wro)^*$ in $h_<$, regardless of what every other independent event reads, $r'$ can still read from $t'$ in the new branch. Hence, $\hat{h}$ can be reached by simply swapping $r$ and $t$ on $h'_{<'}$ instead.

%\nver{One should note that the strict definition of $\genericProtocol$ does not contradict with the $I$- completeness of the algorithm. Indeed, whenever for a pair $(r,t)$ belonging to $\genericCompute(h_<)$, the history $\hat{h}$ returned by $\genericSwap(h_<, r, t, \locals)$ is $I$-consistent but $\genericProtocol(h_<, r, t, \locals)$ does not hold, an alternative history to $h$, $\alter{r}{t}{h}$ satisfies the $\genericProtocol$ condition and the history returned by $\genericSwap(h_<, r, t, \locals)$ coincides with $\genericSwap(\alter{r}{t}{h}_{\hat{<}}, r, t, \locals)$. Indeed, $\alter{r}{t}{h}$ is always well-defined by $I$'s causal-extensibility and it is $I$-consistent by construction. Moreover, as every event where $h$ and $\alter{r}{t}{h}$ disagree is deleted by $\genericSwap$'s call and in $\alter{r}{t}{h}$ and reads a causal valid value, every step related to those events correspond to a simple call to $\textsc{explore-sc}$. In other words, $\alter{r}{t}{h}$ is reachable and both $h$ and its alternative histories coincide after swapping.}

%that is either swapped or not satisfying $\isMaximallyAdded{h_<}{r'}$. Briefly, for those events that will be deleted after swapping, one can take slightly different branches when multiple $\wro$ alternatives arise, reaching another history $h'_{<'}$ where $\genericProtocol(h'_{<'}, r, t, \locals)$ holds. Note that causally-extensibility guarantees that for every read event $r'$, if $(t',r') \in \wro$ and $\tr(h_<,r) \in (\so \cup \wro)^*$ in $h_<$, regardless of what every other independent event reads, $r'$ can still read from $t'$ in the new branch. Hence, $\hat{h}$ can be reached by simply swapping $r$ and $t$ on $h'_{<'}$ instead.} 
 
%\nver{One should note that when swapping a transaction $t$ with respect a read $r$ in a history $h$ for obtaining an $I$-consistent history $\hat{h}$, if the $\genericProtocol$ condition is not satisfied, there must be a read $r'$ that in swapped in $h$. Hence, there is a previous history $(h_p, <_p)$ where $r'$ is no swapped. By induction on the number of swapped events after $r$ in the history, one can conclude there is a previous history where $\genericProtocol$ is satisfied and that leads to $\hat{h}$. Therefore, $\genericProtocol$ condition achieves strong-optimality without loosing $I$-completeness.}

%Given a history $h$, if firstly some event $r$ is swapped with respect a transaction $t$ and later on in a second swap $r$ is deleted for obtaining a history $h'$, some computation made by the algorithm is lost. In particular, from $h$ we can construct a history $h''$ where we do not swap $r$ and we add every event after $r$ enforcing the wr relation to coincide for those added events with the history explored immediately before $h'$. If we do the second swap on $h''$ we would obtain again $h'$, thereby, completeness is not lost. For optimality, one of these two exploration paths must be discarded. We discard the one where swapped events are deleted.

%Intuitively, definition~\ref{def:max_added} allow us to detect when a $\iread$ event $r$ reads from some \textit{default} value, the last $\iwrite$ $w$ event writing $x$ that was added before $r$ and such that the resultant history is consistent. In general, the source of non-optimality comes from the existence of histories differing in some $\wro$-edge involving a transaction that will be deleted. Therefore, we can stablish a simple criterion for guaranteeing optimality: a swap between two events can only happen when every event that have to be re-executed is maximally added. This criterion is defined as function $\protocol$ and it will play the role of $\genericProtocol$ function in our algorithm \ref{algorithm:algo-class}'s instance.

%\begin{figure}[H]
%	
%	\centering
%	\begin{subfigure}[b]{.3\textwidth}
%		\resizebox{\textwidth}{!}{
%			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
%				semithick, transform shape]
%				
%				\node[draw, rounded corners=2mm,outer sep=0] (t1) at (-3, 0) {\begin{tabular}{l} $\wrt{x}{0}$ \\ $a \gets \rd{x}$ \end{tabular}};
%				\node[draw, rounded corners=2mm,outer sep=0] (t2) at (-3, -1.75) {\begin{tabular}{l} $b \gets \rd{x}$\end{tabular}};
%				\node[draw, rounded corners=2mm,outer sep=0] (t3) at (0, 0) {\begin{tabular}{l} $\wrt{x}{2}$ \\ $\wrt{y}{2}$\end{tabular}};
%				\node[draw, rounded corners=2mm, outer sep=0] (t4) at (3, -0) {
%					\begin{tabular}{l} 
%						$c \gets \rd{x}$ \\
%						{\pgfsetfillopacity{0.3}$\wrt{x}{3}$}
%				\end{tabular}};
%				\node[draw, rounded corners=2mm, opacity=0.3] (t5) at (3, -1.75) {\begin{tabular}{l} $\wrt{y}{4}$ \end{tabular}};
%				\path[opacity=0.3] (t4) edge node[opacity=0.3] {$\so$} (t5);
%				
%				
%				\path (t3.south east) -- (t3.east) coordinate[pos=0.67] (t3x);
%				\path (t4.south west) -- (t4.west) coordinate[pos=0.67] (t4x);
%				\path (t3x) edge[above] node[yshift=0,xshift=0] {$\wro_x$} (t4x);
%				
%				\path (t1.north west) -- (t1.north) coordinate[pos=0.5] (t1a);
%				\path (t1.west) edge [out=140, in=120, looseness=2.25] (t1a);
%				%[out=100,in=120,looseness=5] bend left=50, 
%				
%				\node[above left =0.125 and 0.05 of t1.north](t1alab) {$\wro_x$};
%				\path (t1) edge [left] node {$\wro_x$} (t2);
%			\end{tikzpicture}  
%			
%		}
%		\caption{Current history.}
%		\label{fig:add_write:a}
%	\end{subfigure}
%	\hspace{.5cm}
%	\centering
%	\begin{subfigure}[b]{.3\textwidth}
%		\resizebox{\textwidth}{!}{
%			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
%				semithick, transform shape]
%				\node[draw, rounded corners=2mm,outer sep=0] (t1) at (-3, 0) {\begin{tabular}{l} $\wrt{x}{0}$ \\ $a \gets \rd{x}$ \end{tabular}};
%				\node[draw, rounded corners=2mm,outer sep=0] (t2) at (-3, -1.75) {\begin{tabular}{l} $b \gets \rd{x}$\end{tabular}};
%				\node[draw, rounded corners=2mm,outer sep=0] (t3) at (0, 0) {\begin{tabular}{l} $\wrt{x}{2}$ \\ $\wrt{y}{2}$\end{tabular}};
%				\node[draw, rounded corners=2mm, outer sep=0] (t4) at (3, -0) {
%					\begin{tabular}{l} 
%						$c \gets \rd{x}$ \\
%						$\wrt{x}{3}$
%				\end{tabular}};
%				\node[draw, rounded corners=2mm, opacity=0.3] (t5) at (3, -1.75) {\begin{tabular}{l} $\wrt{y}{4}$ \end{tabular}};
%				\path[opacity=0.3] (t4) edge node[opacity=0.3] {$\so$} (t5);
%				
%				
%				\path (t3.south east) -- (t3.east) coordinate[pos=0.67] (t3x);
%				\path (t4.south west) -- (t4.west) coordinate[pos=0.67] (t4x);
%				\path (t3x) edge[above] node[yshift=0,xshift=0] {$\wro_x$} (t4x);
%				
%				\path (t4.south west) edge [bend left=15] node[above] {$\wro_x$} (t2.east);
%				
%				\path (t1.north west) -- (t1.north) coordinate[pos=0.5] (t1a);
%				\path (t1.west) edge [out=140, in=120, looseness=2.25] (t1a);
%				%[out=100,in=120,looseness=5] bend left=50, 
%				
%				\node[above left =0.125 and 0.05 of t1.north](t1alab) {$\wro_x$};
%				
%			\end{tikzpicture}  
%			
%		}
%		\caption{One possible swap.}
%		\label{fig:add_write:b}
%	\end{subfigure}
%	\hspace{.5cm}
%	\centering
%	\begin{subfigure}[b]{.29\textwidth}
%		\resizebox{\textwidth}{!}{
%			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
%				semithick, transform shape]
%				\node[draw, rounded corners=2mm,outer sep=0] (t1) at (-3, 0) {\begin{tabular}{l} $\wrt{x}{0}$ \\ $a \gets \rd{x}$ \end{tabular}};
%				\node[draw, rounded corners=2mm,outer sep=0, inner sep=0.75mm, opacity=0.3] (t2) at (-3, -1.75) {\begin{tabular}{l} $b \gets \rd{x}$\end{tabular}};
%				\node[draw, rounded corners=2mm,outer sep=0] (t3) at (0, 0) {\begin{tabular}{l} $\wrt{x}{2}$ \\ $\wrt{y}{2}$\end{tabular}};
%				\node[draw, rounded corners=2mm, outer sep=0] (t4) at (3, -0) {
%					\begin{tabular}{l} 
%						$c \gets \rd{x}$ \\
%						$\wrt{x}{3}$
%				\end{tabular}};
%				\node[draw, rounded corners=2mm, opacity=0.3] (t5) at (3, -1.75) {\begin{tabular}{l} $\wrt{y}{4}$ \end{tabular}};
%				\path[opacity=0.3] (t4) edge node[opacity=0.3] {$\so$} (t5);
%				
%				
%				\path (t3.south east) -- (t3.east) coordinate[pos=0.67] (t3x);
%				\path (t4.south west) -- (t4.west) coordinate[pos=0.67] (t4x);
%				\path (t3x) edge[above] node[yshift=0,xshift=0] {$\wro_x$} (t4x);
%				
%				\path (t4.north west) edge [bend right=15] node[above] {$\wro_x$} (t1.north east);
%				
%			\end{tikzpicture}  
%			
%		}
%		\caption{Another possible swap.}
%		\label{fig:add_write:c}
%	\end{subfigure}
%	\caption{Extensions of a history by adding a $\iwrite$ event.}
%	\label{fig:add_write}
%	%\vspace{-3mm}
%\end{figure}
%
%%\textcolor{red}{Talk about this example, explain why t2 disappears in 4.3}
%
%Let us show with an example the power of swapping. Here, in Figure~\ref{fig:add_write:a} we can see an incomplete history whose $\nextEvent$ event, $w \coloneqq \wrt{x}{3}$, is a $\iwrite$ event. There are four possible histories, depending if the first and second $\iread$ events, $r_a \coloneqq a \gets \rd{x} $ and $r_b \coloneqq b \gets \rd{x}$, read or not from $w$ (as $c \gets \rd{x}$ will never be able to read from $w$). In Figure~\ref{fig:add_write:b} we can see the history $h_b$ where only $r_b$ reads from $w$. As $r_a <_h r_b$, we simply state that $w \ [\wro] \ r_b$ in $h_b$. The other two cases that modify the write-read relation are due to the edge $w \ [\wro] \ r_a$; their common root. Therefore, we can construct the history $h_c$ depicted in Figure~\ref{fig:add_write:c}, mark $r_b$ as no executed to later on re-execute it and decide, in a later moment, if $w \ [\wro] \ r_b$ or not. In even in this small case we can realize that if $h_c$ would be inconsistent, we would already reduce the number of explored histories by one; its extensions would also be inconsistent. %we can delete $r_b$ for re-executing it later as depicted in Figure~\ref{fig:add_write:c} and by the rules described above, we know that two histories, one where $r_a$ reads from $w$ and another where it does not will be generated. 
%
%In a more general context, when swapping two events $r$ and $w$, we will delete all those events $e$ that are between $r$ and $w$ in the history-order such that $\tr(w)$ does not depends on. Otherwise, deleting some event $e$ such that $\tr(e) \ (\so \cup \wro)^* \ \tr(w)$ holds will produce a history where either some $\iread$ is reading from a deleted $\iwrite$ or some event would be executed before its $\so$-predecessor; both impossible situations in real life.




%The name ``swapping'' $w$ and $r$ refers to the change of relative order between those two events; $r <_{\ora} w$ but in the new history their order is reversed: $w <_h r$. Moreover, every event $e$ after $r$ that does not unlock $w$ (i.e. the condition $\tr(e) \ (\so \cup \wro)^+ \ \tr(w) $ does not hold) will be not taking into account to check this consistency. The reason for this is simple: if we want to compute every possible history, we may need to restate where some read-events read from, and we achieve this by re-executing them. To avoid redundancies, only those that $\tr(w)$ not depend on should being able to be re-executed.

%\begin{comment}
%\begin{algorithm}[H]
%\caption{\textsc{STMC}$_0$}
%\begin{algorithmic}[1]
%\InputAlgorithmic $h$: history.
%\If{ $\lnot \ \textsc{IsConsistent}_{\mathcal{M}}(h)$} \Return
%\ElsIf{$\textsc{IsComplete}(h)$}
%\State $\textsc{processHistory}(h)$
%\Else
%\State $a \gets  \nextEvent(h)$; $\; x \gets a.var()$
%\Switch{$a.type()$}
%\Case{$\ibegin$}
%\Comment{$\ibegin$ and $\iend$ cases coincide.}
%\EndCase
%\Case{$\iend$}
%\State $\textsc{STMC}_0(h \bullet a)$
%\Break
%\EndCase
%\Case{$\iread$}
%\ForAll{$w \in h \text{ s.t. } \writeVar{w}{x}$}
%\State $h' \gets h \bullet a$; $\; h'.\wro[a] \gets w$
%\State $\textsc{STMC}_0(h')$
%\EndFor
%\Break
%\EndCase
%\Case{$\iwrite$}
%\State $\textsc{STMC}_0(h \bullet a)$
%\ForAll{$r \in h \text{ s.t. } \readVar{r}{x}$}
%\State $D \gets \{e \ | \ r <_h e \land \lnot (\tr(e) \ (\so \cup \wro)^* \ \tr(a))\}$
%\State $h' \gets (h \setminus D) \bullet a$; $\; h'.\wro[r] \gets a$
%\State $\textsc{STMC}_0(h')$
%\EndFor
%\Break
%\EndCase
%\EndSwitch
%\EndIf
%
%\end{algorithmic}
%\label{algorithm:stmc0}
%\end{algorithm}
%\end{comment}




==> implementation.tex <==
\section{Implementation}

We implemented algorithm $\textsc{explore-ce}$ and $\textsc{explore-ce}^*$ on top of Java PathFinder (JPF) \textcolor{red}{cite JPF}, a verification tool for Java concurrent programs. We admit as input a Java program that (1) can be parsed and executed by JPF and (2) employs the API according to the specifications. Our tool is parametric in the isolation levels employed.

The API provided allow $\ibegin, \iwrite, \iread$ and $\icommit$ operations. Thanks to this API, we can maintain the database state separately from JPF's internal state and update the current history in each database call. We do not rely on any concrete database but store the information as a collection of String, one per write API call executed; along with the $\so$, $\wro$-dependencies between the events associated to them. Any time there is a need to connect data from the local state to the database one or viceversa we copy and store the concrete String value from one state to the other. %Altogether, we are able to simulate from simple variables to actual tables provided the client has proper methods to transform from one to the other representative.

Our implementation is compatible with JPF's standards, as both algorithm are instances of DFSearch; a JPF for DFS exploring algorithms. Moreover, we built consistency checkers based on the algorithm's presented in \textcolor{red}{Ranadeep and Enea's paper} for different isolation levels to ensure database's soundness. 

However, for performance issues, we developed an iterative version of the algorithm \ref{algorithm:algo-class} for reducing the actual memory consumption. We employ an annotated stack of database states that is modified in each $\textsc{explore-ce}$ call; and we consider the algorithm works with list instead of simply sets.
At every step where we execute a $\iread$, we annotate which $\iwrite$ event is reading from and  when the state pops from the stack, we change the $\wro$-dependency. Analogously, at every step we produce a swap, we annotate which tuple given by $\compute$ we used in the swap for selecting a different tuple when the state is popped out. % In addition, as JPF is not designed for supporting database operations, we developed an API that simulates every database instruction. operations, but they have been proved expressive enough both during our experiments and in real time applications. We admit any Java program that (1) can be parsed and executed by JPF and (2) has an equivalent translation into a program written with the syntax defined in Figure~\ref{fig:syntax}.


